Nearest Neighbors for Matrix Estimation Interpreted as Blind Regression for Latent Variable Model

We consider the setup of nonparametric {\em blind regression} for estimating the entries of a large $m \times n$ matrix, when provided with a small, random fraction of noisy measurements. We assume that all rows $u \in [m]$ and columns $i \in [n]$ of the matrix are associated to latent features $x_{\text{row}}(u)$ and $x_{\text{col}}(i)$ respectively, and the $(u,i)$-th entry of the matrix, $A(u, i)$ is equal to $f(x_{\text{row}}(u), x_{\text{col}}(i))$ for a latent function $f$. Given noisy observations of a small, random subset of the matrix entries, our goal is to estimate the unobserved entries of the matrix as well as to "de-noise" the observed entries. As the main result of this work, we introduce a nearest-neighbor-based estimation algorithm, and establish its consistency when the underlying latent function $f$ is Lipschitz, the underlying latent space is a bounded diameter Polish space, and the random fraction of observed entries in the matrix is at least $\max \left( m^{-1 + \delta}, n^{-1/2 + \delta} \right)$, for any $\delta > 0$. As an important byproduct, our analysis sheds light into the performance of the classical collaborative filtering algorithm for matrix completion, which has been widely utilized in practice. Experiments with the MovieLens and Netflix datasets suggest that our algorithm provides a principled improvement over basic collaborative filtering and is competitive with matrix factorization methods. Our algorithm has a natural extension to the setting of tensor completion via flattening the tensor to matrix. When applied to the setting of image in-painting, which is a $3$-order tensor, we find that our approach is competitive with respect to state-of-art tensor completion algorithms across benchmark images.

==> contents/aux_lemmas/auxlemmas.tex <==
\section{Auxiliary Concentration Inequalities}\label{sec:aux_concentration}
\chris{We can get rid of most of this ...}
\subsubsection*{Chernoff bound}
    There are various forms of Chernoff bounds, each of which are tuned to different assumptions. The following theorem gives the bound for a sum of independent Bernoulli trials.
    \begin{thm}\label{thm:Chernoff}
        Let $X = \sum_{i=1}^n X_i$, where $X_i = 1$ with probability $p_i$, and $X_i = 0$ with probability $1 - p_i$, and $X_i$'s are independent. Let $\mu = \Exp{X} = \sum_{i=1}^n p_i$. Then
        \begin{enumerate}
            \item Upper tail:	$ \Prob{X \geq (1+\delta) \mu} \leq \exp\left(-\frac{\delta^2}{2+\delta}\mu \right)$ for all $\delta > 0$.
            \item Lower tail: 	$ \Prob{X \leq (1-\delta) \mu} \leq \exp\left(-\frac{\delta^2}{2}\mu \right)$ for all $0 < \delta < 1$.
        \end{enumerate}
    \end{thm}
    	
    For $\delta \in (0,1)$, we can combine the upper and lower tails to obtain the following simpler bound:
        \[	\Prob{|X-\mu| \geq \delta \mu}\leq 2 \exp\left(-\frac{\mu \delta^2}{3}\right)\quad for~all~0< \delta< 1.	\]

\subsubsection*{Bernstein's inequality} 
    We will present a form of Bernstein's inequality for bounded random variables.
    \begin{thm}\label{thm:Bernstein}
        Suppose that $X_1, \ldots, X_n$ are independent random variables with zero mean, and that there exists a constant $M$ such that $|X_i| \leq M$ with probability 1 for each $i$. Let $\bar{S} := \frac{1}{n}\sum_{i=1}^n X_i$. Let variance of each
        random variable $X_i$ be bounded above by $V$, i.e. $\Var(X_i) \leq V$ for $1\leq i\leq n$. 
        Then for any $t \geq 0$,
        \[	\Prob{\left|\bar{S}\right| \geq t} \leq 2 \exp \left( -\frac{3nt^2}{6V + 2Mt} \right).	\]
    \end{thm}

    
\subsubsection*{Maurer-Pontil Inequality} This inequality provides bounds for the concentration of sample variance. 
		 \begin{lem}[Maurer-Pontil Inequality \cite{MaurerPontil09} Theorem 7]\label{lem:MaurerPontil}
        For $n \geq 2$, let $X_1, \dots X_n$ be independent random variables such that $X_i \in [a,b]$. Let $V(X)$ denote their sample variance, i.e., $V(X) = \frac{1}{2n(n-1)} \sum_{i,j} (X_i - X_j)^2$. Let $\sigma^2 = \Exp{V(X)}$ denote the true variance. For any $s > 0$,
        \begin{align*}
            \Prob{V(X) - \sigma^2 < - s} &\leq \exp\left(-\frac{(n-1)s^2}{2 (b-a)^2 \sigma^2}\right),
        \end{align*}
        and 
        \begin{align*}
            \Prob{V(X) - \sigma^2 > s} &\leq \exp\left(-\frac{(n-1)s^2}{ (b-a)^2 \left(2 \sigma^2 + s \right)}\right).
        \end{align*}
    \end{lem}
%    The Maurer-Pontil Inequality can be applied to any bounded random variable by normalizing it.
    
%    
%    \begin{coro}
%        For $n \geq 2$, let $X_1, \dots X_n$ be independent random variables such that $X_i \in (a,b)$. Let $V(X)$ denote their sample variance, i.e., $V(X) = \frac{1}{2n(n-1)} \sum_{i,j} (X_i - X_j)^2$. Let $\sigma^2 = \E[V(X)]$ denote the true variance. For any $\delta \in (0,1)$,
%        \begin{align*}
%            \Prob{\left|V(X) - \sigma^2\right| < s)} &\leq 2 \exp\left(-\frac{(n-1)s^2}{(b - a)^2 (2 \sigma^2 + s)}\right).
%        \end{align*}
%    \end{coro}

\subsubsection*{McDiarmid's inequality} While the previous inequalities showed concentration for specific quantities like the mean and variance, McDiarmid's inequality provides concentration results for general functions that satisfy the bounded difference condition. 
    \begin{thm}\label{thm:McDiarmid}
        Let $X_1, \ldots, X_n$ be independent random variables such that for each $i \in [n]$, $X_i \in \cX_i$. Let $\xi: \prod_{i=1}^n \cX_i \to \Reals$ be a function of $(X_1, \ldots, X_n)$ that satisfies $\forall i, \forall x_1, \ldots, x_n, \forall x_i' \in \cX_i$,
        $$    \left| \xi\left(x_1, \ldots, x_i, \ldots, x_n\right) - \xi\left(x_1, \ldots, x_i', \ldots, x_n\right) \right| \leq c_i.    $$
        Then for all $\eps > 0$,
        $$    \Prob{\xi - \Exp{\xi} \geq \eps} \leq \exp \left( \frac{-2 \eps^2}{\sum_{i=1}^n c_i^2} \right).$$
    \end{thm}
    By considering the negation of the function $-\xi$ in lieu of $\xi$, one can obtain the same tail bound for the opposite direction.

\subsubsection*{Kontorovich-Ramanan inequality} While the previous concentration inequalities require the independence assumption, the Kontorovich-Ramanan inequality uses the martingale method to provide concentration results for a class of dependent random sequences on a countable state space. We setup some definitions and notations used in the theorem statement. The theorem and its proof is presented in section 1.2 of \cite{KonRam2008}.

Consider a sequence of random variables $(X_1, \ldots, X_n)$ each of which takes values in a countable space $\cX$. Let the $\sigma$-algebra be the power set of $\cX^n$, which we denote by $\cF$. Let $\bP$ denote the probability measure on $(\cX^n, \cF)$. Let $\cX^n$ be equipped with the Hamming metric $d: \cX^n \times \cX^n \to \Reals_+$, defined by $d(x, y) := \sum_{i=1}^n \Ind\left\{ x_i \neq y_i \right\}$. 

The total variation distance $\left\| P - Q \right\|_{TV}$ between probability measures $P$ and $Q$ defined on a countable space $\cX$ with $\sigma$-algebra $\cF$ is defined as
$$    \left\| P - Q \right\|_{TV} := \sup_{A \in \cF} \left| P(A) - Q(A) \right| = \frac{1}{2}\sum_{x \in \cX} \left| P(x) - Q(x) \right|.$$
Given $1 \leq i < j \leq n$, let $x_i^j$ denote the subsequence $(x_i, x_{i+1}, \ldots, x_j)$. When $i=1$, $x_1^j$ will be written as $x^j$ for simplicity.
For any $1 \leq i < j \leq n$, $x^{i-1} \in \cX^{i-1}$ and $w, \hat{w} \in \cX$, define $\lambda_{ij}$ to be the total variation distance between the probability measures on $X_j^n$ conditioned on the sequences of the first $i$ letters and differing only at the $i$-th position. We denote the respective probability measures by $P_{X_j^n | X^i = x^{i-1} w}$ and $P_{X_j^n | X^i = x^{i-1} \hat{w}}$. Then 
$$    \lambda_{ij}\left(x^{i-1}, w, \hat{w}\right) := \left\| P_{X_j^n | X^i = x^{i-1} w } - P_{ X_j^n | X^i = x^{i-1} \hat{w} } \right\|_{TV}.$$ 
Define $\bar{\lambda}_{ij}$ to be the supremum over possible choices of $w$, $\hat{w}$, and sequences $x^{i-1}$ which have positive probability,
$$    \bar{\lambda}_{ij} := \sup_{x^{i-1} \in \cX^{i-1}, w, \hat{w} \in \cX \atop \Prob{X^i = x^{i-1}w} >0,  \Prob{X^i = x^{i-1}\hat{w}} >0 } \lambda_{ij} \left(x^{i-1}, w, \hat{w}\right).  $$
Finally, we define the mixing coefficient $\Delta_n$ to be
$$\Delta_n := \max_{i \in [n]} \left( 1 + \sum_{j=i+1}^n \bar{\lambda}_{ij}  \right).$$
We use a slightly different notation from the original paper; they used $\Delta_n$ to denote a matrix, and consider its operator norm, which we denote directly by $\Delta_n$.

\begin{thm}\label{thm:Kontorovich}
    Suppose $\cX$ is a countable space, $\cF$ is the power set of $\cX^n$, $\bP$ is a probability measure on $\left(\cX^n, \cF\right)$ and $\psi: \cX^n \to \Reals$ is a $L$-Lipschitz function with respect to the Hamming metric on $\cX^n$ and has mixing coefficient $\Delta_n$. Then for any $\eps > 0$,
    $$    \Prob{\left| \psi - \bE \psi \right| \geq \eps } \leq 2 \exp \left( \frac{-\eps^2}{2n L^2 \Delta_n^2} \right)    .$$
\end{thm}





\section{Geometry of Latent Probability Measure}\label{sec:aux_phi}

\subsubsection*{Existence of $\phi(\cdot)$} We show that a compact metric space admits the underestimator function which we denote by $\phi$ throughout this paper. For that purpose, we define the notion of regular points. We let $B\left(x, r\right)$ denote the open ball of radius $r$ centered at $x$.

\begin{defn}Let $(X, d)$ be a compact metric space and $\mu$ be a Borel probability measure on it. A point $x \in X$ is called regular if $\mu \left( B(x, r ) \right) > 0$, for all $r > 0$.
\end{defn}

\begin{lem}\label{lem:regular_closed}
    Let $R := \left\{ x \in X: x \text{ is regular}\right\}$. Then $R$ is closed, i.e., $\bar{R} = R$.
\end{lem}
\begin{proof}
    Suppose that $x \in \bar{R}$. For any $r > 0$, we can find a point $x_0 \in R$ such that $d(x, x_0) < \frac{r}{2}$.  We have $\mu\left( B\left( x_0, \frac{r}{2}\right) \right) > 0$ because $x_0 \in R$. It follows from $B\left(x_0, \frac{r}{2}\right) \subset B(x, r)$ that $\mu\left(B(x, r)\right) \geq \mu\left(B\left(x_0, \frac{r}{2}\right)\right) > 0 $. Therefore, $x \in R$ by definition. From this, we have $\bar{R} \subset R$, hence, $\bar{R} = R$.
\end{proof}

\begin{lem}\label{lem:regular_exists}
    If $S \subset X$ satisfies $\mu(S) > 0$, then there exists at least one regular point in the clousre of $S$, i.e., $R \cap \bar{S} \neq \emptyset$.
\end{lem}
\begin{proof}
    Assume there exists a set $S$ for which $\mu(S) > 0$ and $R \cap \bar{S} = \emptyset$. We know that $\bar{S}$ is compact because it is a closed subset of $X$. For $n = 1, 2, \ldots$, we consider a sequence of open coverings, $\cG_n := \left\{ B(x, \frac{1}{n}): x \in \bar{S} \right\}$, each of which is the family of open balls with radius $\frac{1}{n}$ centered at $x \in \bar{S}$. Due to the compactness of $\bar{S}$, we can find finite a subcover $\cG_n' = \left\{ B_1^{(n)}, \ldots, B_{N_n}^{(n)} \right\} \subset \cG_n$ for each $n$. Here, $N_n := \left| \cG_n' \right|$ is dependent on the choice of a subcover, and hence, not uniquely defined, however, we have $N_n < \infty$.
    
     For all $n = 1, 2, \ldots$, $S \subset \bar{S} \subset  \cup_{i=1}^{N_n} B_i^{(n)}$ since $\cG_n'$ is still a cover of $\bar{S}$. Therefore, we have $\mu (S) \leq \mu \left( \cup_{i=1}^{N_n} B_i^{(n)} \right) \leq N_n \max_i \mu\left( B_i^{(n)}\right)$. Let $z_n$ denote the center of $B_{i^*}^{(n)}$ where $i^* := \arg\max_i \mu\left( B_i^{(n)}\right)$. From the construction, $z_n \in \bar{S}$. Since $X$ is a metric space, $\bar{S}$ is not only compact, but also sequentially compact. Therefore, there is a convergent subsequence of $\left\{ z_n \right\}$, which converges to a point $z^* \in \bar{S}$. 
     
     This $z^*$ is a regular point. For any $r > 0$, we can find $n(r) > \frac{2}{r}$ such that $d(z_{n(r)}, z^*) < \frac{r}{2}$, since $\left\{ z_n \right\}$ has a convergent subseqeunce. Because 
     $$B\left( z_{n(r)}, \frac{1}{n(r)}\right) \subset B\left( z_{n(r)}, \frac{r}{2}\right) \subset B(z^*, r),$$
     we can conclude that $\mu\left( B(z^*, r) \right) \geq \mu \left( B\left( z_{n(r)}, \frac{1}{n(r)}\right) \right) \geq \frac{\mu(S)}{N_{n(r)}} > 0$. Therefore, $z^* \in R$, and $R \cap \bar{S} \neq \emptyset$.

\end{proof}

The following lemma ascertains that the set of regular points has the full measure, i.e., for almost every point in compact $X$, we can find a neighborhood of strictly positive measure.

\begin{lem} Let $(X, d)$ be a compact metric space and $\mu$ be a Borel probability measure on it. Define $R := \left\{ x \in X: x \text{ is regular}\right\}$. Then $R$ has the full measure in $X$, i.e., $\mu(R) = 1$.
\end{lem}
\begin{proof}
    For $n = 1, 2, \ldots, $, let $\cF_n := \left\{ B(x, \frac{1}{n}): x \in X \right\}$ be the family of open balls with radius $1/n$ centered at $x \in X$, each of which forms an open cover of $X$. Due to the compactness of $X$, we can find a finite subcover $\cF_n' \subset \cF_n$. Furthermore, we will filter out all zero-measure balls in $\cF_n'$ and leave only those having positive measure by defining
    \[    \cF_n'' := \left\{ B \in \cF_n' : \mu(B) > 0 \right\}. \]
Note that the choice of $\cF_n'$ (and hence, that of $\cF_n''$ also) is not unique. We suppose $\cF_n''$ is fixed from now on, but the following arguments hold for any choice of subcovering $\cF_n''$. 
    
%    First, we claim that $R \subset \cup_{B \in \cF_n''} B$. Assume that there exists a regular point $r \in R$, for which $r \not\in \cup_{B \in \cF_n''} B$. By definition of an open cover, there exists $x_0 \in X$ s.t. $r \in B\left( x_0, \frac{1}{n}\right)$ and $B\left( x_0, \frac{1}{n}\right) \in \cF_n' \setminus \cF_n''$. Let $s:= \frac{1}{n} - d(r, x_0)$; $B(r, s) \subset B\left(x_0, \frac{1}{n}\right)$. By definition of regular points, $\mu \left( B(r, s) \right) > 0$, but $B\left(x_0, \frac{1}{n}\right) \in \cF_n' \setminus \cF_n''$ implies that $\mu \left( B\left(x_0, \frac{1}{n}\right) \right) = 0$, which is a contradiction.
    
    Next, we claim that $\cup_{B \in \cF_{n}''}B \subset \cup_{x \in R} B\left(x, \frac{2}{n}\right) = R + B\left(0, \frac{2}{n}\right)$. From the construction above, $\mu(B) > 0$ for all $B \in \cF_n''$. By Lemma \ref{lem:regular_exists}, there exists a regular point $x_B \in R \cap \bar{B}$. Since $\cF_n''$ is a subfamily of $\cF_n$, $B = B\left(x_0, \frac{1}{n}\right)$ for some $x_0 \in X$. Therefore, for every $z \in B$, $d(x_B, z) \leq d(x_B, x_0) + d(x_0, z) < \frac{2}{n}$ by triangle inequality.  It follows that $B \subset B\left( x_B, \frac{2}{n}\right)$. Finally, $\cup_{B \in \cF_{n}''}B \subset \cup_{B \in \cF_n''} B\left(x_B, \frac{2}{n}\right) \subset \cup_{x \in R} B\left(x, \frac{2}{n}\right)$.
    
    
    For each $n = 1, 2, \ldots$, $\mu \left( \cup_{B \in \cF_{n}''}B \right) = 1$. Because $\cup_{B \in \cF_{n}'}B = \left(\cup_{B \in \cF_n'' }B \right) \cup \left(\cup_{B \in \cF_{n}'\setminus \cF_{n}''}B\right)$, we have $\mu \left( \cup_{B \in \cF_{n}'}B \right) \leq \mu\left(\cup_{B \in \cF_n'' }B \right) +  \mu \left(\cup_{B \in \cF_{n}'\setminus \cF_{n}''}B\right)$. Since $\cF_{n}'\setminus \cF_{n}''$ consists of a finite number of balls each of which has measure zero, $\mu \left(\cup_{B \in \cF_{n}'\setminus \cF_{n}''}B\right) = 0$. Therefore, $\mu \left( \cup_{B \in \cF_{n}'}B \right) \leq \mu\left(\cup_{B \in \cF_n'' }B \right)$. 
    
    Combining these with the fact that $X \subset \cup_{B \in \cF_n' }B$, we can conclude that
    $$ \mu \left( R + B\left(0, \frac{2}{n}\right) \right) \geq \mu\left(\cup_{B \in \cF_n'' }B \right) \geq \mu \left( \cup_{B \in \cF_{n}'}B \right) \geq \mu(X) = 1.$$
    Because $\bar{R} = \cap_{n=1}^{\infty} \left(R + B\left(0, \frac{2}{n}\right)\right)$ and $\left\{R + B\left(0, \frac{2}{n_1}\right) \right\}_{n=1}^{\infty}$ consists of a decreasing nested set,
    \begin{align*}
    	\mu\left(\bar{R}\right) &= \mu \left(\lim_{N \to \infty} \cap_{n=1}^{N} \left(R + B\left(0, \frac{2}{n}\right)\right) \right)\\
		& = \lim_{N \to \infty} \mu \cap_{n=1}^{N} \left(R + B\left(0, \frac{2}{n}\right)\right)\\
		&= \lim_{N \to \infty} \mu \left(R + B\left(0, \frac{2}{N}\right)\right)\\
		&= 1.
    \end{align*}
\end{proof}

\begin{lem}
    Let $(X, d)$ be a compact metric space, and $\mu$ be a Borel probability measure on it. Then there exists a function $\phi$ on $(X, d, \mu)$ which satisfies
    \begin{enumerate}
        \item $\phi: \Reals_{++} \to (0, 1]$,
        \item $\phi$ is nondecreasing, and
        \item $\mu\left( B(x, r) \right) \geq \phi(r)$, for all regular $x \in X$ and for all $r > 0$.
    \end{enumerate}
\end{lem}
\begin{proof}
    We define $\phi(r):= \inf_{x \in R} \mu \left( B(x, r) \right)$ and will show this $\phi$ satisfies the desired properties. 
    
    For any given $r > 0$, consider the open cover $\cG_r := \left\{ B\left(x, \frac{r}{2}\right) : x \in R \right\}$ of $R$. We know that $R$ is compact because it is a closed subset of $X$, which is compact. Therefore, we can find a finite subcover $\cG_r' = \left\{ B\left( z_i, \frac{r}{2}\right) \right\}_{i=1}^{N(r)} \subset \cG_r$ of $R$. For every $x \in R$, there should exist $z$ such that $B\left(z, \frac{r}{2} \right) \in \cG_r'$ and $d(x, z) < \frac{r}{2}$ because $\cG_r'$ is a cover of $R$. Therefore, $\mu \left( B\left( x, r \right) \right) \geq \mu \left( B\left(z, \frac{r}{2}\right) \right) \geq \min_{i=1, \ldots, N(r)} \mu \left( B\left(z_i, \frac{r}{2}\right) \right) > 0$. 
    
    Suppose that $r_1 > r_2 > 0$. By definition $\phi(r_1) = \inf_x \mu \left( B \left(x, r_1 \right) \right)$ and hence, for any $\eps > 0$, there exists $x_0(\eps) \in R$ such that $\mu \left( B \left(x_0(\eps), r_1 \right) \right) < \phi(r_1) + \eps$. For every $x \in R$, we have $ \mu\left(B \left(x, r_2 \right)\right) \leq \mu\left(B \left(x, r_1 \right)\right)$ because $ B \left(x, r_2 \right) \subset B \left(x, r_1 \right)$. It follows that $\phi(r_2) \leq \mu\left( B \left(x_0(\eps), r_2 \right) \right)  \leq \mu \left( B \left(x_0(\eps), r_1 \right) \right) < \phi(r_1) + \eps$. By taking the limit $\eps \to 0$, we can conclude that $\phi(r_2) \leq \phi(r_1)$. Therefore, $\phi$ is nondecreasing.
    
    The last property is obvious from the definition of $\phi$: for all $x \in R$, $ \mu \left( B(x, r) \right) \geq \inf_{x \in R} \mu \left( B(x, r) \right) = \phi(r)$.
\end{proof}


Let us consider two examples.
\begin{example}
Suppose $\prxa$ is a uniform measure over a unit cube in $d$ dimensional Euclidean space. 
Then 
$$    \inf_{x_0 \in \cX_1} \prxa\left(d_{\cX_1}(\bx, x_0) \leq r\right)= \min\left\{1,\left(\frac{r}{2} \right)^d\right\}.    $$
\end{example}

\begin{example}
Suppose $\prxa$ is supported only on a finite number of points, i.e., $\left| supp \prxa \right| = N$.
Then for any $r \geq 0$,
$$    \inf_{x_0 \in \cX_1} \prxa\left(d_{\cX_1}(\bx, x_0) \leq r\right) \geq \min_{i = 1, \ldots, N} \msra{x_i}.    $$
\end{example}


==> contents/matrix_proof/lemmas.tex <==

\subsection{Proof of Key Lemmas}

In this section we prove the five key lemmas introduced in the proof outline.

\subsubsection{Sufficiently many rows with large overlap} Using the fact that every entry is independently observed uniformly at random, we can prove Lemma \ref{lem:overlap}. It states that with high probability, for every entry $(u,i)$ which we might want to estimate, there are sufficiently many other rows $v$ for which entry $(v,i)$ is observed and there is a sufficiently large overlap $|\cO^{uv}|$ between rows $u$ and $v$. 

\begin{proof} [Proof of Lemma \ref{lem:overlap}]
	The set $\rowbase$ consists of all rows $v$ such that (a) entry $(v,i)$ is observed, and (b) $|\ovuv| \geq \beta$. With a fixed $u$, for each $v$, define binary random variables $Q_v$ and $R_{uv}$, such that $Q_v = 1$ if $(v,i) \in \cD$, i.e. $Z(v,i)$ is observed, and $0$ otherwise; $R_{uv} = 1$ if $|\ovuv| \geq \beta$ and $0$ otherwise. Then we can equivalently express the cardinality of the set as a sum over $m-1$ binary random variables
	\[|\rowbase| = \sum_{v \neq u} Q_v R_{uv}.\]
	If the events $\sum_{v \neq u} Q_v \in [a, b] $ and $\sum_{v \neq u} R_{uv} = m-1$ are satisfied, it implies $|\rowbase| = \sum_{v \neq u} Q_v R_{uv} \in [a,b]$. It follows from the contrapositive of this statement that
	\[ \left\{ |\rowbase| \not\in [a,b] \right\} \Rightarrow \left\{ \sum_{v \neq u} Q_v \not\in [a, b] \right\}  \vee \left\{ \sum_{v \neq u} R_{uv} < m-1 \right\} .\]
Therefore, by applying the union bound, we obtain that for any $0 \leq a < b \leq m-1$,
	\begin{align}\label{eq:lem1.1}
			\Prob{|\rowbase| \notin [a,b]} & \leq \Prob{\sum_{v \neq u} Q_v \notin [a,b]} + \Prob{\sum_{v \neq u} R_{uv} < m-1}.
	\end{align}
	Given that the entries within each row $v$ are sampled independently with probability $p$, it follows that $\sum_{v \neq u} Q_v$ is Binomial with parameters $(m-1)$ and $p$. We will choose the interval specified by endpoints $a = (1-\theta) (m-1) p$ and $b = (1+\theta) (m-1) p$. Directly applying Chernoff's bound (see Theorem \ref{thm:Chernoff} in Appendix \ref{sec:aux_concentration}) implies that for any $\theta \in (0, 1)$,
	\begin{align}\label{eq:lem1.2}
			\Prob{\left| \sum_{v \neq u} Q_v - (m-1)p \right| > \theta(m-1) p} &\leq 2 \exp\left(- \frac{\theta^2 (m-1)p}{3}\right). 
	\end{align}
	Next recall that the variable $R_{uv} \triangleq \Ind(|\ovuv| \geq \beta)$. Again due to the assumption that each entry is observed independently with probability $p$, it follows that $|\ovuv|$ is Binomial with parameters $n$ and $p^2$. Therefore, for any $\beta \in [2, np^2)$, by an application of Chernoff's bound for lower tails, it follows that for each $v \neq u$,
	\begin{align}
			 \Prob{R_{uv} = 0} & \leq \exp\left(-\frac{\left(np^2-\beta\right)^2}{2np^2}\right).
	\end{align}
By the union bound, it follows that
	\begin{align}\label{eq:lem1.3}
			\Prob{\sum_{v \neq u} R_{uv} < m-1} & \leq \sum_{v\neq u} \Prob{R_{uv} = 0}  ~ \leq (m-1) \exp\left(-\frac{\left(np^2-\beta\right)^2}{2np^2}\right).
	\end{align}
	By combining \eqref{eq:lem1.1}-\eqref{eq:lem1.3}, we obtain the desired result.
\end{proof}



\subsubsection{Concentration of sample mean and sample variance}
Assuming that the overlap between two rows $u$ and $v$ is sufficiently large, the sample mean and variance of the difference between the two rows will concentrates around their expected values.

\begin{proof}[Proof of Lemma  \ref{lem:mean}] 
	Conditioned on a particular realization of the latent features associated to rows $u$ and $v$, i.e. $\bx_1(u) = x_1(u), \bx_1(v) = x_1(v)$, the expected mean between the difference in their values $\muuv$ is a constant. Recall that the empirical mean $\muv$ is defined as 
	\begin{align}
			\muv & = \frac{1}{|\ovuv|} \left(\sum_{j \in \ovuv} Z(u,j) - Z(v,j)\right).
	\end{align}
	We would like to show that $\muv$ concentrates to $\muuv$. For any column $j$, recall that the column latent feature variable $\bx_2(j)$ is sampled according to $\prxb$, independently from the row features $\bx_1(u)$ and $\bx_1(v)$. The additive noise terms associated to each observation is an independent and zero-mean random variable. For each pair $(u,v)$, let us define a new independent random variable, 
	\[W_{uv}(j) = Z(u,j) - Z(v,j) \text{ for } j \in \ovuv,\]
	which has mean $\muuv$ when conditioned on $\bx_1(u) = x_1(u)$ and $\bx_1(v) = x_1(v)$. It follows then that $\tilde{W}_{uv}(j) = W_{uv}(j) - \muuv$ for $j \in \ovuv$ are zero-mean independent random variables conditioned on the row latent features. 
	
	Therefore, conditioned on $\bx_1(u) = x_1(u), \bx_1(v) = x_1(v)$ and the cardinality of overlap $\left|\ovuv \right|$, we can rewrite the difference $\muuv - \muv$ to be the average of $|\ovuv|$ independent, zero mean random variables $\tilde{W}_{uv}(j)$.	By the definition of $B_0 = L \diamxa + 2 B_e$ in \eqref{eq:def_B0}, $\left|W_{uv}(j) \right|$ is upper bounded by $B_0$ for every pair of rows $(u,v)$ and column $j$. It follows that $\left| \muuv \right| \leq B_0$, such that
	\[	\left| \tilde{W}_{uv}(j) \right| = \left| W_{uv}(j) - \muuv \right| \leq \left| W_{uv}(j) \right| + \left| \muuv \right| \leq 2 B_0.\]
In addition, conditioned on  $\bx_1(u) = x_1(u), \bx_1(v) = x_1(v)$, $\muuv$ is a constant so that
	\begin{align*}	Var\left(\tilde{W}_{uv}(j)\right) &= Var\left( W_{uv}(j) \right) = \Exp{W_{uv}(j)^2} - \Exp{W_{uv}(j)}^2\\
		& \leq \Exp{W_{uv}(j)^2} \leq B_0^2.
	\end{align*}
Therefore, an application of Bernstein's inequality (see Lemma \ref{thm:Bernstein}) for a sum of bounded random variables implies that
	\begin{align}
			&\Prob{\left|\mu_{\bx_1(u) \bx_1(v)} - \muv\right| > \mslack \left| \bx_1(u) = x_1(u), \bx_1(v) = x_1(v),  \left|\ovuv\right| \right. }\\
&\qquad\leq \exp\left(- \frac{3 | \ovuv| \mslack^2}{6 B_0^2 + 4 B_0 \mslack}\right). \nonumber
	\end{align}
	When $v \in \rowbase$, $|\ovuv| \geq \beta$. Further, since the above holds inequalities for all possibilities of $x_1(u), x_1(v)$, we conclude that
	\begin{align*}
			\Prob{\left|\muuv - \muv\right| > \mslack \left| v \in \rowbase \right. }	\leq \exp\left(- \frac{3 \beta \mslack^2}{6 B_0^2 + 4 B_0 \mslack}\right).
	\end{align*}
\end{proof}


Next we prove that the sample variance $s_{uv}^2$ converges to its expected value $\sigma_{x_1(u), x_1(v)}^2$ conditioned on the row latent features and a large enough overlap $\cO^{uv}$.
\begin{proof}[Proof of Lemma  \ref{lem:variance}]
	Recall $\sigma_{ab}^2 \triangleq \Var[f(a,\bx_2) - f(b,\bx_2)]$ for $a, b \in \cX_1$, $\bx_2 \sim \prxb$, and the sample variance between rows $u$, $v$ is defined as 
	\begin{align*}
			\suv^2 &= \frac{1}{2|\ovuv|(|\ovuv| - 1)} \sum_{j_1, j_2 \in \ovuv} \left( \left(Z(u,j_1) - Z(v,j_1)\right) - \left(Z(u,j_2) - Z(v,j_2)\right) \right)^2 \\
					&= \frac{1}{|\ovuv| - 1} \sum_{j \in \ovuv} \left( Z(u,j) - Z(v,j) - \muv \right)^2.
	\end{align*}
	Conditioned on $\bx_1(u) = x_1(u), \bx_1(v) = x_1(v)$, it follows from our model of independent additive noise that 
	\[\Exp{\suv^2 ~|~ x_1(u), x_1(v)} = \siguv^2 + 2 \gamma^2,\]
with respect to the randomness of the sampled latent column features induced by $\prxb$ and the independent noise terms. Recall as well that, $W_{uv}(j) = Z(u,j) - Z(v,j)$ are independent random variables conditioned on $\bx_1(u) = x_1(u), \bx_1(v) = x_1(v)$, where $\left|W_{uv}(j)\right| \leq B_0$, by the model assumptions and the definition of $B_0$ in \eqref{eq:def_B0}.
	
	Therefore, by an application of Maurer-Pontil inequality for the sample variance of a set of bounded random variables (see Lemma \ref{lem:MaurerPontil} in Appendix \ref{sec:aux_concentration}), it follows that 
	\begin{align}
			 \mathbb{P}\big(|\suv^2 - &(\sigma_{\bx_1(u)\bx_1(v)}^2 + 2 \gamma^2)| > \vslack \,\big|\, v \in \rowbase, \bx_1(u) = x_1(u), \bx_1(v) = x_1(v) \big) \nonumber \\
			& \qquad \leq 2 \exp\left(-\frac{\left(\beta - 1\right) \vslack^2}{4 B_0^2 (2 (\siguv^2 + 2 \gamma^2) + \vslack)}\right), \label{eq:lem.3.1}
	\end{align}
	where we used the property that $v \in \rowbase$ implies $|\ovuv| \geq \beta$. Since we assumed $\beta \geq 2$, $\beta - 1 \geq \beta/2$. By the same argument used in the proof of Lemma \ref{lem:mean}, we can bound $\siguv^2 + 2\gamma^2 =  Var\left( W_{uv}(j) \right) \leq \Exp{W_{uv}(j)^2} \leq B_0^2$
. Therefore, the right hand side of \eqref{eq:lem.3.1} can be bounded by 
	\begin{align}
			& \leq 2 \exp\left(-\frac{\beta \vslack^2}{8 B_0^2 (2 B_0^2 + \vslack)}\right).
	\end{align}
	Given that this bound is indepedent of $\bx(u), \bx(v)$, we can conclude the desired result. 
\end{proof}




\subsubsection{Sufficiently good k-nearest neighbors} We will next prove that with high probability, the $k$ rows in set $\cS_u^{\beta}(i)$ with the smallest values of $\sigma_{x_1(u) x_1(v)}^2$ are indeed ``close'', i.e. the variance is small. This result depends on the local geometry of the probability measure on the latent space, according to the function $\msr{\cdot}$. 
\begin{defn}
    Given a compact metric space $(\cX, d)$ equipped with a Borel probability measure $P_{\cX}$ and metric $d$, we define the measure underestimator function $\msr{\cdot}$ as the essential infimum of the measure of an $r$-ball. For $r > 0$,
    \[    \msr{r} := \ess \inf_{x \in \cX} P_{\cX} \left( B(x, r) \right), \]
    where $B(x,r) := \left\{ x' \in \cX : d(x, x') \leq r \right\}$.
\end{defn}
We recall the notion of essential infimum. For a function $f$ measurable on $(\cX, P_{\cX})$, its essential infimum on $\cX$ with respect to measure $P_{\cX}$ is defined as
$$	\ess \inf_{x \in \cX} f(x) = \sup \left\{ a: P_{\cX} \left(\left\{ x: f(x) < a \right\} \right) = 0 \right\}.$$
%
For each $r > 0$, we can define $f_r(x) := P_{\cX}\left( B(x, r) \right)$ so that $f_r$ is measurable. Because $P_{\cX}$ is a probability measure, $0 \leq f_r(x) \leq 1$ for all $x \in \cX$ and hence $\phi(r) := \ess \inf_{x \in \cX} f_r(x)$ is well-defined and takes value in $[0,1]$.

The function $\msr{\cdot}$ behaves as an underestimator of the cumulative distribution function of $\prx$, and it always exists under our assumptions that $\cX$ is compact (see Appendix \ref{sec:aux_phi} for a proof of its existence). It is used to ensure that for any $u \in [m]$, with high probability, there exists another row $v \in \rowbase$ such that $d_{\cX}(x_1(v), x_1(v))$ is small, implied by the Lipschitz condition that we can use the values of row $v$ to approximate the values of row $u$ well.

% For example, if $\prx$ is a uniform distribution over a unit cube in $d$ dimensional Euclidean space, then $\phi(r) = \min\left\{1,\left(\frac{r}{2} \right)^d\right\}$. On the other hand, if $\prx$ is supported over finitely many points, then $\phi(r) = \min_{\bx \in \text{supp}(\prx)} \prx(\bx)$ is a positive constant, and the role of the latent dimension becomes irrelevant. Intuitively, the ``geometry'' of $\prx$ through $\phi$ near 0 determines the impact of the latent space dimension on the sample complexity, and our results hold as long as the latent dimension $d = o(\log m)$. This sufficient condition is a restatement of the aforementioned one $m \geq (L^2/\rho)^{d/2\delta}$ in terms of $d$, that is to say, $d \leq \frac{2 \delta}{ \log \left(L^2/\rho \right)} \log m$.

%\begin{lem}\label{lem:regularity}
	%Conditioned on $\Ea, \Ec$, the following bound holds for any $k < N^0 q^0$ and any $\zeta \geq \rho$:
	%\[	\Prob{\Ed^c | \Ea, \Ec} \leq \exp \left[ -\frac{N^0 q^0}{2} \left( 1 - \frac{k}{N^0 q^0} \right)^2 \right],	\]
	%where $N^0 = \frac{1}{2}(m-1)p$ and $q^0 = \msr{ \sqrt{\frac{\zeta - \rho}{L^2}} }$.
%\end{lem}

\begin{proof}[Proof of Lemma  \ref{lem:regularity}]
Define the random variable $Y_{uv} = \Ind(\siguv^2 \leq \zeta)$. Then the following two events are equivalent.

\[\left\{\sum_{v \in \cS_u^{\beta}(i)} Y_{uv} < k \right\} \equiv 
\left\{ \left\{\siguv^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)} > \zeta \right\}.\]
Observe that $\sum_{v \in \cS_u^{\beta}(i)} Y_{uv}$ is simply a Binomial random variable with parameters $\left|\cS_u^{\beta}(i)\right|$ and $\bP\left(\siguv^2 \leq \zeta\right)$.
By the Lipschitz property of $f$, for any $a,b \in \cX_1$, and $y \in \cY$, 
\begin{align}
| f(a, y) - f(b, y) | & \leq L d_{\cX_1}(a, b).
\end{align}
Therefore, it follows that  
\begin{align}
\sigma_{ab}^2 &=\Var[f(a,\by) - f(b,\by)] \nonumber\\
&\leq \E[(f(a,\by) - f(b,\by))^2]  \nonumber \\
&\leq L^2 d_{\cX_1}(a,b)^2. \label{eq:sigma_unif_bound}
\end{align}
From \eqref{eq:sigma_unif_bound}, it follows that $d_{\cX_1}(a,b) \leq \sqrt{\zeta/L^2}$ is a sufficient condition to ensure $\sigma_{ab}^2 < \zeta$. Therefore, using the definition of $\phi_1(\cdot)$, it follows that 
\begin{align*}
\bP\left(\siguv^2 \leq \zeta\right) & \geq \bP\left(d_{\cX_1}(x_1(u), x_1(v)) \leq \sqrt{\frac{\zeta}{L^2}}\right) \nonumber \\
& \geq \msra{\sqrt{\frac{\zeta}{L^2}}}. 
\end{align*}
Since we have also conditioned on the fact that $|\cS_u^{\beta}(i)| \geq \frac{1}{2}(m-1)p$, if $U$ is a Binomial random variable with parameters $\frac{1}{2}(m-1)p$ and $\msra{\sqrt{\frac{\zeta}{L^2}}}$, then $\sum_{v \in \cS_u^{\beta}(i)} Y_{uv}$ dominates $U$, in the sense that
\[\bP\left(\sum_{v \in \cS_u^{\beta}(i)} Y_{uv} < k\right) \leq \bP(U < k).\]
We let $\nthresh$ denote the expectation of $U$, i.e., $\nthresh := \Exp{U} = \frac{1}{2}(m-1)p \msra{\sqrt{\frac{\zeta}{L^2}}}$. Then it follows from Chernoff's bound for the lower tail that 
\[\bP(U < k) \leq \exp\left(-\frac{(\nthresh - k )^2}{2\nthresh}\right) .\]
Therefore, 
\begin{align*}
&\Prob{\left. \left\{\siguv^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)} > \zeta ~\right|~  |\cS_u^{\beta}(i)| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] }  \\
&\qquad\leq  \exp\left(-\frac{(\nthresh - k )^2}{2\nthresh}\right) .
\end{align*}
\end{proof}





\subsubsection{Bound on tail probability of error conditioned on good events} Conditioned on the above events that the overlaps are sufficiently large, mean and variance concentrate, and there are sufficiently many good nearest neighbors, we can upper bound the estimation error using Chebyshev's inequality.

\begin{proof}[Proof of Lemma  \ref{lem:estimate}]
Recall that $\rowbasek$ denotes the set of the $k$ best row indices $v$ in $\rowbase$ which have minimum sample variance $\suv^2$. We are interested in the probabilistic tail bound of the error $Err^k(u,i)$, which can be expressed as
\begin{align*}
&Err^k(u,i) \triangleq A(u,i) - \hat{A}^k(u,i) \\
&\qquad= \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} (A(u,i) - \hat{A}_v(u,i))\\
&\qquad= \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left(A(u,i) -Z(v,i) - \muv \right)\\
&\qquad= \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( \left( A(u,i) - A(v,i) - \eta(v,i) - \muuv \right) \right)\\
& \qquad \qquad -  \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( \left( \muv - \muuv\right) \right) \\
\end{align*}
Its absolute value can be bounded by
\begin{align*}
&\left| A(u,i) - \hat{A}^k(u,i) \right| \\
& \qquad	\leq  \left| \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuv \right) \right|\\
	&\qquad\qquad + \left| \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( \muv - \muuv \right) \right|  \\
\end{align*}

By the same argument as in the proof of Lemma  \ref{lem:overlap}, $\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps$ implies either 
	\begin{equation}\label{eq:event1}
		\left| \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuv \right) \right|  > \eps - \eps_1	
	\end{equation}
or
	\begin{equation}\label{eq:event2}
		\left| \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek}  \muv - \muuv\right| > \eps_1
	\end{equation}
for any choice of $\eps_1$. Recall the definitions of events $\Ea, \Eb, \Ec, \Ed$ from the statement of Lemma \ref{lem:estimate}. Conditioned on $\Eb$, $\left|\muuv - m_{uv}\right| \leq \mslack, ~\forall~ v \in \cS_u^{\beta}(i)$, the second event \eqref{eq:event2} never happens for $\eps_1 \geq \mslack$. By choosing $\eps_1 = \mslack$, it follows that the error probability conditioned on $\Ea, \Eb, \Ec$, and $\Ed$  can be bounded by the probability of the first event \eqref{eq:event1}. We denote $E := \Ea \cap \Eb \cap \Ec \cap \Ed$, and we use ``expr'' to denote the left hand expression in \eqref{eq:event1}.
\begin{align} \label{eq:suff_cond}
&\Prob{\left| A(u, i) - \hat{A}^k(u,i) \right| > \eps ~|~ E}\\
&\leq \Prob{\left.\left| \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuv \right) \right| > \eps - \mslack ~\right|~ E}  \nonumber \\
&= \int_{ \vvec{y} \in \cX_1^m} \sum_{\cS_0 \subset [n]: |\cS_0| = k} \Prob{\left.\left| \text{``expr''} \right| > \eps - \mslack ~\right|~ \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E} \nonumber \\
& \qquad \qquad \qquad \qquad \qquad \qquad \Prob{ \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0 ~|~ E} d\vvec{y}. \nonumber
\end{align}
We can verify that the event $E$ and the set $\rowbasek$ do not depend upon any information from column $i$, therefore $\eta(v,i)$ is independent from $E$ for all $v$. For the same reason, $x_2(i)$ is independent from $E$ and $\rowbasek$. Therefore, we can show that each term in the summation $\left( A(u,i) - A(v,i) - \eta(v,i) - \muuv \right)$ has zero mean by definition of $\muuv$. We use $\bx_2$ to denote an independent random variable sampled as per $P_{\cX_2}$.
\begin{align*}
&\E\big[A(u,i) - A(v,i) - \eta(v,i) - \muuv \big|  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E \big] \\
&= \E\big[f(x_1(u),x_2(i)) - f(x_1(v),x_2(i)) \big|  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E \big] - \mu_{y_u y_v} \\
&= \E_{\bx_2}\big[f(y_u,\bx_2) - f(y_v,\bx_2) \big|  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E \big] - \mu_{y_u y_v} \\
&= 0.
\end{align*}
Therefore an application of Chebyshev inequality yields,
\begin{align} \label{eq:cheby_cond}
&\Prob{\left.\left| \text{``expr''}  \right| > \eps - \mslack ~\right|~ \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E}  \\
&\qquad\leq \frac{\Var\left[\left.\frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left( A(u,i) - A(v,i) - \eta(v,i)\right) ~\right|~ \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E\right]}{(\eps - \mslack)^2}. \nonumber
\end{align}
Recall that $\eta(v,i)$ is independent from $E$ and $\rowbasek$ and has variance $\gamma^2$. In addition, $|\rowbasek| = |\cS_0| = k$. Therefore, by independence of the noise term and using Cauchy-Schwarz inequality, it follows that 
\begin{align}
&\Var \left[ \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left(A(u,i) - A(v,i) - \eta(v,i) \right) \Big| \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0,  E\right] \nonumber \\
&= \Var \left[ \frac{1}{k} \sum_{v \in \rowbasek} \left(A(u,i) - A(v,i)\right) \Big| \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E\right] \nonumber \\
&\qquad \qquad + \Var\left[\frac{1}{k} \sum_{v \in \rowbasek} \eta(v,i) \Big| \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E \right]  \nonumber \\
%&= \frac{1}{|S_k|^2} \sum_{v \in S_k} \sum_{v' \in S_k} Cov\left[\left(A_{ui} - A_{vi}\right) \left(A_{ui} - A_{v'i}\right)\right] + \frac{1}{|S_k|^2} \sum_{v \in S_k} \Var[e_{vi}]\\
%&\leq \frac{1}{|S_k|^2} \sum_{v \in S_k} \sum_{v' \in S_k} \sqrt{\Var\left[A_{ui} - A_{vi}\right] \Var\left[A_{ui} - A_{v'i}\right]} + \frac{\gamma^2}{|S_k|} \\
%&= \frac{1}{|S_k|^2} \sum_{v \in S_k} \sum_{v' \in S_k} \sigma_{x_u x_v} \sigma_{x_u x_{v'}} + \frac{\gamma^2}{|S_k|} \\
&\leq \left(\frac{1}{k} \sum_{v \in \cS_0} \sqrt{\Var\left[A(u,i) - A(v,i)  \big|  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right]}\right)^2 + \frac{\gamma^2}{k}. \label{eq:variancechebyshev}
\end{align}
Next we will bound $\Var\left[A(u,i) - A(v,i)  ~\big|~  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right]$ for any $v \in \cS_0$. Recall that the event $E$ and set $\rowbasek$ is completely independent from $x_2(i)$ because the event does not depend on any data from column $i$. Therefore using the independence of $x_2(i)$, if we let $\bx_2$ denote a random variable which is sampled independently from $P_{\cX_2}$, then
\begin{align*}
&\Var\left[A(u,i) - A(v,i)  ~\big|~  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right] \\
&= \Var\left[f(x_1(u),x_2(i)) - f(x_1(v),x_2(i))  ~\big|~  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right] \\
&= \Var\left[ f(y_u, \bx_2) - f(y_v,\bx_2)  ~\big|~  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right] \\
&= \sigma^2_{y_u y_v}.
\end{align*}
Let $\tilde{\cV}$ denote the subset of rows $v \in \cS_u^{\beta}(i)$ such that $\siguv^2 \leq \zeta$. Conditioned on $\Ed$, the size of set $\tilde{\cV}$ must be at least $k$. Conditioned on $\Ec$, for every $v \in \tilde{\cV} \subset \cS_u^{\beta}(i)$, 
\[\suv^2 \leq \left(\siguv^2 + 2 \gamma^2 \right) + \vslack \leq \zeta + 2 \gamma^2 + \vslack. \]
Therefore, it follows by the definition of $\rowbasek$ as the set of $k$ rows with minimum sample variance, that for all $v \in \rowbasek$, $\suv^2 \leq \zeta + \vslack + 2 \gamma^2$. Due to event $\Ec$ and $\rowbasek = \cS_0$, this implies that for all $v \in \cS_0$, $\siguv^2 \leq \left( s_{uv}^2 + \vslack \right) - 2 \gamma^2 \leq \zeta + 2\vslack$. Therefore for all  $v \in \cS_0$, 
\begin{align*}
\Var\left[A(u,i) - A(v,i)  ~\big|~  \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E  \right] \leq \zeta + 2\vslack.
\end{align*}


Finally we can plug the variance bound into \eqref{eq:variancechebyshev} and \eqref{eq:cheby_cond} to show that
\begin{align*}
&\Prob{\left.\left| \text{``expr''} \right| > \eps - \mslack ~\right|~ \left(x_1(v)\right)_{v \in [m]} = \vvec{y}, \rowbasek = \cS_0, E}  \\
&\qquad\leq \frac{1}{(\eps - \mslack)^2}\left(\left(\frac{1}{k} \sum_{v \in \cS_0} \sqrt{\zeta + 2\vslack}\right)^2 + \frac{\gamma^2}{k}\right) \\
&\qquad\leq \frac{1}{(\eps - \mslack)^2}\left(\zeta + 2\vslack + \frac{\gamma^2}{k}\right). 
\end{align*}

Since this above bound does not depend on the particular choice of $\vvec{y}$ and $\cS_0$, by plugging into \eqref{eq:suff_cond}, it follows that 
\begin{align}
&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps ~|~ E} \\
&\leq \frac{1}{(\eps - \mslack)^2} \left(\zeta + 2\vslack + \frac{\gamma^2}{k} \right).
\end{align}

\end{proof}


==> contents/matrix_proof/proofsketch.tex <==
The proof of the main results corresponds to showing that the estimates associated to the $k$-nearest neighbors selected by the algorithm are indeed close to the true target value. Theorem \ref{thm:main_tail} provides such a probabilistic tail bound for each $(u,i)$, and integrating this leads to the conclusion of Theorem \ref{thm:main_theorem}.

\subsection{Proof Outline}
For any fixed row latent features $a,b \in \cX_1$, and randomly sampled column latent feature variable $\bx_2 \sim P_{\cX_2}$, we denote the mean and variance of the difference $f(a,\bx_2) - f(b,\bx_2)$ with respect to $\bx_2$ according to
\begin{align*}
\mu_{ab} &\triangleq \E_{\bx_2}[f(a,\bx_2) - f(b,\bx_2)] = \E[m_{u v} | \bx_1(u) = a,\bx_1(v) = b],\\
\sigma_{ab}^2 &\triangleq \Var_{\bx_2}[f(a,\bx_2) - f(b,\bx_2)] = \E[s_{uv}^2 | \bx_1(u)=a, \bx_1(v) =b] - 2 \gamma^2.
\end{align*}
This is also equivalent to the expectation of the empirical means and variances computed by the algorithm when we condition on the latent representations of the users. The computation of $\hat{A}_{ui}$ involves two steps: first the algorithm determines the $k$ rows in $\cS_u^{\beta}(i)$ with minimum sample variance, and then it computes the estimate by averaging over the $k$ rows, adjusting each according to the empirical row mean.

The proof involves three key steps, each stated within a lemma. We first prove that every pair of rows has sufficient overlap with high probability. Specifically, Lemma \ref{lem:overlap} proves that for any $(u,i)$, the number of the candidate rows, $|\rowbase|$, concentrates around $(m-1)p$. This relies on concentration of Binomial random variables via Chernoff's bound, using the fact that every entry is independently observed uniformly at random.

    \begin{lem}\label{lem:overlap} Given $p > 0$, $2 \leq \beta < np^2$, and $\theta \in (0, 1)$, for any $(u,i) \in [m] \times [n]$, %***TODO \dogyoon{we may need to use a different letter than $\alpha$ here}
    	\begin{align*}
	    &\Prob{|\rowbase - (m-1)p | > \theta (m-1)p}\\
%	    &\Prob{|\rowbase| \notin (1 \pm \theta) (m-1)p}\\
	    &\qquad		\leq (m-1) \exp \left( - \frac{\left(np^2-\beta\right)^2}{2np^2} \right) + 2 \exp \left( - \frac{\theta^2}{3}(m-1)p \right).
	\end{align*}
    \end{lem}


Next, assuming the overlap between two rows $u$ and $v$ is sufficiently large, Lemmas \ref{lem:mean} and \ref{lem:variance} prove that the sample mean and variance of the difference $Z(u,i) - Z(v,i)$ , denoted by $\muv$ and $\suv^2$ and defined in \eqref{eq:row_mean} and \eqref{eq:row_var} of Section \ref{sec:uu-kNN_alg}, concentrate around their expectations $\muuv$ and $\siguv^2$ with high probability. Recall that $B_0 = L \diamxa + 2 B_e$, defined in \eqref{eq:def_B0}, uniformly upper bounds $\left| Z(u,i) - Z(v,i) \right|$ for any $u,v \in [m]$ and $i \in [n]$, due to the properties that $f$ is Lipschitz, $\cX_1$ is compact, and the noise terms are bounded by $B_e$. We will use the Bernstein and Maurer-Pontil inequalities along with the boundedness of the variables to show the following concentration results for the mean and variance.

\begin{lem}\label{lem:mean}
        Given $u \in [m], i \in [n]$, and $\beta \geq 2$, for any $\mslack > 0$, 
        \[	\Prob{\left|\muuv - \muv \right| > \mslack \left| v \in \rowbase \right.} \leq \exp \left( -\frac{3\beta \mslack^2}{6B_0^2 + 4 B_0 \mslack} \right).	\]
%        where $B_0 = \sup \left| z_{ui} - z_{vi} \right| \leq \min \left\{2, L\diamx + 2 B_e \right\}$.
    \end{lem}
    
    \begin{lem}\label{lem:variance}
        Given $u \in [m], i \in [n]$, and $\beta \geq 2$, for any $\vslack > 0$,
        \[	\Prob{\left| \suv^2 - \left( \siguv^2 + 2\gamma^2 \right) \right| > \vslack \left| v \in \rowbase \right.} \leq 2 \exp\left(-\frac{\beta \vslack^2}{8 B_0^2 (2 B_0^2 + \vslack)}\right).	\]
%        where $B_0 = \sup \left| z_{ui} - z_{vi} \right| \leq \min \left\{2, L\diamx + 2 B_e \right\}$.
    \end{lem}


Next, Lemma \ref{lem:regularity} proves that since the latent features are sampled iid from a bounded metric space, for any index pair $(u,i)$, there exists $k$ ``good'' neighboring rows in $\cS_u^{\beta}(i)$, whose $\sigma_{x_1(u) x_1(v)}^2$ is sufficiently small. Let $\left\{\sigma_{x_1(u) x_1(v)}^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)}$ denote the value of the $k$-th minimum element in the set $\left\{\sigma_{x_1(u) x_1(v)}^2\right\}_{v \in \cS_u^{\beta}(i)}$.

    \begin{lem}\label{lem:regularity}
		Given $u \in [m]$, $i \in [n]$, for any $\zeta > 0$ and for any integer $k \in (0, \nthresh]$,
        \begin{align*}	
				&\Prob{\left. \left\{\sigma_{x_1(u) x_1(v)}^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)} > \zeta ~\right|~  |\cS_u^{\beta}(i)| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] } \\
				&\qquad	\leq  \exp\left(-\frac{(\nthresh - k )^2}{2\nthresh}\right) ,	
				\end{align*}
        where $\nthresh = \frac{1}{2}(m-1)p \msra{\sqrt{\frac{\zeta}{L^2}}}$ and $\msra{r} := \ess \inf_{x' \in \cX_1} \prxa \left(d_{\cX_1}(\bx, x') \leq r\right)$.
    \end{lem}
		
		
Given that there exist $k$ good neighbors in $\cS_u^{\beta}(i)$ whose variance is small, and conditioned on the event that all the sample variances concentrate, it follows that the true variance between $u$ and its $k$ nearest neighbors are small with high probability. Therefore, we can provide a bound on the tail probability of the estimation error conditioned on these good events by using Chebyshev's inequality.
\begin{lem}\label{lem:estimate}
Given $\mslack > 0$, $\vslack > 0$, for any $\eps > \mslack$, $\zeta \geq 0$ and any integer $k \in (0, \nthresh]$, the estimate produced by the user-user $k$-nearest neighbor with overlap parameter $\beta$ satisfies
\[\Prob{\left. \left| A(u,i) - \hat{A}^k(u,i) \right| > \eps ~\right|~ E } \leq \frac{1}{(\eps - \mslack)^2} \left(\zeta + 2\vslack + \frac{\gamma^2}{k} \right),\]
where the events $E, \Ea, \Eb, \Ec$ and $\Ed$ are defined as follows
\begin{align*}
E &:= \Ea \cap \Eb \cap \Ec \cap \Ed, \\
\Ea &:= \left\{|\cS_u^{\beta}(i)| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right]\right\}, \\
\Eb &:= \left\{\left|\mu_{x_1(u) x_1(v)} - m_{uv}\right| \leq \mslack, ~\forall~ v \in \cS_u^{\beta}(i) \right\}, \\
\Ec &:= \left\{\left|s_{uv}^2 - (\sigma_{x_1(u) x_1(v)}^2 + 2 \gamma^2)\right| \leq \vslack, ~\forall~ v \in \cS_u^{\beta}(i) \right\}, \\
\Ed &:= \left\{\left\{\sigma_{x_1(u) x_1(v)}^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)} \leq \zeta \right\}.
%\Ed &:= \left\{(s_{uv}^2)^{(k)} \leq \zeta + 2 \gamma^2 \right\}.
\end{align*}
\end{lem} 

Finally we combine the lemmas which bound each of the deviating events to obtain a bound on the tail probability of the error. 
    \begin{thm}\label{thm:main_tail} Suppose that
        \begin{align*}
		&p \geq \max \left\{ m^{-1 + \delta}, n^{-\frac{1}{2} + \delta} \right\} \text{ for some } \delta > 0,\\
		&\zeta \text{ satisfies } \msra{\sqrt{\frac{\zeta}{L^2}}}\geq c_{\phi} \left(mp \right)^{-2/3} \text{ for some } c_{\phi} \geq 0,\\
		&2 \leq \beta \leq c np^2 \text{for some }c \in (0, 1),\text{ and}\\
		&k \leq \frac{c_k}{2}(m-1)p \msra{\sqrt{\frac{\zeta}{L^2}}}\text{ for some }c_k \in [0,1).
	\end{align*}
	For any $\eps > \left( np^2 \right)^{-1/3}$, the tail probability of the error of the estimate produced by the user-user $k$-nearest neighbor algorithm with overlap parameter $\beta$ is upper bounded by:
     \begin{align*}
	&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps} \\
	&\qquad \leq  \frac{1}{\left(\eps - \beta^{-1/3}\right)^2} \left(\zeta + 2\beta^{-1/3} + \frac{\gamma^2}{k} \right)\\
	&\qquad\qquad	+ 3 \exp \left( - c_1 \left( mp \right)^{1/3} \right) + \left( m + \frac{9}{2}mp \right) \exp\left( - c_2 \beta^{1/3} \right),
    \end{align*}
    where
        $ c_1 := \min \left\{ \frac{1}{24}, \frac{c_{\phi}\left( 1 - c_k \right)^2}{8} \right\}$ and $c_2 := \min \left\{ \frac{c^2}{2}, \frac{3}{6B_0^2 + 4 B_0 }, \frac{1}{8 B_0^2 \left(2B_0 ^2 + 1 \right)}  \right\}$
    are absolute constants, which depend only on the geometry of the latent spaces.
    \end{thm}
Note that we can obtain a similar theorem for the item-item $k$-nearest neighbor variant by exchanging $m$ and $n$ in Theorem \ref{thm:main_tail}. 
Given an upper bound on the tail of the error probability, we can prove an upper bound on the MSE by integrating the tail bound. The results for the user-user variant is stated in the final Theorem \ref{thm:main_theorem}. Corresponding results for the item-item variant is stated in Theorem \ref{thm:main_theorem_item}, which follows from taking the transpose of the matrix and simply exchanging $m$ and $n$.


==> contents/matrix_proof/thmproof.tex <==
\subsection{Proof of Error Probability Tail Bounds (Theorem \ref{thm:main_tail})}
Lemmas \ref{lem:overlap}, \ref{lem:mean}, \ref{lem:variance}, and \ref{lem:regularity} provide probability bounds on the following events defined in Lemma \ref{lem:estimate}: 
\begin{align*}
\Ea &:= \left\{|\cS_u^{\beta}(i)| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right]\right\}, \\
\Eb &:= \left\{\left|\muuv - m_{uv}\right| \leq \mslack, ~\forall~ v \in \cS_u^{\beta}(i) \right\}, \\
\Ec &:= \left\{\left|s_{uv}^2 - (\siguv^2 + 2 \gamma^2)\right| \leq \vslack, ~\forall~ v \in \cS_u^{\beta}(i) \right\}, \\
\Ed &:= \left\{\left\{\siguv^2\right\}_{v \in \cS_u^{\beta}(i)}^{(k)} \leq \zeta \right\}.
%\Ed &:= \left\{(s_{uv}^2)^{(k)} \leq \zeta + 2 \gamma^2 \right\}.
\end{align*}
Lemma \ref{lem:estimate} provides a bound on the tail of the probability of error conditioned on the events $\Ea, \Eb, \Ec, \Ed$. Theorem \ref{thm:main_tail} simply combines the lemmas with the proper conditioning to prove an upper bound on the tail of the error probability.

\begin{proof}
	First of all, note that the error probability can be decomposed into bounding the probability of violating each event, according to
	\begin{align*}
			&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}	\\
			&= \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea \cap \Eb \cap \Ec \cap \Ed} \Prob{\Ea \cap \Eb \cap \Ec \cap \Ed} \\
			& \quad + \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea^c \cup \Eb^c \cup \Ec^c \cup \Ed^c} \Prob{\Ea^c \cup \Eb^c \cup \Ec^c \cup \Ed^c} \\
			&\leq \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea \cap \Eb \cap \Ec \cap \Ed} \\
			& \quad + \Prob{\Ea^c \cup \Eb^c \cup \Ec^c \cup \Ed^c} \\
%			&\leq \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea \cap \Eb \cap \Ec \cap \Ed} \\
%			& \quad + \Prob{\Ea^c} \Prob{ \Ea^c \cup \Eb^c \cup \Ec^c \cup \Ed^c | \Ea^c } + \Prob{\Ea} \Prob{ \Ea^c \cup \Eb^c \cup \Ec^c \cup \Ed^c | \Ea } \\
%			&\leq \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea \cap \Eb \cap \Ec \cap \Ed} \\
%			& \quad + \Prob{\Ea^c} + \Prob{ \Eb^c \cup \Ec^c \cup \Ed^c | \Ea } \\
			&\leq \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea \cap \Eb \cap \Ec \cap \Ed} \\
			& \quad + \Prob{\Ea^c} + \Prob{ \Eb^c  | \Ea} + \Prob{\Ec^c | \Ea} + \Prob{\Ed^c | \Ea }.
	\end{align*}
	The first inequality uses the fact that probabilities cannot exceed $1$. The last inequality is derived from the additivity of the measure $\bP$ and the union bound. Because $A \cup B = A \cup \left( B \cap A^c \right)$,
	\begin{align*}
	    \Prob{ A \cup B } &= \Prob{A } + \Prob{ B \cap A^c }\\
	    	& = \Prob{A } + \Prob{ \left. B \right| A^c }\Prob{A^c}\\
		&\leq \Prob{A } + \Prob{ \left. B \right| A^c } \qquad \because \Prob{A^c} \leq 1. 	
	\end{align*}
	Then we can obtain the last inequality by applying the union bound after taking $A = \Ea^c$ and $B = \Eb^c \cup \Ec^c \cup \Ed^c$.
	By Lemma \ref{lem:estimate},
	\begin{align*}
			\Prob{\left. \left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| \Ea, \Eb, \Ec, \Ed}	&\leq \frac{1}{(\eps - \mslack)^2} \left(\zeta + 2\vslack + \frac{\gamma^2}{k} \right).
	\end{align*}
	Using Lemma \ref{lem:overlap}, we have
\begin{align*}
		\Prob{\Ea^c}	&= \Prob{|\rowbase| \not\in \left[ \frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p \right]}\\
&\leq (m-1) \exp \left( -\frac{\left(np^2-\beta\right)^2}{2np^2} \right) + 2 \exp \left( -\frac{(m-1)p}{12} \right) .
\end{align*}
Similarly, by using Lemma \ref{lem:mean} with union bound,
\begin{align*}
		\Prob{\Eb^c | \Ea} &= \Prob{\bigcup_{v \in \rowbase} \left\{ |\muuv - \muv| > \mslack \right\}}\\
&\leq \frac{3}{2}(m-1)p \exp \left( -\frac{3\beta \mslack^2}{6B_0^2 + 4B_0\mslack} \right),
\end{align*}
where we recall that $B_0 = L \diamxa + 2B_e$. 
By using Lemma \ref{lem:variance} with union bound again,
\begin{align*}
	\Prob{\Ec^c | \Ea} &= \Prob{\bigcup_{v \in \rowbase} \left\{ \left| \suv^2 - \left( \siguv^2 + 2\gamma_{ui}^2 \right) \right| > \vslack \right\}}\\
&\leq 3 (m-1)p \exp \left( - \frac{\beta \vslack^2}{ 8B_0^2 \left( 2B_0^2 + \vslack \right)} \right).
\end{align*}
By Lemma \ref{lem:regularity} with $N_0 := \frac{1}{2}(m-1)p \msra{\sqrt{\frac{\zeta}{L^2}}}$ as previously defined,
\begin{align*}
	\Prob{\Ed^c | \Ea} &\leq \exp \left( -\frac{(\nthresh - k)^2 }{2 \nthresh} \right).
\end{align*}
Putting everything together, we obtain the following inequality,
\begin{align}
&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}		\nonumber\\
&	\leq  \frac{1}{(\eps - \mslack)^2} \left(\zeta + 2\vslack + \frac{\gamma^2}{k} \right)	\nonumber\\
&\qquad	+ (m-1) \exp \left( -\frac{\left(np^2-\beta\right)^2}{2np^2}\right) + 2 \exp \left( - \frac{(m-1)p}{12}\right) 			\label{eq:expterm1}\\
&\qquad	+ \frac{3}{2}(m-1)p \exp \left( -\frac{3 \beta \mslack^2}{6B_0^2 + 4 B_0 \mslack} \right)	\label{eq:expterm2} \\
&\qquad	+ 3(m-1)p \exp \left( -\frac{\beta \vslack^2}{8 B_0^2 \left(2B_0 ^2 + \vslack \right)} \right)	\label{eq:expterm3}\\
&\qquad	+ \exp \left( -\frac{\left( \nthresh - k \right)^2}{2 \nthresh} \right).						\label{eq:expterm4}
\end{align}
Note that $\zeta, \mslack, \vslack$ are parameters which are introduced purely for the purpose of analysis. Requiring all exponential terms decay to $0$ as $m, n \to \infty$ restricts the range of values $\zeta, \mslack, \vslack$ can take. We will let $\mslack = \vslack = \beta^{-1/3}$. Also, we enforce $\zeta$ satisfies $\msra{\sqrt{\frac{\zeta}{L^2}}}\geq c_{\phi}\left( mp \right)^{-2/3}$ so that $\nthresh \geq \frac{c_{\phi}}{4}\left( mp \right)^{1/3}$ as described in the theorem statement. Additionally, we require $\beta \to \infty$ as $m, n \to \infty$ and $np^2 - \beta \geq c np^2$ for some $c > 0$. We will show these are sufficient conditions for the convergence of exponential error terms.

Given a sequence of problems of size $(m,n)$, suppose that $p = \omega(m^{-1})$ and $p = \omega(n^{-1/2})$. Then $mp, np^2 \to \infty$ as $m, n \to \infty$. We may assume without loss of generality that $m$ and $n$ are large enough such that $mp, np^2, \beta \geq 2$ for simplicity. 

Assuming $\beta \to \infty$ as $m,n \to \infty$, we can observe that $\mslack, \vslack \to 0$ as $m, n \to \infty$. In addition, we have $\mslack \leq 1$, $\vslack \leq 1$, since we assumed $\beta \geq 2$ (hence, $\geq 1$). Therefore, the exponential terms Eq. \eqref{eq:expterm2} and Eq. \eqref{eq:expterm3} reduce as follows:
\begin{align*}
	\frac{3}{2}(m-1)p \exp \left( -\frac{3 \beta \mslack^2}{6B_0^2 + 4 B_0 \mslack} \right)	&\leq	\frac{3}{2}(m-1)p \exp \left( -\frac{3}{6B_0^2 + 4 B_0} \beta^{1/3}\right),	\\
	3(m-1)p \exp \left( -\frac{\beta \vslack^2}{8 B_0^2 \left(2B_0 ^2 + \vslack \right)} \right)	&\leq	3(m-1)p \exp \left( -\frac{1}{8 B_0^2 \left(2B_0 ^2 + 1 \right)} \beta^{1/3} \right).
\end{align*}
In the theorem statement, we assumed that $k \leq c_k \nthresh$ for some $c_k \in (0, 1)$, and the constraints on the parameter $\zeta$, which depend on the latent geometry via $\phi_1$, allow us to reduce the last exponential error term Eq. \eqref{eq:expterm4} to the following bound:
\[	\exp \left( -\frac{\left( \nthresh - k \right)^2}{2 \nthresh} \right) \leq \exp\left( - \frac{c_{\phi}\left( 1 - c_k \right)^2}{8} \left(mp \right)^{1/3} \right).	\]
From the assumption $np^2 - \beta \geq c np^2$ for some $c \in (0,1)$, it follows that $-\frac{\left(np^2-\beta\right)^2}{2np^2} \leq - \frac{c^2}{2}np^2$. Since we assumed $\beta < np^2$,
$$	(m-1) \exp \left( -\frac{\left(np^2-\beta\right)^2}{2np^2}\right) \leq (m-1) \exp \left( -\frac{c^2}{2} np^2\right) \leq (m-1) \exp \left( -\frac{c^2}{2} \beta\right).	$$
Finally, we can obtain the following upper bound on Eq. \eqref{eq:expterm1} using our assumption that $\beta > 1$ and $mp \geq 2$:
\begin{align*}
	&(m-1) \exp \left( -\frac{\left(np^2-\beta\right)^2}{2np^2}\right) + 2 \exp \left( - \frac{(m-1)p}{12}\right) \\
	&\qquad\leq  (m-1) \exp \left( -\frac{c^2}{2}\beta^{1/3}\right) + 2 \exp \left( - \frac{1}{24}\left(mp\right)^{1/3}\right). 
\end{align*}
By substituting in the above inequalities, the error probability bound reduces to
\begin{align*}
&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}\\
&	\leq  \frac{1}{\left(\eps - \beta^{-1/3} \right)^2} \left(\zeta + 2\beta^{-1/3} + \frac{\gamma^2}{k} \right)\\
&\qquad	+ 3 \exp \left( - c_1 \left( mp \right)^{1/3} \right) + \left( m + \frac{9}{2}mp \right) \exp\left( - c_2 \beta^{1/3} \right)
\end{align*}
where
$ c_1 := \min \left\{ \frac{1}{24}, \frac{c_{\phi}\left( 1 - c_k \right)^2}{8} \right\}$ and $c_2 := \min \left\{ \frac{c^2}{2}, \frac{3}{6B_0^2 + 4 B_0 }, \frac{1}{8 B_0^2 \left(2B_0 ^2 + 1 \right)}  \right\}$
are absolute constants, which may depend only on the geometry of the latent spaces.

%In order for the last term to converge to zero, we need that $np^2 \rho^2$ goes to infinity, so we enforce the looser condition that $\rho = \Omega((np^2)^{-1/3})$. In order for the second to last term to converge, we need $mp \msr{\sqrt{\frac{\zeta - \rho}{L^2}}}$ to go to infinity, so we enforce the looser condition that $\msr{\sqrt{\frac{\zeta - \rho}{L^2}}} = \Omega((mp)^{-2/3})$. Therefore, the exponential error terms are asymptotically dominated by $\exp \left( - \frac{(mp)^{1/3}}{16}\right)$ and $mp \exp \left( -c_1 (np^2)^{1/3}\right)$ for $c_2 = \min\left(\frac{3\cdot 2^{2/3}}{12B_0^2}, \frac{1}{8 B_0^2 \left(2B_0 + 4\gamma^2\right)}\right)$.
	
%Since $0 \leq \msr{\cdot} \leq 1$, it is clear that $-\frac{1}{24}m^{\delta} \leq -\frac{1}{32}\msr{\sqrt{\frac{\zeta - \rho}{L^2}}}m^{\delta}$. Next, $2 \exp \left( -\frac{1}{24}m^{\delta}\right) + m \exp \left( -\frac{1}{8} m^{2\delta}\right) \geq m \exp \left( -\frac{1}{8} m^{2\delta}\right)$ if $-\frac{1}{24}m^{\delta} \geq -\frac{1}{8} m^{2\delta} + \log \frac{m}{2}$. With substituting $X := m^{\delta}$, this condition is equivalent to $3 X^2 - X \geq \frac{1}{\delta} \log X - \log 2$, which holds as $m \geq M(\delta)$. Also, we can observe that this inequality holds as $X \to 0$. Hence, we can conclude from continuity that $m \exp \left( -\frac{1}{8} m^{2\delta}\right) \leq C(\delta) \exp \left( -\frac{1}{24}m^{\delta}\right)$ for some constant which depends only on $\delta$.

%Also, assuming $\rho = \Omega\left(n^{-\frac{2}{3}\delta}\right)$, two exponential terms with $n^{\delta}$ is guaranteed to be in the class $O\left(m^{\delta} \exp\left(-c n^{\frac{2}{3}\delta}\right)\right) = O\left(\exp\left(-c n^{\frac{2}{3}\delta} + \delta \log m\right)\right) = O\left(\exp\left(-c' n^{\frac{2}{3}\delta}\right)\right)$ as long as the matrix is neither too thin nor too fat, i.e., $m = n^{\theta}$ for some $\theta \in (0, \infty)$.

%To summarize, we can conclude that
%\begin{align*}
%&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}	\leq \frac{1}{(\eps - 2^{1/3} (np^2)^{-1/3})^2} \left(\zeta + \rho + \frac{4\gamma^2}{(m-1)p} \msr{\sqrt{\frac{\zeta - \rho}{L^2}}}^{-1} \right)\\
%&\qquad\qquad + C_1 \exp \left( - \frac{(mp)^{1/3}}{16}\right) + C_2 mp \exp \left( -c_2 (np^2)^{1/3}\right),
%\end{align*}
%where $c_2 = \min\left(\frac{3\cdot 2^{2/3}}{12B_0^2}, \frac{1}{8 B_0^2 \left(2B_0 + 4\gamma^2\right)}\right)$, and $C_1, C_2$ are some constants depending on $\delta$.
\end{proof}


\subsection{Proof of Main Result for Matrix Estimation (Theorem \ref{thm:main_theorem})} 
Given the error probability bound in Theorem \ref{thm:main_tail}, we integrate the probability to provide a bound on the mean squared error.

\begin{proof}
For a fixed $(u,i)$, 
\begin{align*}
&Err^k(u,i) \triangleq A(u,i) - \hat{A}^k(u,i) \\
&\qquad= \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} (A(u,i) - \hat{A}_v(u,i))\\
&\qquad= \frac{1}{|\rowbasek|} \sum_{v \in \rowbasek} \left(A(u,i) -Z(v,i) - \muv \right).
\end{align*}
By our model assumptions and the definition of $B_0$, it follows that $|m_{uv}| \leq B_0$, and $|A(u,i) - Z(v,i)| \leq L\diamxa + B_e \leq B_0$. Therefore $|Err^k(u,i)| \leq 2 B_0$. Since $Err^k(u,i)^2 \geq 0$, the mean squared error can be written as the following integral:
\begin{align*}
MSE(\hat{A}^k) &:= \frac{1}{mn} \sum_{u,i} \Exp{ Err^k(u,i)^2} 	\\
 &= \frac{1}{mn} \sum_{u,i} \int_0^{\infty} \Prob{Err^k(u,i)^2 \geq t} dt\\
	&= \frac{1}{mn} \sum_{u,i}\int_0^{\infty} \Prob{Err^k(u,i) \geq \sqrt{t}} dt\\
	&= \frac{1}{mn} \sum_{u,i} \int_0^{4B_0^2} \Prob{Err^k(u,i) \geq \sqrt{t}} dt.
\end{align*}

A probability cannot exceed 1, hence it follows from Theorem \ref{thm:main_tail} that for all $(u,i)$,
\[	\Prob{Err^k(u,i) \geq \sqrt{t}} \leq \left[ \frac{\Fa}{(t^{1/2} - \Fb)^2} + \Fc \right] \wedge 1,	\]
where $\Fa = \zeta + 2\beta^{-1/3} + \frac{\gamma^2}{k}$, $\Fb = \beta^{-1/3}$, and $\Fc = 3 \exp \left( - c_1 \left( mp \right)^{1/3} \right) + \left( m + \frac{9}{2}mp \right) \exp\left( - c_2 \beta^{1/3} \right)	$, with the parameters $\zeta, k, \beta$ and constants $c_1, c_2$ as described in the theorem statement.

Since the function $\frac{\Fa}{(t^{1/2} - \Fb)^2} + \Fc$ is monotone decreasing for $t > \Fb^2$, for any partitioning parameter $t^* > \Fb^2$, it follows that
	\begin{align*}
MSE(\hat{A}^k) 	&\leq \int_0^{t^*} 1 dt + \int_{t^*}^{4B_0^2} \left( \frac{\Fa}{(t^{1/2} - \Fb)^2} + \Fc \right) dt \\
&= t^* + 2\Fa \left.\left( - \frac{\Fb}{t^{1/2} - \Fb} + \ln(t^{1/2} - \Fb) \right)\right|_{t^*}^{4B_0^2} + \Fc (4B_0^2 - t^*) \\
&= t^* - \frac{2 \Fa \Fb}{2B_0 - \Fb} + 2 \Fa \ln(2B_0 - \Fb) \\
&~~~~+ \frac{2 \Fa \Fb}{(t^*)^{1/2} - \Fb} - 2 \Fa \ln((t^*)^{1/2} - \Fb) + \Fc (4B_0^2 - t^*) \\
&\leq t^* + 2 \Fa \Fb\left(\frac{1}{(t^*)^{1/2} - \Fb} - \frac{1}{2B_0 - \Fb}\right) \\
&~~~~+ 2 \Fa \ln\left(\frac{2B_0 - \Fb}{(t^*)^{1/2} - \Fb}\right) + 4B_0^2 \Fc.
\end{align*}

Let's choose $t^* = \left(\Fa + \Fb\right)^2$, which satisfies $t^* > \Fb^2$ because $\Fa > 0$. We can verify that that the definitions of $\Fa$ and $\Fb$, along with the constraints on the parameters specified in the theorem statement, guarantee that $\Fa \to 0$ and $\Fb \to 0$ as $n,m \to \infty$, whereas $B_0$ is a constant. Therefore we can assume $n,m$ are large enough such that this choice of $t^* \leq 4 B_0^2$. By substituting in our choice of $t^*$, it follows that
	\[ MSE(\hat{A}^k) 	\leq \left(\Fa + \Fb \right)^2 + 2 \Fa\Fb \left( \frac{1}{\Fa} - \frac{1}{2B_0-\Fb} \right) + 2\Fa \ln \left( \frac{2B_0-\Fb}{\Fa} \right) + 4B_0^2\Fc.  \]
We assume without loss of generality that $m,n$ are large enough such that $\Fb < 2 B_0$, which implies
\[\frac{1}{\Fa} - \frac{1}{2B_0-\Fb} \leq \frac{1}{\Fa} ~\text{ and }~ \frac{2B_0-\Fb}{\Fa} \leq \frac{2B_0}{\Fa}.\]
Therefore by substitution,
	\begin{align}
MSE(\hat{A}^k) 	&\leq (\Fa + \Fb)^2 + 2 \Fb + 2\Fa \ln\left(\frac{2B_0}{\Fa}\right) + 4B_0^2 \Fc \nonumber\\
				&= 2 \Fa \ln \left( \frac{2B_0}{\Fa}\right) + \left(\Fa + \Fb \right)^2 + 2\Fb + 4B_0^2 \Fc. \label{eqn:MSE_bd}
\end{align}
This MSE upper bound converges to $0$ as $\Fa, \Fb, \Fc \to 0$.
\end{proof}


\subsection{Results for Specific Probability Measures}

In this section, we simplify the results from Theorem \ref{thm:main_theorem} for specific choices of probability measures, namely the uniform measure over a $d$ dimensional Euclidean cube, or a measure which is only supported on finitely many points. Each of these cases leads to a specific form of the underestimator function $\phi(\cdot)$, which gives concrete bounds. We then choose specific expressions for $\zeta$, and $k$ to ensure that the mean squared error of our user-user $k$-nearest neighbor algorithm converges to zero. The parameter $\zeta$ in Theorem statement is introduced purely for the purpose of analysis, and is not used within the implementation of the the algorithm. Recall that it is used to define event $\Ed$, which holds when the $k$ rows in $\rowbase$ with minimum variance all satisfy $\sigma_{x_1(u) x_1(v)}^2 \leq \zeta$.  Intuitively, $\zeta$ is the thresholding parameter for the membership of similar neighbors. 

%To achieve the consistency of user-user variants, we require our matrix to be balanced, i.e., $m \leq \alpha n^{\Delta}$ for some $\alpha, \Delta > 0$. For the consistency of item-item variants, we need the other direction: $n \leq \alpha' m^{\Delta'}$ for some $\alpha', \Delta' > 0$. We also let the overlap parameter increase as the size of matrix at the rate faster than both $\log m$ and $\log n$, say, $\beta \geq c n^q$ for some $c, q > 0$.

\begin{proof}[Proof of Corollary \ref{coro:uniform}]

When the latent space is a cube in $\Reals^d$ equipped with the uniform probability measure, 
\[ \msra{ \sqrt{\frac{\zeta}{L^2}} } = C(2L)^{-d} \zeta^{d/2},\]
where $C$ is a normalization constant to ensure $\msra{\cX_1} = 1$.
We need to choose $\zeta$ so that $\zeta\geq \left(\frac{c_{\phi}}{C}\right)^{2/d} (2L)^{2} (mp)^{-4/3d} $ to satisfy the constraint on $\zeta$ in the statement of Theorem \ref{thm:main_theorem}: 
\begin{equation}\label{eqn:msra}
	\msra{\sqrt{\frac{\zeta}{L^2}}}\geq c_{\phi} \left(mp \right)^{-2/3} \text{ for some } c_{\phi} \geq 0.
\end{equation}
Therefore, let $c_{\phi} = 1$, and set $\zeta = \frac{(2L)^{2}}{C^{2/d}} (mp)^{-4/3d} $. We can plug it into the expression $\Fa$ in Theorem \ref{thm:main_theorem}  to get
\begin{align}
	\Fa 	&= \zeta + 2 \beta^{-1/3} + \frac{\gamma^2}{k}	\nonumber \\
		&\leq \left[ \frac{(2L)^{2}}{C^{2/d}} + 2 \right] \max \left\{ (mp)^{-4/3d}, \beta^{-1/3} \right\} + \frac{\gamma^2}{k}.		\label{eqn:F1_bound}
\end{align}

The assumption that $p \geq \max \left\{ m^{-1 + \delta}, n^{-\frac{1}{2} + \delta} \right\}$ for some $\delta > 0$ guarantees that $mp$ and $np^2$ diverge to $\infty$ as $m, n \to \infty$. As a result, $\Fb = (np^2)^{-1/3}$ converges to $0$.

To ensure $\Fc \to 0$ exponentially fast, we additionally require that $\log m < (np^2)^{\delta'/3}$ for some $\delta' > 0$. Additionally recall that $\beta = np^2/2$. The second term of $\Fc$ is thus upper bounded by
\begin{align*}
	\left( m + \frac{9}{2}mp\right) \exp \left( - c_2 \beta^{1/3} \right) &\leq \frac{11}{2} m  \exp \left( - c_2 (np^2/2)^{1/3} \right)\\
		& \leq \exp \left( \log \frac{11}{2} + (np^2)^{\delta'/3}  - c_2 (np^2/2)^{1/3} \right)\\
		&\leq \exp \left( \log \frac{11}{2}  - (np^2)^{1/3} \left( 2^{-1/3} c_2 - (np^2)^{-(1 - \delta')/3} \right) \right).
\end{align*}
Therefore, the exponent diverges to $-\infty$ polynomially in $np^2$ as $n \to \infty$ and hence, $\Fc$ decays exponentially to $0$ as $n \to \infty$.

We observe in Eq. (\ref{eqn:F1_bound}) that the rate of convergence of $\Fa$ is determined by the slowest among $\left\{ (mp)^{-4/3d}, \beta^{-1/3}, \frac{1}{k} \right\}$. Since $\Fb = \beta^{-1/3}$ and $\Fc$ decays exponentially fast, we can see that $\Fa$ is the critical error term, which converges to 0 most slowly among $\Fa, \Fb, \Fc$. By definition, $\Fa \geq 2 \Fb$. Hence, the convergence rate of MSE in Eq. (\ref{eqn:MSE_bd}) is dominated by the first term $2 \Fa \ln \left( \frac{2B_0}{\Fa} \right)$. To be more concrete, since $\Fa + \Fb =  \zeta + 3\beta^{-1/3} + \frac{\gamma^2}{k} \leq \frac{3}{2}\Fa$, $\left(\Fa+ \Fb \right)^2 \leq \frac{9}{4} \Fa^2 \leq \frac{9}{4}\Fa$. Given $\Fa \leq \frac{1}{2}$, we have $\Fa \leq \ln \left(\frac{2B_0}{\Fa}\right)$ because $B_0 \geq 1$ and $\ln \left( \frac{2}{x} \right) \geq 1$ for $0 < x \leq \frac{1}{2}$. Therefore,
    \begin{align}
	MSE(\hat{A}) &\leq  2 \Fa \ln \left( \frac{2B_0}{\Fa}\right) + \left(\Fa + \Fb \right)^2 + 2\Fb + 4B_0^2 \Fc	\nonumber\\
		&\leq 2 \Fa \ln \left( \frac{2B_0}{\Fa}\right) + \frac{9}{4}\Fa^2 + \Fa + 4B_0^2 \Fc	\nonumber\\
		&\leq \frac{21}{4} \Fa \ln \left( \frac{2B_0}{\Fa}\right) + 4B_0^2\Fc 	\label{eqn:MSE_simplified}
    \end{align}
given $\Fa \leq \frac{1}{2}$, which is satisfied for large enough $np^2 \gg 1$ and $k \gg 1$.

Now suppose that we choose $k = \frac{1}{8}\left(mp\right)^{1/3}$. Our choice of $\zeta= \frac{(2L)^{2}}{C^{2/d}} (mp)^{-4/3d} $ guarantees $\msra{\sqrt{\frac{\zeta}{L^2}}} \geq (mp)^{-2/3}$ in Eq. (\ref{eqn:msra}), and hence, $k \leq \frac{c_k}{2}(m-1)p \msra{\sqrt{\frac{\zeta}{L^2}}}$ for $c_k = \frac{1}{2}$ (we assumed $\frac{m}{2} \leq m - 1$ here). Then
\begin{align*}
	\Fa 	&= \zeta + 2 \beta^{-1/3} + \frac{\gamma^2}{k} \\
		&\leq \left[ \frac{(2L)^{2}}{C^{2/d}} + 2 + 8 \gamma^2 \right] \max \left\{ (mp)^{-4/3d}, \beta^{-1/3}, \left( mp \right)^{-1/3} \right\}.
\end{align*}
Plugging this into Eq. (\ref{eqn:MSE_simplified}) gives a simplified bound in Corollary \ref{coro:uniform}.

\end{proof}

%Therefore, we can reduce the bound to
%\begin{align*}
%MSE(\hat{A})
%&\leq 2\Fa \ln\left(\frac{2^{1/2}}{\Fa}\right) + 2 \Fb + (\Fb + \Fa)^2 + 2 \Fc \\
%&= \tilde{O}\left( \Fa \right)\\
%&= \tilde{O}\left(  \max \left\{ (mp)^{-4/3d}, (np^2)^{-1/3}, \left( mp \right)^{-1/3} \right\} \right).
%\end{align*}

A slight modification of the above proof yields a proof for the MSE bound when the latent row feature variable distribution $P_{\cX_1}$ is only supported on a finite number of atoms.
\begin{proof}[Proof of Corollary \ref{coro:discrete}]
When the latent space consists of a finite number of points, in other words, $\prxa$ is supported only on a finitely many points, any choice of $\zeta > 0$ satisfies $\msra{\sqrt{\frac{\zeta}{L^2}}}\geq \min_{x \in supp(\prxa)}\{\msra{x}\}$, and hence, one can easily find $c_{\phi} \geq 0$ for which $\msra{\sqrt{\frac{\zeta}{L^2}}}\geq c_{\phi} \left(mp \right)^{-2/3}$. We will simply let $\zeta = \beta^{-1/3}$ in such a case. Again, suppose that we choose $k = \frac{1}{8}\left(mp\right)^{1/3}$. This leads to
\begin{align*}
	\Fa 	&= \zeta + 2 \beta^{-1/3} + \frac{\gamma^2}{k} \\
		&\leq \left[ 3 + 8 \gamma^2 \right] \max \left\{ \beta^{-1/3}, \left( mp \right)^{-1/3} \right\}.
\end{align*}
The remaining arguments in the proof of Corollary 4.3 with regards to terms $\Fb$ and $\Fc$ also follow. We plug in this upper bound for $\Fa$ again into Eq. (\ref{eqn:MSE_simplified}) to prove Corollary \ref{coro:discrete}.
\end{proof}

==> contents/matrix_results/comparison_USVT.tex <==




==> contents/matrix_results/maintheorem_christina.tex <==
\section{Main Results} \label{sec:main.result}

%%% ====================================================================
%%%	Theorem Statement
%%% ====================================================================

\subsection{Theorem Statement}

We present a theorem which upper bounds the MSE of the estimate produced by the user-user $k$-nearest neighbor algorithm 
presented in Section \ref{sec:user_user} (cf. Algorithm \ref{alg:user_algorithm}). Recall from our problem statement in Section \ref{sec:setup} 
that $p$ is the probability each entry is observed, $\lip$ is the Lipschitz constant of the latent function $f$, $ \diamrow$ is the diameter of 
the latent space of the row latent variables, and $\sigma^2$ is an upper bound on the noise variance\footnote{In fact, $\| N(u,i) \|_{\psi_2} 
\leq \sigma$. We may identify $\sigma^2$ with an upper bound on the variance, up to an absolute constant.}. We shall use 
notation $B(x,r) = \{x' \in \latsprow: \drow(x, x') \leq r \}$ for any $r > 0$. 


\chris{It turns out that the relevant property (rather than Lipschitzness) is the local measure with respect to the $L_2$ functional distances ... let us denote
\begin{align*}
\phi(\featrow{1}, r) = \Prob{\big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq r ~|~ \featrow{1}}
\end{align*}
Let $K$ denote an upper bound on $\big\| Z(1,j) - Z(v,j) \big\|_{\psi_2}$. For the Lipschitz setting, we can use
\[K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2\]
but for the finite types setting, then it doesn't depend on Lipschitz constant.}



%
%We introduce a function $\msrrow: \Reals_{++} \to [0,1]$ which reflects a property of the local measure and geometry of the latent space. For any $r > 0$,
%\[	\msrrow(r) \triangleq \ess\inf_{x \in \latsprow} \murow(B(x, r)),	\]
%where $B(x,r) = \{x' \in \latsprow: \drow(x, x') \leq r \}$. This function gives a lower bound on the measure of a ball with radius $r$ centered at 
%a typical point $x \in \latsprow$. One can interpret this as a lower bound on the probability for a typical row to find a neighbor within distance $r$ 
%at a random draw.
%
%\begin{example}[Finite support]
%	If $\murow$ has a finite support on $\latsprow$, then $\msrrow(r) \geq \min_{x \in \supp \murow} \murow(x)$ for all $r > 0$.
%\end{example}
%
%\begin{example}[Cube and the Lebesgue measure]
%	If $\latsprow = [0, D]^d$ (equipped with the $\ell_{\infty}$-metric topology) for some positive integer $d$, and $\murow$ is 
%	the Lebesgue measure on the unit cube, then $\msrrow(r) = \big(\frac{r}{D}\big)^d$ for all $r \in [0, D]$.	
%\end{example}
%
Theorem \ref{thm:main_mse_user} presents an upper bound on the mean-squared error (cf. \eqref{eqn:MSE}) of the user-user fixed radius nearest neighbor 
algorithm described in Algorithm \ref{alg:user_algorithm}. %Recall the definition of MSE from \eqref{eqn:MSE}.

Due to exchangeability, the expected error is identically distributed for different entries, and thus without loss of generality we present the error bound based on estimating entry $(1,1)$.
\begin{theorem}[Main Theorem]\label{thm:main_mse_user}
Let $\hA_{11}$ be the estimator returned by the Algorithm \ref{alg:user_algorithm} for estimating entry $(1,1)$. Suppose that our algorithm uses threshold parameter $\eta \geq \eta' 
+ K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)$ for some $\eta' \geq 2 \sigma^2$. Then
\begin{align*}
	\E[(\hA_{11} - A_{11})^2] &\leq \big( \eta - 2\sigma^2 \big) + CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg]
		+ 2 \bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg]^{-1}\Bigg] \\
		&\qquad 	+ \frac{1}{m-1}
		+ \bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg) \Bigg]
		+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
In the above expression, $C, c > 0$ are absolute constants, and 
\begin{align*}
\phi(\featrow{1}, r) = \Prob{\big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq r ~|~ \featrow{1}}
\end{align*}
for any $x \in  \latsprow$ and $r > 0$. 
\end{theorem}

\DG{Should plug in the result from Lemma \ref{lem:prob_zero}: add $(\lip \diamrow)^2 \bbE_{\featrow{1}} \Big[\Prob{\Nbase = 0 ~\big|~ \featrow{1}}\Big]$ where
\begin{align*}
	\Prob{\Nbase = 0 ~\big|~ \featrow{1}}
		&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
			+ \frac{1}{(m-1)^2} + \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
}

The threshold $\eta \geq 0$ is a tunable parameter that our algorithm uses. Our analysis captures the bias-variance tradeoff associated with 
the parameter $\eta$. When $\eta$ is too large, our upper bound becomes loose because the algorithm utilizes information from 
less reliable neighbors; on the other hand, when $\eta$ is chosen too small, the resulting estimate count only on a few neighbors 
and suffers from large variance. 

The first two terms of the MSE bound come from bounding the bias of the estimator. The first term $\big( \eta - 2\sigma^2 \big)$ reflects the bias that is unavoidable due to the selection of the threshold $\eta$ and the error in estimating $\dissimrow(u,v)$, and the second term bounds the tail of the bias along with the bad event that $| \basesim(u) \cap \basesim(v) |$ is too small to produce a good estimate of $\dissimrow(u,v)$. The remaining four terms bound the variance of the estimator. 

%
%, where $2 \left[  (m-1)p  \cdot \msrrow ( \sqrt{\eta' - 2\sigma^2}/L) \right]^{-1}$ is the dominating term, reflecting that the variance scales as one over the number of ``nearest neighbors'' that our estimator averages over. The last three terms result from bounding the probability of bad events where $| \basesim(u) \cap \basesim(v) |$ or $| \baseest(u,i) |$ are too small. The optimal choice of $\eta$ is the one that trades off between the dominating terms of the bias and the variance.

%Comparing the sample requirements for $p$ in both theorems indicates that the user-user variant is more suitable for a fat matrix, and the item-item variant is more suitable for a tall matrix. This is due to the fact that the limiting condition of our sample complexity requires that there is a sufficiently large overlap between pairs of rows or columns. A fat matrix will naturally satisfy the condition $(np^2)^{\delta'/3} \geq n^{2 \delta' \delta/3 } \geq \log m$, and a tall matrix will naturally satisfy the condition $ (mp^2)^{\delta'/3} \geq m^{2 \delta' \delta/3 } \geq \log n$, and a square matrix will satisfy both conditions, guaranteeing that the term $\Fc$ decays to $0$ exponentially fast. 
%
%The parameter $\beta$ determines the required overlap between rows, such that choosing $\beta$ to grow with $m, n$, such as $\beta = np^2/2$, ensures that asymptotically the empirical mean $\muv$ and variance $\suv^2$ computed in the algorithm converge to the true mean and variance. Given any choice of $\beta$, we can derive the rates of convergence of the empirical mean and variance statistics (see Lemmas \ref{lem:mean} and \ref{lem:variance}), which also impacts the MSE of the final estimate. The parameter $k$ determines the number of nearest neighbor rows which are incorporated in the final estimate in \eqref{eq:user-user_final_est}. We choose $k$ to balance bias and variance, ensuring that $k$ goes to infinity with $m$ and $n$ to drive down the error due to the individual additive noise terms $\eta$, yet also controlling that $k$ grows slowly enough to guarantee that the sample variance $\suv^2$ of the $k$ nearest neighbor rows goes to zero as well.
%
%In the process of proving the bound on the mean squared error, we are able to in fact upper bound the tail probability of error for each entry as presented in Theorem \ref{thm:main_tail}. This entry-wise error bound is stronger than a MSE bound over the aggregate error, suggesting that the error is evenly spread amongst different entries.


%%% ====================================================================
%%%	Two Examples
%%% ====================================================================

\subsection{Implications} 

Theorem \ref{thm:main_mse_user} provides bound on MSE for Algorithm \ref{alg:user_algorithm}, which depends on 
the underlying probability measure through $\phi$. Here we evaluate this implicit bound for
two special examples of $\murow$, distribution with finite support and uniform; as well as an explicit bound for
any distribution.  

\medskip
\noindent{\bf $\murow$ has finite support.} We state the following Corollary of Theorem \ref{thm:main_mse_user} when $\murow$ 
has finite support. 
\begin{coro}[Finite support]\label{coro:finite}
Suppose that $\latsprow$ is equipped with the discrete metric\footnote{$\drow(x_1, x_2) = 1$ if and only if $x_1 \neq x_2$.} topology 
and $\murow$ has finite support in $\latsprow$ with $\supp(\murow)$ denoting the support of $\murow$. Let 
$$\eta = \eta' + K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg), \quad \mbox{and}\quad \eta' = 2\sigma^2 + \min\Bigg(\frac{L^2}{4}, K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)\Bigg) $$
where $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$.\chris{update $K$ expression} If 
$p \geq \max\Bigg(\frac{8}{m-1}, \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}\Bigg)$, then 
\begin{equation}\label{cor.MSE_finite}
	\MSE(\hat{A}) 
		\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)
		+ C' \frac{|\supp(\murow)|}{(m-1)p} 
\end{equation}
where $C, c, C' > 0$ are absolute constants. 
\end{coro}
That is, as long as $p \gg \max\Bigg(\frac{1}{m}, \sqrt{\frac{\log m}{n}}\Bigg)$, under discrete measure with finite support 
\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee \frac{|\supp(\murow)|}{(m-1)p} \Bigg).	\]

\begin{proof}[Proof of Corollary \ref{coro:finite}]
Our interest is in bounding 
\begin{align}\label{eq.term1}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \phi(\featrow{1}, \eta'-2\sigma^2) \bigg]^{-1}\Bigg] 
\end{align}
and 
\begin{align}\label{eq.term2}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg) \Bigg]
\end{align}
from the statement of Theorem \ref{thm:main_mse_user} to obtain the desired result. Since we are considering discrete metric with measure having finite support, 
for any value of $r \geq 0$ and $x \in \supp(\murow)$,  $\phi(x, r) \geq \murow(x)$. Given choice of $\eta'$, we have that 
$\eta'-\sigma^2 \geq 0$. Therefore, \eqref{eq.term1} can be written as
\begin{align}\label{eq.term1a}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot   \phi(\featrow{1}, \eta'-2\sigma^2) \bigg]^{-1}\Bigg] 
& \geq \sum_{x \in \supp(\murow)} \murow(x) \times \frac{1}{(m-1)p  \murow(x)} \nonumber  \\
& = \frac{| \supp(\murow)| }{(m-1)p}.
\end{align}
Similarly, \eqref{eq.term2} reduces to 
\begin{align}\label{eq.term2a}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot  \phi(\featrow{1}, \eta'-2\sigma^2) \bigg) \Bigg] 
& = \sum_{x \in \supp(\murow)} \murow(x) \times \exp\bigg( - \frac{(m-1)p}{8} \murow(x)  \bigg) \nonumber \\
& \leq | \supp(\murow)| \Bigg\{ \sup_{\theta \in [0,1]} \theta \exp\bigg( - \frac{(m-1)p}{8} \theta  \bigg) \Bigg\} \nonumber \\
& = | \supp(\murow)| \frac{8\exp(-1)}{(m-1)p}.
\end{align}
In above, we have used an easy to verify fact that $ \sup_{\theta \in [0,1]}  \theta \exp\bigg( - \frac{(m-1)p}{8} \theta  \bigg)$ is
achieved for $\theta = \frac{8}{(m-1)p} \in [0,1]$. Replacing \eqref{eq.term1a} and \eqref{eq.term2a} in the statement of Theorem \ref{thm:main_mse_user}, we obtain \eqref{cor.MSE_finite}.
\end{proof}

\medskip
\noindent{\bf $\murow$ is uniform measure.} We consider setting where $\murow$ is uniform Lebesgue measure on $[0,1]^d$, the unit cube in $d$ dimension. 
There exists universal constant $\alpha, \beta > 0$ such that for any $d \geq 1$, and $x \in [0,1]^d$ and $r > 0$, 
\begin{align}
\mbox{Vol}(B(x,r)) & \geq \min(1, \alpha \beta^d  r^d). 
\end{align} 
We state the following implication of Theorem \ref{thm:main_mse_user} in this setting. 
\begin{coro}[Unit cube and the Lebesgue measure]\label{coro:uniform}
Let $\murow$ be uniform measure on $\latsprow = [0,1]^d$. Let 
$$\eta = \eta' +  K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big), \quad\mbox{and}$$
$$ \eta' = 2 \sigma^2 +  \alpha^{2/d} \beta^2 L^2 \Big((m-1)p\Big)^{-\frac{2}{d+2}},$$
%
%(LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}.$$ 
where $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$.  If $p \geq \max\Bigg(\frac{8}{m-1}, \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}\Bigg)$, then
\begin{align}\label{cor.MSE_uniform}
	\MSE(\hat{A}) 
		&\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)
		+ C' \alpha^{2/d} \beta^2 L^2 \big[ (m-1)p \big]^{-\frac{2}{d+2}}
		+  \exp\Big( - \frac{1}{8} \big[ (m-1)p \big]^{\frac{2}{d+2}} \Big)
\end{align}
where $C, C', c > 0$ are absolute constants.
\end{coro}
That is, as long as $p \gg \max\Bigg(\frac{1}{m}, \sqrt{\frac{\log m}{n}}\Bigg)$, under uniform measure 
\[	\MSE(\hat{A}) = O \Bigg( (LD + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee L^2 \Big(\frac{1}{(m-1)p}\Big)^{\frac{2}{d+2}} \Bigg).	\]
\begin{proof}[Proof of Corollary \ref{coro:uniform}]
Similar to proof of Corollary \ref{coro:finite}, our interest is in bounding \eqref{eq.term1} and \eqref{eq.term2}. To that end, under
%uniform Lebesgue measure, $\murow$, on $d$ dimensional unit cube $\lastprow$, it follows that for any $x \in \lastprow$ and $r > 0$
\begin{align}
\localprob(x, r) & \geq \min\Big(1, \alpha \beta^d r^d\Big), 
\end{align}
where $C(d)$ is constant that is dependent on $d$, precisely exponentially small in $d$. Therefore, by choice of $\eta'$
\begin{align}\label{eq.term1b}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg] 
& \leq \frac{1}{(m-1)p} \times \frac{\alpha \beta^d L^d}{(\eta' - 2\sigma^2)^{d/2}} \nonumber \\
& = \Big((m-1)p\Big)^{-\frac{2}{d+2}}.
\end{align}
Similarly, 
\begin{align}\label{eq.term2b}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg] 
& \leq \exp\bigg( - \frac{(m-1)p}{8}  \times \frac{(\eta' - 2\sigma^2)^{d/2}}{\alpha \beta^d L^d}\bigg) \nonumber \\
& \leq \exp\bigg( - \frac18 \Big((m-1)p\Big)^{\frac{2}{d+2}}\bigg).
\end{align}
From \eqref{eq.term1b} and \eqref{eq.term2b}, and statement of Theorem \ref{thm:main_mse_user}, we conclude \eqref{cor.MSE_uniform}.
\end{proof}



%\medskip
%\noindent{\bf $\murow$ is any measure.}

%
%
%
%\subsection{Two Examples Given Local Geometry of Latent Probability Measure}
%Observe that the upper bound on the MSE in Theorem \ref{thm:main_mse_user} consists of multiple terms. Ideally, we want to choose 
%$\eta \to 2\sigma^2$ so that the first term vanishes, however, that leads to $\msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \to 0$ and 
%the inflation of the terms $2 \Big[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \Big]^{-1}$ and 
%$ \exp\Big( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \Big)$. Therefore, we want to find the best upper bound 
%where the competing terms in the upper bound are balanced.
%
%The ``local geometry'' of the probability measure $\murow$ on the latent space $\latsprow$ through the function $\msrrow$ determines 
%the impact of the latent space dimension on the sample complexity and error convergence rate of the user-user $k$-nearest neighbor algorithm. 
%We consider two examples -- discrete probability measure with finite support and the Lebesgue measure on the unit cube in $\Reals^d$ -- to 
%illustrate the impact. 
%
%%Since the algorithm is a neighbor-based method, we need to guarantee that for each row $u \in [m]$, there are sufficiently many rows $v \in \rowbase$ such that the variances of their row differences are small, which we showed in section \ref{sec:taylor} intuitively implies bounds on $|\hat{A}_{vj}(u,i) - \hat{A}(u,i)|$ for the average column $j$. By our model assumption that the matrix $A$ is described by an $L$-Lipschitz function $f$, it is sufficient to show that with high probability, there exists sufficiently many rows $v \in \rowbase$ such that $d_{\cX_1}(x_1(u), x_1(v))$ is small, which implies the differences in their functional values are small, and thus the sample variance of their differences is also small. This is directly related to the function $\phi_1$, since it lower bounds the probability for the latent variable $x_1(v)$ to be sampled within a $r$-radius ball around $x_1(u)$ such that $d_{\cX_1}(x_1(u), x_1(v)) < r$.
%
%In the simple setting where $\murow$ is supported only on a finite number of points, i.e. there are only finitely many latent row 
%types, the convergence rate of the MSE upper bound and the sample complexity have {\em no} dependency on dimension of the latent 
%spaces. This follows from the fact that $\msrrow(r) \geq \min_{x \in \latsprow} \murow(x)$ even when $r \to 0$. Corollary \ref{coro:finite} presents the simplified 
%MSE upper bound for the finite support setting.
%
%\begin{coro}[Finite support]\label{coro:finite}
%Suppose that $\latsprow$ is equipped with the discrete metric\footnote{$\drow(x_1, x_2) = 1$ if and only if $x_1 \neq x_2$.} topology and $\murow$ has finite support 
%in $\latsprow$. Let $\pmin \triangleq \min_{x \in \supp~ \murow} \murow(x)$. Let $\hat{A}$ be the output of our user-user $k$-nearest neighbor algorithm using a threshold parameter of $\eta \geq \eta' + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, 
%\frac{4 \log (m-1)}{c(n-1)p^2} \Big)$ for some $\eta' \geq 2 \sigma^2$. If $p \geq \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}$, 
%then
%\begin{equation*}\label{eqn:MSE_finite}
%	\MSE(\hat{A}) 
%		\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2}, \frac{2}{m-1} \bigg)
%		+ \frac{2}{\pmin\cdot (m-1)p} 
%		+  \exp\bigg( - \frac{\pmin}{8} (m-1)p \bigg)
%\end{equation*}
%where $C, c > 0$ are absolute constants. \chris{Do we need to repeat or reference the definition of $K$ again?}
%\end{coro}
%
%\begin{remark}\label{rem:finite}
%When the latent space is a discrete metric space and the underlying measure is supported on a finitely many number of points, 
%\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee \frac{1}{\pmin}\frac{1}{(m-1)p} \Bigg).	\]
%\DG{I believe that $L$ should be removed; but we cannot do that with our current analysis.}
%\end{remark}
%
%\begin{remark}
%	\DG{***TODO: I don't know whether we can do this.}Simplification to
%	\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee | \supp ~ \murow |\frac{1}{(m-1)p} \Bigg).	\]
%\end{remark}
%
%Next, we suppose $\murow$ is the Lebesgue probability measure on the cube of side length $D$ in $\Reals^d$ (i.e. uniform measure on the 
%$d$-dimensional cube). Then for $r > 0$,
%\[
%	\msrrow(r) = \min_{x_0 \in \cX_1} \murow\big( B(x_0, r \big))= \min\left\{1, \Big(\frac{r}{D}\Big)^d\right\}.
%\]
%\begin{remark}[Maximum latent dimension for the neighbor-based algorithm to succeed.]
%Due to the uniform random sampling of the latent features, this expressions shows that we need to sample $\Omega(r^{-d})$ number of rows 
%to guarantee that there is at least one row whose latent feature is within distance $r$ of $x_0$ for all $x_0 \in \latsprow$. Therefore, we 
%require $m \gg r^{-d}$ in the regime $r \to 0$. This implies that we need the dimension of the latent space to satisfy $d = o(\log m)$. 
%\end{remark}
%
%Corollary \ref{coro:uniform} presents a simplified MSE upper bound when the row latent variables are sampled according to the uniform measure on the $d$-dimensional 
%unit cube.
%
%\begin{coro}[Unit cube and the Lebesgue measure]\label{coro:uniform}
%Suppose that $\murow$ is the uniform measure on $\latsprow = [0,1]^d$ and our user-user $k$-nearest neighbor algorithm uses $\eta \geq \eta' + 
%K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$ where $\eta' = 2 \sigma^2 + (LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}$. 
%If $p \geq \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \frac{4 \sqrt{\log(m-1)}}{\sqrt{n-1}}$, then
%\begin{align*}\label{eqn:MSE_uniform}
%	\MSE(\hat{A}) 
%		&\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2}, \frac{2}{m-1} \bigg)
%		+ 3(LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}
%		+  \exp\Big( - \frac{1}{8} \big[ (m-1)p \big]^{\frac{2}{d+2}} \Big)
%\end{align*}
%where $C, c > 0$ are absolute constants.
%\end{coro}
%
%\begin{remark}\label{rem:uniform}
%When the latent space is a $d$-dimensional cube of side length $D$ equipped with the uniform measure on it, 
%\[	\MSE(\hat{A}) = O \Bigg( (LD + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee (LD)^{\frac{2d}{d+2}} \Big(\frac{1}{(m-1)p}\Big)^{\frac{2}{d+2}} \Bigg).	\]
%\end{remark}


==> contents/matrix_results/maintheorem_ds.tex <==
\section{Main Results} \label{sec:main.result}

%%% ====================================================================
%%%	Theorem Statement
%%% ====================================================================

\subsection{Theorem Statement}

We present a theorem which upper bounds the MSE of the estimate produced by the user-user $k$-nearest neighbor algorithm 
presented in Section \ref{sec:user_user} (cf. Algorithm \ref{alg:user_algorithm}). Recall from our problem statement in Section \ref{sec:setup} 
that $p$ is the probability each entry is observed, $\lip$ is the Lipschitz constant of the latent function $f$, $ \diamrow$ is the diameter of 
the latent space of the row latent variables, and $\sigma^2$ is an upper bound on the noise variance\footnote{In fact, $\| N(u,i) \|_{\psi_2} 
\leq \sigma$. We may identify $\sigma^2$ with an upper bound on the variance, up to an absolute constant.}. We shall use 
notation $B(x,r) = \{x' \in \latsprow: \drow(x, x') \leq r \}$ for any $r > 0$. 
%
%We introduce a function $\msrrow: \Reals_{++} \to [0,1]$ which reflects a property of the local measure and geometry of the latent space. For any $r > 0$,
%\[	\msrrow(r) \triangleq \ess\inf_{x \in \latsprow} \murow(B(x, r)),	\]
%where $B(x,r) = \{x' \in \latsprow: \drow(x, x') \leq r \}$. This function gives a lower bound on the measure of a ball with radius $r$ centered at 
%a typical point $x \in \latsprow$. One can interpret this as a lower bound on the probability for a typical row to find a neighbor within distance $r$ 
%at a random draw.
%
%\begin{example}[Finite support]
%	If $\murow$ has a finite support on $\latsprow$, then $\msrrow(r) \geq \min_{x \in \supp \murow} \murow(x)$ for all $r > 0$.
%\end{example}
%
%\begin{example}[Cube and the Lebesgue measure]
%	If $\latsprow = [0, D]^d$ (equipped with the $\ell_{\infty}$-metric topology) for some positive integer $d$, and $\murow$ is 
%	the Lebesgue measure on the unit cube, then $\msrrow(r) = \big(\frac{r}{D}\big)^d$ for all $r \in [0, D]$.	
%\end{example}
%

Theorem \ref{thm:main_mse_user} presents an upper bound on the mean-squared error (cf. \eqref{eqn:MSE}) of 
the user-user Fixed radius nearest neighbor algorithm described in Algorithm \ref{alg:user_algorithm}. %Recall the definition of MSE from \eqref{eqn:MSE}.
Before presenting the theorem statement, we remark that 
\[	\MSE(\hA) = \Exp{\big( \hA(u,i) - A(u,i) \big)^2 }	 = \Exp{\big( \hA(1,1) - A(1,1) \big)^2 }.	 \]
due to the exchangeability of the model and the linearity of the expectation. In Theorem \ref{thm:main_mse_user}, 
we provide an upper bound on $\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1} }$, conditioned on $\featrow{1}$, 
which is the latent feature of the first row.

\begin{theorem}[Main Theorem]\label{thm:main_mse_user}
Let $\hA$ be the estimator returned by the Algorithm \ref{alg:user_algorithm}. Let constant $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$. Suppose that our algorithm uses threshold parameter $\eta \geq \eta' 
+ K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)$ for some $\eta' \geq 2 \sigma^2$. Then
\begin{align*}
	&\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1} }\\
	&\qquad\leq \big( \eta - 2\sigma^2 \big) + CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg]
		+ 2 \bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  
		\localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg] \\
		&\qquad \quad
		+ \big( (\lip \diamrow)^2 + 1 \big) \bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot 
		\localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg]\\
		&\qquad \quad
		+ \big[ (m-1) + (\lip \diamrow)^2 \big] \bigg[  \frac{1}{(m-1)^2} + \exp \Big( - \frac{(n-1)p^2}{8} \Big) \bigg].
\end{align*}
In the above expression, $C, c > 0$ are absolute constants, and $\localprob(x, r) = \murow(B(x, r))$ for any $x \in  \latsprow$ and $r > 0$. 
\end{theorem}

The threshold $\eta \geq 0$ is a tunable parameter that our algorithm uses. Our analysis captures the bias-variance tradeoff associated with 
the parameter $\eta$. When $\eta$ is too large, our upper bound becomes loose because the algorithm utilizes information from 
less reliable neighbors; on the other hand, when $\eta$ is chosen too small, the resulting estimate count only on a few neighbors 
and suffers from large variance. 

The first two terms of the MSE bound come from bounding the bias of the estimator. The first term $\big( \eta - 2\sigma^2 \big)$ reflects the bias that is unavoidable due to the selection of the threshold $\eta$ and the error in estimating $\dissimrow(u,v)$, and the second term bounds the tail of the bias along with the bad event that $| \basesim(u) \cap \basesim(v) |$ is too small to produce a good estimate of $\dissimrow(u,v)$. The remaining three terms bound the variance of the estimator; the error bound for the trivial estimates (when $\baseest(1,1) = \emptyset$), given in the form of $(\lip \diamrow)^2 \Prob{\baseest(1,1) = \emptyset} $ is also subsumed in these three terms.

\begin{remark}
Given a lower bound on $\inf_{\featrow{1} \in \latsprow }q(\featrow{1}, r)$, replacing $q$ functions in the upper bound stated in 
Theorem \ref{thm:main_mse_user} with the uniform (with respect to $\featrow{1} \in \latsprow$) lower bound yields a uniform 
upper bound on $\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1} }$, which leads to an upper bound on
\[	\MSE(\hA) = \bbE_{\featrow{1} \sim \murow} \Big[ \Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1} } \Big].	\]
%In Theorem \ref{thm:main_mse_user}, we presented an upper bound on the mean squared error, in the conditional form on 
%$\featrow{1}$. The main purpose was 
\end{remark}

%
%, where $2 \left[  (m-1)p  \cdot \msrrow ( \sqrt{\eta' - 2\sigma^2}/L) \right]^{-1}$ is the dominating term, reflecting that the variance scales as one over the number of ``nearest neighbors'' that our estimator averages over. The last three terms result from bounding the probability of bad events where $| \basesim(u) \cap \basesim(v) |$ or $| \baseest(u,i) |$ are too small. The optimal choice of $\eta$ is the one that trades off between the dominating terms of the bias and the variance.

%Comparing the sample requirements for $p$ in both theorems indicates that the user-user variant is more suitable for a fat matrix, and the item-item variant is more suitable for a tall matrix. This is due to the fact that the limiting condition of our sample complexity requires that there is a sufficiently large overlap between pairs of rows or columns. A fat matrix will naturally satisfy the condition $(np^2)^{\delta'/3} \geq n^{2 \delta' \delta/3 } \geq \log m$, and a tall matrix will naturally satisfy the condition $ (mp^2)^{\delta'/3} \geq m^{2 \delta' \delta/3 } \geq \log n$, and a square matrix will satisfy both conditions, guaranteeing that the term $\Fc$ decays to $0$ exponentially fast. 
%
%The parameter $\beta$ determines the required overlap between rows, such that choosing $\beta$ to grow with $m, n$, such as $\beta = np^2/2$, ensures that asymptotically the empirical mean $\muv$ and variance $\suv^2$ computed in the algorithm converge to the true mean and variance. Given any choice of $\beta$, we can derive the rates of convergence of the empirical mean and variance statistics (see Lemmas \ref{lem:mean} and \ref{lem:variance}), which also impacts the MSE of the final estimate. The parameter $k$ determines the number of nearest neighbor rows which are incorporated in the final estimate in \eqref{eq:user-user_final_est}. We choose $k$ to balance bias and variance, ensuring that $k$ goes to infinity with $m$ and $n$ to drive down the error due to the individual additive noise terms $\eta$, yet also controlling that $k$ grows slowly enough to guarantee that the sample variance $\suv^2$ of the $k$ nearest neighbor rows goes to zero as well.
%
%In the process of proving the bound on the mean squared error, we are able to in fact upper bound the tail probability of error for each entry as presented in Theorem \ref{thm:main_tail}. This entry-wise error bound is stronger than a MSE bound over the aggregate error, suggesting that the error is evenly spread amongst different entries.


%%% ====================================================================
%%%	Two Examples
%%% ====================================================================

\subsection{Implications} 

Theorem \ref{thm:main_mse_user} provides an upper bound on MSE for Algorithm \ref{alg:user_algorithm}, which depends on 
the underlying probability measure $\murow$ through $\localprob$. Here we evaluate this implicit bound for
two special examples of $\murow$, distribution with finite support and uniform; as well as an explicit bound for
any distribution.  

\medskip
\noindent{\bf $\murow$ has finite support.} We state the following Corollary of Theorem \ref{thm:main_mse_user} when $\murow$ 
has finite support. 
\begin{coro}[Finite support]\label{coro:finite}
Suppose that $\latsprow$ is equipped with the discrete metric\footnote{$\drow(x_1, x_2) = 1$ if and only if $x_1 \neq x_2$.} topology 
and $\murow$ has finite support in $\latsprow$ with $\supp(\murow)$ denoting the support of $\murow$. Let 
$$\eta = \eta' + K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg), \quad \mbox{and}\quad \eta' = 2\sigma^2 + \min\Bigg(\frac{L^2}{4}, K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)\Bigg) $$
where $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$. If 
$p \geq \max\Bigg(\frac{8}{m-1}, \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}\Bigg)$, then 
\begin{equation}\label{cor.MSE_finite}
	\MSE(\hat{A}) 
		\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)
		+ C' \frac{|\supp(\murow)|}{(m-1)p} 
\end{equation}
where $C, c, C' > 0$ are absolute constants. 
\end{coro}
That is, as long as $p \gg \max\Bigg(\frac{1}{m}, \sqrt{\frac{\log m}{n}}\Bigg)$, under discrete measure with finite support 
\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee \frac{|\supp(\murow)|}{(m-1)p} \Bigg).	\]

\begin{proof}[Proof of Corollary \ref{coro:finite}]
Our interest is in bounding 
\begin{align}\label{eq.term1}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg] 
\end{align}
and 
\begin{align}\label{eq.term2}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg]
\end{align}
from the statement of Theorem \ref{thm:main_mse_user} to obtain the desired result. Since we are considering discrete metric with measure having finite support, 
for any $r \in (0,1)$ and $x \in \supp(\murow)$,  $\localprob(x, r) = \murow(x)$. Given choice of $\eta'$, we have that 
$\frac{\sqrt{\eta' - 2\sigma^2}}{{L}} \leq \frac12$. Therefore, \eqref{eq.term1} can be written as
\begin{align}\label{eq.term1a}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg] 
& = \sum_{x \in \supp(\murow)} \murow(x) \times \frac{1}{(m-1)p  \murow(x)} \nonumber  \\
& = \frac{| \supp(\murow)| }{(m-1)p}.
\end{align}
Similarly, \eqref{eq.term2} reduces to 
\begin{align}\label{eq.term2a}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg] 
& = \sum_{x \in \supp(\murow)} \murow(x) \times \exp\bigg( - \frac{(m-1)p}{8} \murow(x)  \bigg) \nonumber \\
& \leq | \supp(\murow)| \Bigg\{ \sup_{\theta \in [0,1]} \theta \exp\bigg( - \frac{(m-1)p}{8} \theta  \bigg) \Bigg\} \nonumber \\
& = | \supp(\murow)| \frac{8\exp(-1)}{(m-1)p}.
\end{align}
In above, we have used an easy to verify fact that $ \sup_{\theta \in [0,1]}  \theta \exp\bigg( - \frac{(m-1)p}{8} \theta  \bigg)$ is
achieved for $\theta = \frac{8}{(m-1)p} \in [0,1]$. Replacing \eqref{eq.term1a} and \eqref{eq.term2a} in the statement of Theorem \ref{thm:main_mse_user}, we obtain \eqref{cor.MSE_finite}.
\end{proof}

\medskip
\noindent{\bf $\murow$ is uniform measure.} We consider setting where $\murow$ is uniform Lebesgue measure on $[0,1]^d$, the unit cube in $d$ dimension. 
There exists universal constant $\alpha, \beta > 0$ such that for any $d \geq 1$, and $x \in [0,1]^d$ and $r > 0$, 
\begin{align}
\mbox{Vol}(B(x,r)) & \geq \min(1, \alpha \beta^d  r^d). 
\end{align} 
We state the following implication of Theorem \ref{thm:main_mse_user} in this setting. 
\begin{coro}[Unit cube and the Lebesgue measure]\label{coro:uniform}
Let $\murow$ be uniform measure on $\latsprow = [0,1]^d$. Let 
$$\eta = \eta' +  K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big), \quad\mbox{and}$$
$$ \eta' = 2 \sigma^2 +  \alpha^{2/d} \beta^2 L^2 \Big((m-1)p\Big)^{-\frac{2}{d+2}},$$
%
%(LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}.$$ 
where $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$.  If $p \geq \max\Bigg(\frac{8}{m-1}, \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}\Bigg)$, then
\begin{align}\label{cor.MSE_uniform}
	\MSE(\hat{A}) 
		&\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \bigg)
		+ C' \alpha^{2/d} \beta^2 L^2 \big[ (m-1)p \big]^{-\frac{2}{d+2}}
		+  \exp\Big( - \frac{1}{8} \big[ (m-1)p \big]^{\frac{2}{d+2}} \Big)
\end{align}
where $C, C', c > 0$ are absolute constants.
\end{coro}
That is, as long as $p \gg \max\Bigg(\frac{1}{m}, \sqrt{\frac{\log m}{n}}\Bigg)$, under uniform measure 
\[	\MSE(\hat{A}) = O \Bigg( (LD + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee L^2 \Big(\frac{1}{(m-1)p}\Big)^{\frac{2}{d+2}} \Bigg).	\]
\begin{proof}[Proof of Corollary \ref{coro:uniform}]
Similar to proof of Corollary \ref{coro:finite}, our interest is in bounding \eqref{eq.term1} and \eqref{eq.term2}. To that end, under
%uniform Lebesgue measure, $\murow$, on $d$ dimensional unit cube $\lastprow$, it follows that for any $x \in \lastprow$ and $r > 0$
\begin{align}
\localprob(x, r) & \geq \min\Big(1, \alpha \beta^d r^d\Big), 
\end{align}
where $C(d)$ is constant that is dependent on $d$, precisely exponentially small in $d$. Therefore, by choice of $\eta'$
\begin{align}\label{eq.term1b}
\bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg] 
& \leq \frac{1}{(m-1)p} \times \frac{\alpha \beta^d L^d}{(\eta' - 2\sigma^2)^{d/2}} \nonumber \\
& = \Big((m-1)p\Big)^{-\frac{2}{d+2}}.
\end{align}
Similarly, 
\begin{align}\label{eq.term2b}
\bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg] 
& \leq \exp\bigg( - \frac{(m-1)p}{8}  \times \frac{(\eta' - 2\sigma^2)^{d/2}}{\alpha \beta^d L^d}\bigg) \nonumber \\
& \leq \exp\bigg( - \frac18 \Big((m-1)p\Big)^{\frac{2}{d+2}}\bigg).
\end{align}
From \eqref{eq.term1b} and \eqref{eq.term2b}, and statement of Theorem \ref{thm:main_mse_user}, we conclude \eqref{cor.MSE_uniform}.
\end{proof}



\medskip
\noindent{\bf $\murow$ is any measure on a Polish space.} Let $\murow$ be {\em any} measure on $\latsprow$, where
$\latsprow$ is a complete, separable metric space aka Polish space\footnote{Recall that a metric space is separable if it has countable dense set, and 
complete if every Cauchy sequence converges within the space.}. An importance consequence is that $\murow$ is {\em tight},
i.e. for any $\varepslilon > 0$, there exists a compact set $S_\varepslilon \subset \latsprow$ such that $\murow(S_\varepslilon) \geq 1-\varepslilon$. And subsequently, for any $r > 0$, there exists finite collection $\{B(x_i,r ) : x_i \in  \latsprow, i \in I\}$
so that $S \subset \cup_{i \in I} B(x_i, r)$. That is, the effective covering number $




%
%
%
%\subsection{Two Examples Given Local Geometry of Latent Probability Measure}
%Observe that the upper bound on the MSE in Theorem \ref{thm:main_mse_user} consists of multiple terms. Ideally, we want to choose 
%$\eta \to 2\sigma^2$ so that the first term vanishes, however, that leads to $\msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \to 0$ and 
%the inflation of the terms $2 \Big[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \Big]^{-1}$ and 
%$ \exp\Big( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \Big)$. Therefore, we want to find the best upper bound 
%where the competing terms in the upper bound are balanced.
%
%The ``local geometry'' of the probability measure $\murow$ on the latent space $\latsprow$ through the function $\msrrow$ determines 
%the impact of the latent space dimension on the sample complexity and error convergence rate of the user-user $k$-nearest neighbor algorithm. 
%We consider two examples -- discrete probability measure with finite support and the Lebesgue measure on the unit cube in $\Reals^d$ -- to 
%illustrate the impact. 
%
%%Since the algorithm is a neighbor-based method, we need to guarantee that for each row $u \in [m]$, there are sufficiently many rows $v \in \rowbase$ such that the variances of their row differences are small, which we showed in section \ref{sec:taylor} intuitively implies bounds on $|\hat{A}_{vj}(u,i) - \hat{A}(u,i)|$ for the average column $j$. By our model assumption that the matrix $A$ is described by an $L$-Lipschitz function $f$, it is sufficient to show that with high probability, there exists sufficiently many rows $v \in \rowbase$ such that $d_{\cX_1}(x_1(u), x_1(v))$ is small, which implies the differences in their functional values are small, and thus the sample variance of their differences is also small. This is directly related to the function $\phi_1$, since it lower bounds the probability for the latent variable $x_1(v)$ to be sampled within a $r$-radius ball around $x_1(u)$ such that $d_{\cX_1}(x_1(u), x_1(v)) < r$.
%
%In the simple setting where $\murow$ is supported only on a finite number of points, i.e. there are only finitely many latent row 
%types, the convergence rate of the MSE upper bound and the sample complexity have {\em no} dependency on dimension of the latent 
%spaces. This follows from the fact that $\msrrow(r) \geq \min_{x \in \latsprow} \murow(x)$ even when $r \to 0$. Corollary \ref{coro:finite} presents the simplified 
%MSE upper bound for the finite support setting.
%
%\begin{coro}[Finite support]\label{coro:finite}
%Suppose that $\latsprow$ is equipped with the discrete metric\footnote{$\drow(x_1, x_2) = 1$ if and only if $x_1 \neq x_2$.} topology and $\murow$ has finite support 
%in $\latsprow$. Let $\pmin \triangleq \min_{x \in \supp~ \murow} \murow(x)$. Let $\hat{A}$ be the output of our user-user $k$-nearest neighbor algorithm using a threshold parameter of $\eta \geq \eta' + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, 
%\frac{4 \log (m-1)}{c(n-1)p^2} \Big)$ for some $\eta' \geq 2 \sigma^2$. If $p \geq \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \sqrt{\frac{\log(m-1)}{n-1}}$, 
%then
%\begin{equation*}\label{eqn:MSE_finite}
%	\MSE(\hat{A}) 
%		\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2}, \frac{2}{m-1} \bigg)
%		+ \frac{2}{\pmin\cdot (m-1)p} 
%		+  \exp\bigg( - \frac{\pmin}{8} (m-1)p \bigg)
%\end{equation*}
%where $C, c > 0$ are absolute constants. \chris{Do we need to repeat or reference the definition of $K$ again?}
%\end{coro}
%
%\begin{remark}\label{rem:finite}
%When the latent space is a discrete metric space and the underlying measure is supported on a finitely many number of points, 
%\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee \frac{1}{\pmin}\frac{1}{(m-1)p} \Bigg).	\]
%\DG{I believe that $L$ should be removed; but we cannot do that with our current analysis.}
%\end{remark}
%
%\begin{remark}
%	\DG{***TODO: I don't know whether we can do this.}Simplification to
%	\[	\MSE(\hat{A}) = O \Bigg( (\lip + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee | \supp ~ \murow |\frac{1}{(m-1)p} \Bigg).	\]
%\end{remark}
%
%Next, we suppose $\murow$ is the Lebesgue probability measure on the cube of side length $D$ in $\Reals^d$ (i.e. uniform measure on the 
%$d$-dimensional cube). Then for $r > 0$,
%\[
%	\msrrow(r) = \min_{x_0 \in \cX_1} \murow\big( B(x_0, r \big))= \min\left\{1, \Big(\frac{r}{D}\Big)^d\right\}.
%\]
%\begin{remark}[Maximum latent dimension for the neighbor-based algorithm to succeed.]
%Due to the uniform random sampling of the latent features, this expressions shows that we need to sample $\Omega(r^{-d})$ number of rows 
%to guarantee that there is at least one row whose latent feature is within distance $r$ of $x_0$ for all $x_0 \in \latsprow$. Therefore, we 
%require $m \gg r^{-d}$ in the regime $r \to 0$. This implies that we need the dimension of the latent space to satisfy $d = o(\log m)$. 
%\end{remark}
%
%Corollary \ref{coro:uniform} presents a simplified MSE upper bound when the row latent variables are sampled according to the uniform measure on the $d$-dimensional 
%unit cube.
%
%\begin{coro}[Unit cube and the Lebesgue measure]\label{coro:uniform}
%Suppose that $\murow$ is the uniform measure on $\latsprow = [0,1]^d$ and our user-user $k$-nearest neighbor algorithm uses $\eta \geq \eta' + 
%K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$ where $\eta' = 2 \sigma^2 + (LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}$. 
%If $p \geq \Big(4 \vee \sqrt{\frac{2}{c}} \Big)\cdot \frac{4 \sqrt{\log(m-1)}}{\sqrt{n-1}}$, then
%\begin{align*}\label{eqn:MSE_uniform}
%	\MSE(\hat{A}) 
%		&\leq C K \max\bigg( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2}, \frac{2}{m-1} \bigg)
%		+ 3(LD)^{\frac{2d}{d+2}} \big[ (m-1)p \big]^{-\frac{2}{d+2}}
%		+  \exp\Big( - \frac{1}{8} \big[ (m-1)p \big]^{\frac{2}{d+2}} \Big)
%\end{align*}
%where $C, c > 0$ are absolute constants.
%\end{coro}
%
%\begin{remark}\label{rem:uniform}
%When the latent space is a $d$-dimensional cube of side length $D$ equipped with the uniform measure on it, 
%\[	\MSE(\hat{A}) = O \Bigg( (LD + \sigma)^2 \sqrt{\frac{\log (m-1)}{(n-1)p^2}} \vee (LD)^{\frac{2d}{d+2}} \Big(\frac{1}{(m-1)p}\Big)^{\frac{2}{d+2}} \Bigg).	\]
%\end{remark}


==> contents/new_proof/matrix_proof_christina.tex <==
\section{Proof of Theorem \ref{thm:main_mse_user}}\label{sec:proof_main_thm}
\subsection{Outline of the Proof}\label{sec:proof_outline}

There are $m + n + 2mn$ independent sources of randomness in our model, $ \big\{ \featrow{u}\big\}_{u \in [m]}$, 
$\big\{ \featcol{i} \big\}_{i \in [n]}, \big\{ N(u,i) \big\}_{(u,i) \in [m] \times [n]}$,  $\big\{ M(u,i) \big\}_{(u,i) \in [m] \times [n]}$. 
We let $\Frandom$ denote the collection of these random variables. 

Due to the exchangeability of the model and the linearity of the expectation,
\[	\MSE(\hA) = \Exp{\big( \hA(u,i) - A(u,i) \big)^2 }	 = \Exp{\big( \hA(1,1) - A(1,1) \big)^2 }.	 \]
In Theorem \ref{thm:main_mse_user}, we provide an upper bound on $\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1} }$, 
conditioned on the latent feature of the first row.


Recall from Algorithm \ref{alg:user_algorithm} that
\[	\hA(1,1) = 	 \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} Z(v,1) \] 
in our user-user $k$-nearest neighbor algorithm when $\Nbase \geq 1$ and $\hA(1,1) = 0$ when $\Nbase = 0$. Therefore,
\begin{align*}
	\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\big|~ \featrow{1}}
		&= \Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase = 0 }\big) ~\big|~ \featrow{1}} \\
			&\quad	+ \Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase \geq 1 }\big) ~\big|~ \featrow{1}}.
\end{align*}
We observe that 
\begin{align*}
	\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase = 0 }\big) ~\big|~ \featrow{1} }
		&\leq \lip^2  \diamrow^2 \Prob{ \Nbase = 0 ~\big|~ \featrow{1}}
\end{align*}
and that
\begin{align*}
	&\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase \geq 1 }\big) ~\big|~ \featrow{1}}\\
%		&\qquad=  \Exp{ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
%			~\Ind\big( { \Nbase \geq 1 }\big)
%				+ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2
%				~\Ind\big( { \Nbase \geq 1 }\big) }\\
		&\qquad=  \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
			~\Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1} \Bigg]\\
		&\qquad\quad + \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 
				~\Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1}\Bigg]\\
		&\qquad\stackrel{(a)}{\leq}
				\bbE_{\Frandom \setminus \featcol{1} } 
				\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2 
					~\Ind\big( { \Nbase \geq 1 }\big)	~\Big|~ \featrow{1} \bigg]\\
			&\qquad\quad + C \sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~\Ind\big( { \Nbase \geq 1 }\big) ~\Big|~ \featrow{1} \bigg]
\end{align*}
where $C > 0$ is an absolute constant (coming from $\| X \|_{\psi_2} \leftrightarrow \Var(X)$). 
The inequality in (a) follows from Lemmas \ref{lem:signal_MSE_upper} and \ref{lem:noise_MSE_upper}.


We need local properties of the probability measure on the latent space to upper bound the two terms in the last line; 
see Lemmas \ref{lem:signal_technical} and \ref{lem:noise_technical}. 
Also, we prove in Lemma \ref{lem:prob_zero} that 
\begin{align*}
	\Prob{\Nbase = 0 ~\big|~ \featrow{1}}
		&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)\\
		&\quad	+ \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) \frac{1}{2}(n-1)p^2 \bigg] 
			+ \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}


%%% ==========================================
%%%	Helper Lemma 1: Signal Contribution
%%% ==========================================
\subsection{Upper Bounding the Contribution of Signal on MSE}
\begin{lemma}\label{lem:signal_MSE_upper}
	\begin{align*}
		&\bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2
		~\Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1} \Bigg]\\
			&\qquad= \bbE_{\Frandom \setminus \featcol{1} } 
				\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2 
				~\Ind\big( { \Nbase \geq 1 }\big)	~\bigg|~ \featrow{1}\bigg].
	\end{align*}
\end{lemma}
\begin{proof}
Recall from Section \ref{sec:proof_outline} that we let $\Frandom$ denote the collection of $m + n + 2mn$ independent sources of randomness 
in our model, $ \big\{ \featrow{u}\big\}_{u \in [m]}$, $\big\{ \featcol{i} \big\}_{i \in [n]}, \big\{ N(u,i) \big\}_{(u,i) \in [m] \times [n]}$,  
$\big\{ M(u,i) \big\}_{(u,i) \in [m] \times [n]}$. 

By the tower property of expectation,
\begin{align*}
	&\bbE_{\Frandom | \featrow{1}}\Bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2	
	~\Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1} \Bigg]\\
		&= \bbE_{\Nbase}\Bigg[ ~ \bbE_{\Frandom \big| \featrow{1}, \Nbase }\bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} 
		\big( A(v,1) - A(1,1) \big) \bigg)^2 ~\Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1}, \Nbase \bigg] ~\Bigg].
\end{align*}
We investigate the conditional expectation, again using the tower property and the fact that $\Nbase$ is fully determined when we condition on $\Frandom \setminus \featcol{1}$. 
For the sake of readability, $\Ind\big( { \Nbase \geq 1 }\big)$ is omitted in the lines below.
\begin{align*}
	&\bbE_{\Frandom \big| \featrow{1}, \Nbase}\bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
		~\bigg|~ \featrow{1}, \Nbase \bigg] \\
		&	= \frac{1}{| \baseest(1,1) |^2} \bbE_{\Frandom \big| \featrow{1}, \Nbase }\bigg[ \bigg(  \sum_{(v,1) \in \baseest(1,1)} 
			\big( A(v,1) - A(1,1) \big) \bigg)^2 ~\bigg|~ \featrow{1}, \Nbase \bigg] \\
		&	\leq \frac{1}{| \baseest(1,1) |^2} \bbE_{\Frandom \big| \featrow{1}, \Nbase }\Bigg[ \Bigg(   \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)} 
			\big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| \Bigg) ~\bigg|~ \featrow{1}, \Nbase \Bigg] \\
		&	\stackrel{(a)}{=} \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \featrow{1}, \Nbase } \Bigg[~ \bbE_{\featcol{1} | \featrow{1}, \Nbase}
			\bigg[\\
			&\qquad \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
			\big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| ~ \Big| ~ \featrow{1}, \Nbase \bigg] ~\bigg|~ \featrow{1}, \Nbase \Bigg]\\
		&	= \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \featrow{1}, \Nbase } \Bigg[ \\
			&\qquad\sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\bbE_{\featcol{1}  \big| \featrow{1} } \Big[ \big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| ~\Big|~ \featrow{1}\Big]
			~\bigg|~ \featrow{1}, \Nbase \Bigg]\\
%		&	\stackrel{(a)}{=} \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \Nbase } 
%		\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
%				\bbE_{\featcol{1} \big| \Frandom \setminus \featcol{1}} \Big[ \big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| ~\Big|~ \Frandom \setminus \featcol{1} \Big]
%			~\bigg|~ \Nbase \Bigg]\\
		&	= \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \featrow{1}, \Nbase } \Bigg[\\
			&\qquad \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\Big\| \big[ f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big] \big[ f(\featrow{v'}, \cdot ) - f(\featrow{1}, \cdot) \big] \Big\|_{L^1}
			~\bigg|~ \featrow{1}, \Nbase \Bigg]\\
		&	\stackrel{(b)}{\leq} \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \featrow{1}, \Nbase } \Bigg[ \\
			&\qquad\sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2} \Big\| f(\featrow{v'}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}
			~\bigg|~ \featrow{1}, \Nbase \Bigg]\\
		&	\leq \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \featrow{1}, \Nbase } 
			\Bigg[ \Nbase^2  \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
			~\bigg|~ \featrow{1}, \Nbase \Bigg]\\
		&	=  \bbE_{\Frandom \setminus \featcol{1} \big| \featrow{1}, \Nbase } 
			\Bigg[ \max_{(v,1) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
			~\bigg|~ \featrow{1},  \Nbase \Bigg].
\end{align*}
%Equation (a) follows from the independence between $\baseest(1,1)$ and $\featcol{1}$ in our user-user $k$-nearest neighbor algorithm; 
Equation (a) follows from the conditional independence, and (b) follows from Cauchy-Schwarz inequality.

Consequently, it follows that 
\begin{align*}
	&\bbE\Bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 \Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1}\Bigg]\\
		&\qquad= \bbE_{\Frandom \setminus \featcol{1} } 
			\Bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2 \Ind\big( { \Nbase \geq 1 }\big) ~\bigg|~ \featrow{1} \Bigg].
\end{align*}
\end{proof}

\DG{resume here}

\begin{lemma}\label{lem:signal_technical}
Let $\eta \geq 2\sigma^2$. The following inequality holds for user-user $k$-nearest neighbor algorithm:
	\begin{align*}
		&\bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \max_{(v,1) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
			\Ind\big( { \Nbase \geq 1 }\big)	\bigg]\\
			&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{\sqrt{2 c (n-1)p^2}} + \frac{2K e^{-\frac{c}{2} (n-1)p^2}}{c (n-1)p^2}
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg) \exp\Big( - \frac{(n-1)p^2}{8} \Big)\\
			&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c' (n-1)p^2\big) \bigg].
	\end{align*}
In the above expression, $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$ and $C, c, c' > 0$ are absolute constants. 
\end{lemma}
\begin{proof}
\textbf{Step 1:}
Choose $v \in [m] \setminus \{1\}$ such that $(v,1) \in \baseest(1,1)$. Observe that 
\[
	\dissimrow(1,v) = \frac{1}{|\basesim(1) \cap \basesim(v)|} \sum_{j \in \basesim(1) \cap \basesim(v)} \big( Z(1,j) - Z(v,j) \big)^2.
\] 
Note that $Z(1,j) - Z(v,j) = \big( X(1,j) -X(v,j) \big) + \big( N(1,j) - N(v,j) \big)$. By the model assumptions, we have
\begin{align*}
	&|X(1,j) - X(v,j)| \leq \lip \diamrow \quad\forall v, j	\qquad \Rightarrow \qquad \big\| X(1,j) - X(v,j) \big\|_{\psi_2} 
		\leq \frac{\lip \diamrow}{\sqrt{\ln 2}},\\
	&\big\| N(1,j) - N(v,j) \big\|_{\psi_2} \leq \big\| N(1,j) \big\|_{\psi_2} + \big\| N(v,j) \big\|_{\psi_2} = 2\sigma.
\end{align*}
Therefore (cf. \cite[Lemma 2.7.6]{vershynin2018high}),
\begin{align*}
	\big\| Z(1,j) - Z(v,j) \big\|_{\psi_2} &\leq \big\| X(1,j) - X(v,j) \big\|_{\psi_2} + \big\| N(1,j) - N(v,j) \big\|_{\psi_2} 
		\leq  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma,\\
	\big\| \big(Z(1,j) - Z(v,j) \big)^2 \big\|_{\psi_1} &= \big\| Z(1,j) - Z(v,j) \big\|_{\psi_2}^2
		\leq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2.
\end{align*}

\chris{Let $K$ denote an upper bound on $\big\| Z(1,j) - Z(v,j) \big\|_{\psi_2}$, then we can write all subsequent results as a function of $K$. The above argument upper bounds $K$ using the Lipschitz condition. Without Lipschitz, simply bounded entries of $X$ would be sufficient (e.g. finite types)}

For notational conciseness, we let $f_{1v}^2$ denote the conditional expectation of $\dissimrow(1,v)$:
\begin{equation}\label{eqn:exp_dissim}
	f_{1v}^2 \triangleq \Exp{\dissimrow(1,v) | \featrow{1},\featrow{v}} 
		= \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 + 2\sigma^2.
\end{equation}
Now, suppose that $|\basesim(1) \cap \basesim(v)| = N_v$. We observe that 
$\Exp{\dissimrow(1,v) | \featrow{1},\featrow{v}, |\basesim(1) \cap \basesim(v)| = N_v} = f_{1v}^2$ regardless of $N_v$. 
Then it follows from Bernstein's inequality (cf. \cite[Theorem 2.8.2]{vershynin2018high}) that for any $t \geq 0$,
\begin{equation}\label{eqn:conc_dissim}
	\Prob{ \dissimrow(1,v) - f_{1v}^2 \leq - t ~ \Big|~ \featrow{1}, \featrow{v}, |\basesim(1) \cap \basesim(v)| = N_v} 
		\leq \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) N_v \bigg].
\end{equation}
By plugging in the value of $f_{1v}^2$, this leads to the following inequality: for any $t \geq 0$,
\begin{align*}
	\Prob{  \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 \geq \dissimrow(1,v) - 2\sigma^2 + t  
		~ \Big|~ |\basesim(1) \cap \basesim(v)| = N_v}
		&\leq  \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) N_v \bigg].	
\end{align*}
Note that we provided an upper bound on the conditional probability in \eqref{eqn:conc_dissim} that holds for 
any realization of $\featrow{1}$ and $\featrow{v}$, and thus we could remove the conditioning on $\featrow{1}$ and $\featrow{v}$.

For later use, we remark here that we can also obtain the concentration inequality for the other side by similar arguments:
\begin{equation}\label{eqn:conc_dissim2}
	\Prob{ \dissimrow(1,v) - f_{1v}^2 \geq t ~ \Big|~ \featrow{1}, \featrow{v}, |\basesim(1) \cap \basesim(v)| = N_v} 
		\leq \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) N_v \bigg].
\end{equation}


\textbf{Step 2:} Let $v^* \in [m] \setminus \{1\}$ denote the maximizer such that $(v^*, 1) \in \baseest(1,1)$ and 
\[	\Big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
		= \max_{(v,1) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2.	\]
According to the description of our user-user $k$-nearest neighbor algorithm, $\dissimrow(1,v^*) \leq \eta$.
\begin{align}
	&\bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \max_{(v,i) \in \baseest(1,1) } \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	\bigg]	\nonumber\\
		&\qquad= \bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	\bigg]	\nonumber\\
		&\qquad= \bbE_{N_v }  \Bigg[ \int_0^{\infty}
			\bbP\bigg( \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	 \geq s 
			~ \Big| ~  |\basesim(1) \cap \basesim(v)| = N_v \bigg) ~ds \Bigg].	\label{eqn:upper_signal_term.1}
\end{align}

Now we observe that 
\begin{align}
	& \int_0^{\infty} \bbP\bigg( \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	 \geq s 
			~ \Big| ~  |\basesim(1) \cap \basesim(v)| = N_v \bigg) ~ds	\nonumber\\
		&\qquad\leq \int_0^{\eta - 2\sigma^2} ds
			+ \int_{0}^{K} \exp \bigg[ -c N_v \frac{t^2}{K^2} \bigg] ds
			+ \int_{K}^{\infty} \exp \bigg[ -c N_v \frac{t}{K} \bigg] ds	\nonumber\\
		&\qquad\leq \big( \eta - 2\sigma^2 \big) 
			+ \int_{0}^{\infty} \exp \bigg[ -c N_v \frac{t^2}{K^2} \bigg] ds
			+ \int_{K}^{\infty} \exp \bigg[ -c N_v \frac{t}{K} \bigg] ds	\nonumber\\
		&\qquad= \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v}.	\label{eqn:upper_signal_term.2}
\end{align}
Recall that for $a > 0$ and $b \in \Reals$,
\[	
	\int_0^{\infty} e^{-a x^2} dx = \frac{1}{2}\sqrt{\frac{\pi}{a}}
	\qquad\text{and}\qquad
	\int_b^{\infty} e^{-a x} dx = \frac{1}{a}e^{-ab}.	
\]
%\DG{***TODO - The following must be made a formal argument:}
%Since $N_v$ sharply concentrates to $(n-1)p^2$, the upper bound in \eqref{eqn:upper_signal_term.1} (using \eqref{eqn:upper_signal_term.2}) 
%becomes
%\[	 \big( \eta - 2\sigma^2 \big)
%			+ CK \bigg[  \frac{ \sqrt{\pi}}{2\sqrt{c (n-1) p^2}} + \frac{e^{-c (n-1)p^2}}{c (n-1)p^2} \bigg].	\]

\textbf{Step 3:} Observe that $ |\basesim(1) \cap \basesim(v)| \sim \textrm{Binomial}(n-1, p^2)$. By the binomial Chernoff theorem,
\begin{equation}\label{eqn:overlap_lower}
	\Prob{ |\basesim(1) \cap \basesim(v)| \leq \frac{1}{2} (n-1)p^2} \leq \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{equation}
Therefore, with the shorthand notation $N_v = |\basesim(1) \cap \basesim(v)|$, we can see that
\begin{align*}
	&\bbE \Bigg[ \big( \eta - 2\sigma^2 \big)	+ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} \Bigg]\\
		&\qquad= \big( \eta - 2\sigma^2 \big)
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v > \frac{1}{2} (n-1)p^2 \bigg]
			\Prob{N_v > \frac{1}{2} (n-1)p^2}\\
			&\qquad\quad
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v \leq \frac{1}{2} (n-1)p^2 \bigg]
			\Prob{N_v \leq \frac{1}{2} (n-1)p^2}\\
		&\qquad\stackrel{(a)}{\leq} \big( \eta - 2\sigma^2 \big)
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v > \frac{1}{2} (n-1)p^2 \bigg]\\
			&\qquad\quad
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg)
			\Prob{N_v \leq \frac{1}{2} (n-1)p^2}\\
		&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{\sqrt{2 c (n-1)p^2}} + \frac{2K e^{-\frac{c}{2} (n-1)p^2}}{c (n-1)p^2}
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg) \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
The inequality in (a) follows from that $N_v \geq 1$ and $\frac{K e^{-c N_v}}{cN_v}$ is maximized when $N_v = 1$.
\end{proof}




%%% ==========================================
%%%	Helper Lemma 2: Noise Contribution
%%% ==========================================

\subsection{Upper Bounding the Contribution of Noise on MSE}
%We take the convention that $\frac{0}{0} = 0$. This is easily justified by defining our estimate $\widehat{A}(1,1) = 0$ when $\Nbase = 0$.
\begin{lemma}\label{lem:noise_MSE_upper}
	\begin{align*}
		 \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2~\Ind\big( { \Nbase \geq 1 }\big) \Bigg]
		 	&\leq C\sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~\Ind\big( { \Nbase \geq 1 }\big) \bigg].
	\end{align*}
\end{lemma}
\begin{proof}
By the tower property of expectation,
\begin{align*}
	& \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2~\Ind\big( { \Nbase \geq 1 }\big) \Bigg]\\
	 	&\qquad = \bbE\Bigg[ ~ \bbE\bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2
			~\Ind\big( { \Nbase \geq 1 }\big) ~ \bigg|~ \Nbase \bigg] ~\Bigg]\\
		&\qquad \leq \bbE\Bigg[ ~ \bbE\bigg[  \frac{1}{| \baseest(1,1) |} \max_{(v,1) \in \baseest(1,1) } | N(v,1) |^2
			~\Ind\big( { \Nbase \geq 1 }\big) ~ \bigg|~ \Nbase \bigg] ~\Bigg]\\
		&\qquad \leq \bbE\Bigg[ ~  \frac{1}{| \baseest(1,1) |}~  \bbE\Big[ ~C \sigma^2 ~ \Big|~ \Nbase \Big]
			~ \Ind\big(\Nbase \geq 1\big) ~\Bigg]	\\
		&\qquad \leq C\sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg].
\end{align*}
\end{proof}


\begin{lemma}\label{lem:noise_technical}
	Let $\eta' \geq 2\sigma^2$ and $\eta \geq \eta' + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$. 
	The following inequality holds for user-user fixed radius nearest neighbor algorithm:
	\begin{align*}
		\bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  ~ \Big| ~  \featrow{1} \bigg]
			&\leq 2 \bigg[  (m-1)p \cdot \phi(\featrow{1}, \eta'-2\sigma^2)  \bigg]^{-1}	+ \frac{1}{m-1} \\
				&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
				+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
%
%
%
%			&\leq 2 \bigg[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg]^{-1}	+ \frac{1}{m-1} \\
%				&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)
%				+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
	\end{align*}
where $\phi(\featrow{1}, r) = \Prob{\big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq r ~|~ \featrow{1}}$  for any $x \in \latsprow$ and $r \geq 0$.
\end{lemma}

%\DG{***TODO:}
%We expect $| \baseest(1,1) | \gtrsim (m-1)p~ \msra{ \frac{\sqrt{\eta - 2\sigma^2}}{\lip} }$

\begin{proof}
\textbf{Step 1:}
%% old proof
%
%
%Let $\eta' = \eta - K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.
%For each $v \in [m] \setminus \{ 1 \}$, the following two conditions
%\begin{equation}\label{eqn:cond_good_row}
%	M(v,1) = 1	\qquad\text{and}\qquad  \drow(\featrow{1}, \featrow{v}) \leq \frac{\sqrt{\eta' - 2\sigma^2}}{L}
%\end{equation}
%are satisfied with success probability\footnote{Note that the first condition solely depends on $M(v,1)$, while the second condition 
%depends only on $\featrow{1}, \featrow{v}$, hence, they are independent events.} at least 
%$p \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big)$. Let $\goodrows \subset [m] \setminus \{1 \}$ denote the set of row indices 
%that satisfy the two conditions described in \eqref{eqn:cond_good_row}. By the binomial Chernoff bound,
%\begin{equation}\label{eqn:upper_noise_term.1}
%	\Prob{ |\goodrows| \leq \frac{1}{2} (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) }
%		\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg).
%\end{equation}
%
%
%% 
\chris{Instead of depending on the representation, let us consider quantities in terms of the $L_2$ distance itself ...}
\begin{align*}
\phi(\featrow{1}, r) = \Prob{\big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq r ~|~ \featrow{1}}
\end{align*}

Our interest is in bounding conditional expectation of $\frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)$ given 
$\featrow{1} \in \latsprow$. To that end, let us fix $\featrow{1}$.  
%
Let $\eta' = \eta - K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.
For each $v \in [m] \setminus \{ 1 \}$, the following two conditions
%\begin{equation}\label{eqn:cond_good_row}
	%M(v,1) = 1	\qquad\text{and}\qquad  \drow(\featrow{1}, \featrow{v}) \leq \frac{\sqrt{\eta' - 2\sigma^2}}{L}
%\end{equation}
\chris{
\begin{equation}\label{eqn:cond_good_row}
	M(v,1) = 1	\qquad\text{and}\qquad  \big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq \eta' - 2\sigma^2
\end{equation}
}
are satisfied with success probability\footnote{Note that the first condition solely depends on $M(v,1)$, 
while the second condition depends only on $\featrow{1}, \featrow{v}$, hence, they are independent events.} 
$p \cdot \phi(\featrow{1}, \eta'-2\sigma^2)$.

\chris{For Lipschitz setting, $\drow(\featrow{1}, \featrow{v}) \leq \frac{\sqrt{\eta' - 2\sigma^2}}{L}$ implies $\big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq \eta' - 2\sigma^2$ therefore we can lower bound $\phi(\featrow{1}, \eta'-2\sigma^2)$ with 
$\murow\big( B(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L} \big)) = \localprob\big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\big)$.}

Let $\goodrows \subset [m] \setminus \{1 \}$ denote the set of row indices 
that satisfy the two conditions described in \eqref{eqn:cond_good_row}. By the binomial Chernoff bound, 
\begin{equation}\label{eqn:upper_noise_term.1}
	\Prob{ |\goodrows| \leq \frac{1}{2} (m-1)p  \cdot \phi(\featrow{1}, \eta'-2\sigma^2) ~ \bigg|~ \featrow{1} }
		\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg).
\end{equation}







\textbf{Step 2:}
Next, we want to show that $\{(v,1): v \in \goodrows\} \subset \baseest(1,1)$ with high probability.
For that purpose, we first require $|\basesim(1) \cap \basesim(v) |$ to be sufficiently large for all $v \in \goodrows$. Observe that 
for each $v \in \goodrows$, $|\basesim(1) \cap \basesim(v) |$ is distributed following $\textrm{Binomial}(n-1, p^2)$. Again by the binomial 
Chernoff bound (as in \eqref{eqn:overlap_lower}), we have 
\[	\Prob{|\basesim(1) \cap \basesim(v)| \leq \frac{(n-1)p^2}{2}} \leq \exp \Big( - \frac{(n-1)p^2}{8} \Big).	\]
Since $|\goodrows| \leq m-1$, it follows from the union bound that 
\begin{equation}\label{eqn:upper_noise_term.2}
	\Prob{ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| \leq \frac{(n-1)p^2}{2}} \leq (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
\end{equation}

By \eqref{eqn:conc_dissim2} and another application of the union bound, this implies that 
\begin{align*}
	&\Prob{ \max_{v \in \goodrows }\dissimrow(1,v) \geq \eta' + t ~\bigg| ~ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2}}\\ 
		&\qquad\leq (m-1)  \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) \frac{(n-1)p^2}{2} \bigg].
\end{align*}
Therefore\footnote{Recall that $\eta' = \eta - t$ with $t = K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.},
\begin{equation}\label{eqn:upper_noise_term.3}
	\Prob{ \max_{v \in \goodrows }\dissimrow(1,v) \geq \eta ~\bigg| ~ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2}}
		\leq \frac{1}{m-1}.
\end{equation}
Observe that 
\begin{equation}\label{eqn:upper_noise_term.4}
	\text{if}\quad
	\max_{v \in \goodrows }\dissimrow(1,v) \leq \eta
	\qquad\text{then}\quad
	\{(v,1): v \in \goodrows\} \subset \baseest(1,1),
\end{equation}
which implies that $|\baseest(1,1)| \geq |\goodrows|$.

\textbf{Step 3:}
Let 
\begin{align*}
	\Eva	&\triangleq \bigg\{  |\goodrows| > \frac{1}{2} (m-1)p  \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg\}\\
	\Evb	&\triangleq \bigg\{  \max_{v \in \goodrows }\dissimrow(1,v) \leq \eta  \bigg\},\\
	\Evc	&\triangleq \bigg\{  \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2} \bigg\}.
\end{align*}
By the law of total probability,
\begin{align*}
	~& \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~ \featrow{1} \bigg]  \\
	~	& \qquad \stackrel{(a)}{\leq} \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~\featrow{1},  \Eva \cap \Evb  \bigg] \Prob{\Eva \cap \Evb} 
			+ \Prob{\Eva^c \cup \Evb^c }\\
	~	&\qquad \leq \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~ \featrow{1}, \Eva \cap \Evb  \bigg] 
			+ \Prob{\Eva^c} + \Prob{\Evb^c|\Evc} + \Prob{\Evc^c}\\
	~	&\qquad  \stackrel{(b)}{\leq}
			2 \bigg[  (m-1)p  \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg]^{-1}	+ \frac{1}{m-1} \\
				&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
				+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big)
\end{align*}
where (a) follows from $ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) \leq 1$; and (b) follows from that \eqref{eqn:upper_noise_term.4} and
\begin{align*}
	\Prob{\Eva^c}	&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg),
			&\because \eqref{eqn:upper_noise_term.1}\\
	\Prob{\Evb^c|\Evc} &\leq	\frac{1}{m-1},		
			&\because \eqref{eqn:upper_noise_term.3}\\
	\Prob{\Evc^c}	&\leq (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).		
			&\because\eqref{eqn:upper_noise_term.2}
\end{align*}

\end{proof}



%\subsection{Completing the Proof of Theorem \ref{thm:main_mse_user}}
%\chris{This section is repeated from the outline (Part A), but that's okay right?}
%\begin{proof}[Proof of Theorem \ref{thm:main_mse_user}]
%Due to the exchangeability of the model and the linearity of the expectation,
%\[	\MSE(\hA) = \Exp{\big( \hA(u,i) - A(u,i) \big)^2 }	 = \Exp{\big( \hA(1,1) - A(1,1) \big)^2 }.	 \]
%Recall from Algorithm \ref{alg:user_algorithm} that
%\[	\hA(1,1) = 	 \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} Z(v,1) \] 
%in our user-user $k$-nearest neighbor algorithm when $\Nbase \geq 1$ and $\hA(1,1) = 0$ when $\Nbase = 0$. Therefore,
%\begin{align*}
%	\Exp{\big( \hA(1,1) - A(1,1) \big)^2 }
%		&= \Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase = 0 }\big) } 
%				+ \Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase \geq 1 }\big) }.
%\end{align*}
%We observe that 
%\begin{align*}
%	\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase = 0 }\big) }
%		&\leq \lip^2  \diamrow^2 \Prob{ \Nbase = 0 }
%\end{align*}
%and that
%\begin{align*}
%	&\Exp{\big( \hA(1,1) - A(1,1) \big)^2 ~\Ind\big( { \Nbase \geq 1 }\big) }\\
%%		&\qquad=  \Exp{ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
%%			~\Ind\big( { \Nbase \geq 1 }\big)
%%				+ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2
%%				~\Ind\big( { \Nbase \geq 1 }\big) }\\
%		&=  \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
%			~\Ind\big( { \Nbase \geq 1 }\big)\Bigg]\\
%		&\qquad		+ \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 
%				~\Ind\big( { \Nbase \geq 1 }\big)\Bigg]\\
%		&\stackrel{(a)}{\leq}
%				\bbE_{\Frandom \setminus \featcol{1} } 
%				\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2 
%					~\Ind\big( { \Nbase \geq 1 }\big)	\bigg]
%			+ C \sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~\Ind\big( { \Nbase \geq 1 }\big)  \bigg]
%\end{align*}
%where $C > 0$ is an absolute constant (coming from $\| X \|_{\psi_2} \leftrightarrow \Var(X)$). 
%The inequality in (a) follows from Lemmas \ref{lem:signal_MSE_upper} and \ref{lem:noise_MSE_upper}.
%
%We need local properties of the probability measure on the latent space to upper bound the two terms in the last line. By Lemma 
%\ref{lem:signal_technical}, when $\eta \geq 2\sigma^2$:
%\begin{align*}
%	&\bbE_{\Frandom \setminus \featcol{1} } 
%		\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
%			~\Ind\big( { \Nbase \geq 1 }\big)	\bigg]\\
%		&\qquad\leq \big( \eta - 2\sigma^2 \big)
%		+ CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg].
%\end{align*}
%Moreover, when $\eta' \geq 2\sigma^2$ and $\eta \geq \eta' + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$, 
%it follows from Lemma \ref{lem:noise_technical} that
%\begin{align*}
%	\bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg] & = \bbE_{ \featrow{1}} \Bigg[  \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~ \featrow{1} \bigg] \Bigg] \\
%		&\leq 2 \bbE_{ \featrow{1}} \Bigg[ \bigg[  (m-1)p  \cdot  \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg]^{-1}\Bigg]+ \frac{1}{m-1} \\
%			&+ \bbE_{ \featrow{1}}\Bigg[ \exp\bigg( - \frac{(m-1)p}{8} \cdot \localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg) \Bigg]
%			+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
%\end{align*}
%Putting above together, we obtain statement of Theorem \ref{thm:main_mse_user}.
%\end{proof}


%%% ==========================================
%%%	Helper Lemma 3: Failure Probability
%%% ==========================================

\subsection{Upper Bounding the Probability of $\Nbase = 0$}

\begin{lemma}\label{lem:prob_zero}
Let $\eta' \geq 2\sigma^2$ and $\eta \geq \eta' + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$. 
The following inequality holds for user-user $k$-nearest neighbor algorithm:
\begin{align*}
	\Prob{\Nbase = 0 ~\big|~ \featrow{1}}
		&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
			+ \frac{1}{(m-1)^2} + \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
\end{lemma}
\begin{proof}
Recall the definition of $\goodrows$ from \eqref{eqn:cond_good_row}:
\[	\goodrows = \left\{ v \in [m] \setminus \{1 \} ~\text{ such that }~
		M(v,1) = 1	~\text{ and }~  \big\| f(\featrow{1}, \cdot) - f(\featrow{v}, \cdot) \big\|_{L^2}^2 \leq \eta' - 2\sigma^2 \right\}.	\]
Note that we obtain in \eqref{eqn:upper_noise_term.1} that
\[
	\Prob{ |\goodrows| \leq \frac{1}{2} (m-1)p  \phi(\featrow{1}, \eta'-2\sigma^2) ~\bigg|~ \featrow{1} }
		\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
\]
by applying the binomial Chernoff bound.

Now we observe that if there exists at least one $v \in \goodrows$, for which 
\[	\dissimrow(1,v) - \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 - 2\sigma^2 \leq \eta - \eta', 	\]
then $\dissimrow(1,v) \leq \eta$ and thus $\Nbase \geq 1$. Therefore, we have 
\begin{align}
	\Prob{\Nbase = 0}
		&\leq \Prob{ |\goodrows| = 0 } \nonumber\\
		&\quad + \Prob{ \dissimrow(1,v) - \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 - 2\sigma^2 \leq \eta - \eta', ~~ \forall v \in \goodrows} \Prob{ |\goodrows| \geq 1 }\nonumber\\
		&\leq \Prob{ |\goodrows| = 0 } + \Prob{ \dissimrow(1,v_0) - \big\|  f(\featrow{v_0}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 - 2\sigma^2 \leq \eta - \eta' } \label{eq:prob_0_term.1}
\end{align}
where $v_0 = \min \{ v \in \goodrows \}$.

We bound the two terms in \eqref{eq:prob_0_term.1} separately. First, as long as $\localprob\Big(\featrow{1}, \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) > 0$, it follows from \eqref{eqn:upper_noise_term.1} that
\begin{align*}
	\Prob{ |\goodrows| = 0 ~\big|~ \featrow{1} }
		&\leq \Prob{ |\goodrows| \leq \frac{1}{2} (m-1)p  \cdot \phi(\featrow{1}, \eta'-2\sigma^2) ~\bigg|~ \featrow{1}}\\
		&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg).
\end{align*}
Second, by the usual trick of total probability (recall from \eqref{eqn:exp_dissim} that $f_{1v_0}^2$ denotes 
$\Exp{\dissimrow(1,v_0) | \featrow{1}, \featrow{v_0}}$),
\begin{align*}
	&\Prob{ \dissimrow(1,v_0) - f_{1v_0}^2 \leq \eta - \eta' ~\big|~ \featrow{1}}\\
		&\qquad\leq \Prob{ \dissimrow(1,v_0) - f_{1v_0}^2 \leq \eta - \eta' ~\Big|~ \featrow{1}, |\basesim(1) \cap \basesim(v_0)| \geq \frac{1}{2}(n-1)p^2 }\\
		&\qquad\quad
			+ \Prob{  |\basesim(1) \cap \basesim(v_0)| < \frac{1}{2}(n-1)p^2 ~\bigg|~ \featrow{1}}\\
	&\qquad\stackrel{(a)}{\leq} \exp \bigg[ -c \min \Big( \frac{(\eta - \eta')^2}{K^2}, \frac{\eta - \eta'}{K} \Big) \frac{1}{2}(n-1)p^2 \bigg] 
		+ \Prob{  |\basesim(1) \cap \basesim(v_0)| < \frac{1}{2}(n-1)p^2 }\\
	&\qquad\stackrel{(b)}{\leq} \exp \big[ -2 \log(m-1) \big] 
		+ \exp\Big( - \frac{(n-1)p^2}{8} \Big)	
\end{align*}
where (a) follows from \eqref{eqn:conc_dissim} and the independence between $|\basesim(1) \cap \basesim(v_0)|$ and $\featrow{1}$; 
and (b) follows from \eqref{eqn:overlap_lower} and the assumption that $\eta - \eta' \geq K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.

All in all, 
\begin{align*}
	\Prob{\Nbase = 0 ~\big|~ \featrow{1}}
		&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \phi(\featrow{1}, \eta'-2\sigma^2) \bigg)
			+ \frac{1}{(m-1)^2} + \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
\end{proof}

\newpage


==> contents/new_proof/new_proof.tex <==
\section{New Version of Algorithm and Proof}
%\subsection{Model Assumption}
%Our data matrix $Y$ is an $m \times n$ matrix that is generated as follows. For each $(u,i) \in [m] \times [n]$,
%\[	Y(u,i) = \big( A(u,i) + N(u,i) \big) \circ M(u,i).	\]
%Here, $A \in \Reals^{m \times n}$ denotes the signal matrix, $N \in \Reals^{m \times n}$ denotes the noise matrix, 
%and $M \in \{0, 1\}^{m \times n}$ denotes the masking matrix. For each $(u,i) \in [m] \times [n]$, 
%\[
%	Y(u,i) = \begin{cases}
%			A(u,i) + N(u,i)	&	\text{when }M(u,i) = 1,\\
%			\text{unknown}	&	\text{when }M(u,i) = 0.
%		\end{cases}
%\]
%Let $\Omega \triangleq \{ (u,i) \in [m] \times [n]: M(u,i) = 1 \}$. 
%
%\subsubsection{Latent Variable Model}
%We assume $A(u,i)$ is generated by the following model:
%\begin{itemize}
%	\item
%	Nonparametric model: there exists a latent function $f$ such that
%	\[	A(u,i) = f( \featrow{u}, \featcol{i})	\]
%	for all $(u,i) \in [m] \times [n]$. Here, $\featrow{u}, \featcol{i}$ denote latent varialbes associated with row $u$ 
%	and column $i$, respectively.
%	\item
%	Regularity Assumptions
%	\begin{itemize}
%		\item
%		For all $u \in [m]$, $\featrow{u} \in \latsprow$, where $(\latsprow, \drow)$  is a metric space such that 
%		$\diam \latsprow = \sup_{\alpha, \alpha'} \drow(\alpha, \alpha') \leq \diamrow$. 
%		Moreover, $\latsprow$ is equipped with a Borel probability measure $\murow$.
%		\item
%		For all $i \in [n]$, $\featcol{i} \in \latspcol$, where $(\latspcol, \dcol)$  is a metric space such that 
%		$\diam \latspcol = \sup_{\beta, \beta'} \dcol(\beta, \beta') \leq \diamcol$. 
%		Moreover, $\latspcol$ is equipped with a Borel probability measure $\mucol$.
%		\item
%		Latent function $f$ is $\lip$-Lipschitz in the sense that 
%		\[	\big| f( \alpha_1, \beta_1) - f( \alpha_2, \beta_2) \big|
%				\leq \lip \max \big( \drow(\alpha_1, \alpha_2), \dcol(\beta_1, \beta_2) \big).	\]
%	\end{itemize}
%\end{itemize}
%
%\subsubsection{Noise}
%We assume $N(u,i)$ is a centered, sub-gaussian random variable for all $(u,i) \in [m] \times [n]$ such that
%\begin{itemize}
%	\item
%	Centered: $\bbE N(u,i) = 0$ for all $(u,i) \in [m] \times [n]$.
%	\item
%	Sub-gaussian: there exists $\sigma > 0$ such that $\| N(u,i) \|_{\psi_2} \leq \sigma$ for all $(u,i) \in [m] \times [n]$.
%	\item
%	Independent and identically distributed: $N(u,i)$'s are independent and identically distributed (due to the exchangeability).
%\end{itemize}
%
%\subsubsection{Masking}
%We assume $M$ is a random matrix with each entry drawn as per $Bernoulli(p)$ for some $p \in (0,1]$, i.i.d. That is, for each 
%$(u,i) \in [m] \times [n]$, 
%\[	
%	M(u,i) = \begin{cases}
%			1	&	\text{with probability }p,\\
%			0	&	\text{with probability }1-p.
%			\end{cases}	
%\]


%\subsection{Algorithm}
%\subsubsection{General Form}
%Our algorithm takes (i) the data matrix $Y$, (ii) rule for sample splitting, and (iii) thresholding parameter $\eta \geq 0$ as its input. 
%The algorithm outputs $\hA \in \Reals^{m \times n}$. 
%\begin{enumerate}
%	\item
%	Split the observations in $\Omega$. 
%	For each $(u,i) \in \Omega$, put it in $\Omega_1$ or $\Omega_2$.
%	
%	\item
%	For each $(u,i) \in [m] \times [n]$, determine the set of reliable neighbors $ \baseest(u,i) \subset \Omega_2$ with 
%	similarity/dissimilarity computed based on $\Omega_1$.
%	
%	\item
%	For each $(u,i) \in [m] \times [n]$, compute $\hA(u,i)$ using $\baseest(u,i)$.
%\end{enumerate}
%
%{\em Remark.} 
%We note that sample splitting is done for the ease of analysis, and is not essential in executing the algorithm.
%
%{\em Remark.} 
%There are many variations in (1) how we determine the set of reliable neighbors (e.g., by defining similarity/dissimilarity functions), 
%and (2) how we compute the final estimate based on the observations at those neighbors.
%
%\subsubsection{Prime Example: User-user $k$-nearest Neighbor (of $0$-th order)}
%Let $(u,i) \in [m] \times [n]$ fixed.
%\begin{enumerate}
%	\item
%	Split the observations in $\Omega$. 
%	For each $(v,j) \in \Omega$, put it in $\Omega_1$ if $j \neq i$, and put it in $\Omega_2$ otherwise.
%	
%	\item
%	Determine the set of reliable neighbors using $\Omega_1$.
%	\begin{itemize}
%		\item
%		For each $v \in [m]$, define 
%		\[	\basesim(v) \triangleq \{ j \in [n]: (v,j) \in \Omega_1  \},	\]
%		which is the base set of $u$ to determine its similarity to other rows.
%		\item
%		For each $v \in [m]$, estimate the (overestimator of) dissimilarity between two rows $u, v \in [m]$ as
%		\[	\dissimrow(u,v) = \frac{1}{ | \basesim(u) \cap \basesim(v) | } \sum_{j \in \basesim(u) \cap \basesim(v)} \big( Y(u,j) - Y(v,j) \big)^2	\]
%		\item
%		We consider $\{ v \in [m]: \dissimrow(u,v) \leq \eta \}$ as the set of reliable neighbor rows of $u$.
%		\item
%		Define 
%		\[	\baseest(u,i) \triangleq \big\{ (v,j) \in [m] \times [n]: \dissimrow(u,v) \leq \eta ~~\text{and}~~ (v,j) \in \Omega_2  \big\}.	\]
%	\end{itemize}
%	
%	\item
%	Compute the estimate for $(u,i)$ as
%		\[	\hA(u,i) = \frac{1}{| \baseest(u,i) |} \sum_{(v,j) \in \baseest(u,i)} Y(v,j) .	\]
%\end{enumerate}
%
%{\em Remark.}
%Note that for each $v \in [m]\setminus \{1\}$, $(v,1) \in \baseest(1,1)$ if and only if $M(v,1) = 1$ and $\dissimrow(1,v) \leq \eta$. 
%Also, $M(v,1) = 1$ is independent of $\dissimrow(1,v) \leq \eta$.
%
%{\em Remark.}
%\DG{Note that the version we analyzed in NIPS paper is of order $1$.}


\subsection{Analysis}
%We want to establish an upper bound on the mean-squared error.
%\[	\MSE(\hA) = \Exp{ \frac{1}{mn} \sum_{u,i} \big( \hA(u,i) - A(u,i) \big)^2 .}	\]
%Here, expectation is taken over all randomness in the data generation process: (i) realization of the latent variables; 
%(ii) realization of the noise variables; and (iii) masking. We may consider the latent function $f$ is unknown, yet deterministic.
%
%\begin{theorem}[Main Theorem]\label{thm:main_mse_user}
%For user-user $k$-nearest neighbor algorithm,
%\begin{align*}
%	\MSE(\widehat{A}) &\leq \big( \eta - 2\sigma^2 \big)
%		+ CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg]
%		+ 2 \bigg[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg]^{-1}\\
%		&\qquad 	+ \frac{1}{m-1}
%		+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)
%		+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
%\end{align*}
%Here, $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$ and $C, c > 0$ are absolute constants. 
%\end{theorem}
%
%\begin{proof}[Proof of Theorem \ref{thm:main_mse_user}]
%Due to the exchangeability of the model and the linearity of the expectation,
%\[	\MSE(\hA) = \Exp{\big( \hA(u,i) - A(u,i) \big)^2 }	 = \Exp{\big( \hA(1,1) - A(1,1) \big)^2 }.	 \]
%Recall from Algorithm \ref{alg} that 
%\[	\hA(1,1) = 	 \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} Z(v,1) \]
%in our user-user $k$-nearest neighbor algorithm. Therefore,
%\begin{align*}
%	&\Exp{\big( \hA(1,1) - A(1,1) \big)^2 }\\
%		&\qquad=  \Exp{ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2
%				+ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 }\\
%		&\qquad=  \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 \Bigg]
%				+ \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 \Bigg]\\
%		&\qquad\stackrel{(a)}{\leq}
%				\bbE_{\Frandom \setminus \featcol{1} } 
%				\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2	\bigg]
%			+ C \sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~\Ind\big( { \Nbase \geq 1 }\big)  \bigg]
%\end{align*}
%where $C > 0$ is an absolute constant (coming from $\| X \|_{\psi_2} \leftrightarrow \Var(X)$). 
%The inequality in (a) follows from Lemmas \ref{lem:signal_MSE_upper} and \ref{lem:noise_MSE_upper}.
%
%We will need local properties of the probability measure on the latent space to upper bound the two terms in the last line. By Lemma 
%\ref{lem:signal_technical}, when $\eta \geq 2\sigma^2$:
%\begin{align*}
%	\bbE_{\Frandom \setminus \featcol{1} } 
%		\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2	\bigg]
%		&\leq \big( \eta - 2\sigma^2 \big)
%		+ CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg].
%\end{align*}
%
%Moreover, when $\eta \geq 2\sigma^2 + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$ we have
%\begin{align*}
%	\bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg]
%		&\leq 2 \bigg[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg]^{-1}	+ \frac{1}{m-1} \\
%			&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)
%			+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big)
%\end{align*}
%by Lemma \ref{lem:noise_technical}.
%\end{proof}


\subsection{Helper Lemmas}
\subsubsection{Reduction}
\paragraph{Upper Bounding Signal MSE}
\begin{lemma}\label{lem:signal_MSE_upper}
	\begin{align*}
		\bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 \Bigg]
			= \bbE_{\Frandom \setminus \featcol{1} } 
				\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2	\bigg].
	\end{align*}
\end{lemma}
\begin{proof}
First, we note that the expectation is taken with respect to $m + n + 2mn$ independent sources of randomness, $ \big\{ \featrow{u}\big\}_{u \in [m]}$, 
$\big\{ \featcol{i} \big\}_{i \in [n]}, \big\{ N(u,i) \big\}_{(u,i) \in [m] \times [n]}$,  $\big\{ M(u,i) \big\}_{(u,i) \in [m] \times [n]}$. We let $\Frandom$ denote 
the collection of these random variables. Then,
\begin{align*}
	&\bbE\Bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 \Bigg]\\
		&\qquad= \bbE_{\Nbase}\Bigg[ ~ \bbE_{\Frandom | \Nbase  }\bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 ~\bigg|~ \Nbase \bigg] ~\Bigg].
\end{align*}
We investigate the conditional expectation.
\begin{align*}
	&\bbE_{\Frandom \big| \Nbase }\bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 ~\bigg|~ \Nbase \bigg] \\
		&\qquad	= \frac{1}{| \baseest(1,1) |^2} \bbE_{\Frandom \big| \Nbase }\bigg[ \bigg(  \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 
			~\bigg|~ \Nbase \bigg] \\
		&\qquad	= \frac{1}{| \baseest(1,1) |^2} \bbE_{\Frandom \big| \Nbase }\bigg[ \Bigg(   \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)} 
			\big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| ~\bigg|~ \Nbase \Bigg] \\
		&\qquad	= \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \Nbase } \Bigg[~ \bbE_{\featcol{1} \big| \Nbase}
			\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)} \big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big|
			~\bigg|~ \Nbase \Bigg] ~\Bigg|~ \Nbase \Bigg] \\
		&\qquad	= \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \Nbase } 
			\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\bbE_{\featcol{1}  \big| \Nbase } \Big[ \big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| ~\Big|~ \Nbase \Big]
			~\bigg|~ \Nbase \Bigg]\\
		&\qquad	\stackrel{(a)}{=} \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \Nbase } 
			\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\bbE_{\featcol{1}} \Big[ \big| A(v,1) - A(1,1) \big|\big| A(v',1) - A(1,1) \big| \Big]
			~\bigg|~ \Nbase \Bigg]\\
		&\qquad	= \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1}  \big| \Nbase } 
			\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\Big\| \big[ f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big] \big[ f(\featrow{v'}, \cdot ) - f(\featrow{1}, \cdot) \big] \Big\|_{L^1}
			~\bigg|~ \Nbase \Bigg]\\
		&\qquad	\stackrel{(b)}{\leq} \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \Nbase } 
			\Bigg[ \sum_{(v,1) \in \baseest(1,1) \atop (v',1) \in \baseest(1,1)}
				\Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2} \Big\| f(\featrow{v'}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}
			~\bigg|~ \Nbase \Bigg]\\
		&\qquad	\leq \frac{1}{| \baseest(1,1) |^2 } \bbE_{\Frandom \setminus \featcol{1} \big| \Nbase } 
			\Bigg[ | \baseest(1,1) |^2  \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
			~\bigg|~ \Nbase \Bigg]\\
		&\qquad=  \bbE_{\Frandom \setminus \featcol{1} \big| \Nbase } 
			\Bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
			~\bigg|~ \Nbase \Bigg].
\end{align*}
Here, (a) follows from the independence between $\baseest(1,1)$ and $\featcol{1}$ in our user-user $k$-nearest neighbor algorithm; 
(b) follows from Cauchy-Schwarz inequality.

Consequently, it follows that 
\[	\bbE\Bigg[ \bigg( \frac{1}{\Nbase} \sum_{(v,1) \in \baseest(1,1)} \big( A(v,1) - A(1,1) \big) \bigg)^2 \Bigg]
		= \bbE_{\Frandom \setminus \featcol{1} } 
			\Bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2	\Bigg].
\]
\end{proof}

\paragraph{Upper Bounding Noise MSE}
We take the convention that $\frac{0}{0} = 0$. This is easily justified by defining our estimate $\widehat{A}(1,1) = 0$ when $\Nbase = 0$.
\begin{lemma}\label{lem:noise_MSE_upper}
	\begin{align*}
		 \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 \Bigg]
		 	&\leq C\sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~\Ind\big( { \Nbase \geq 1 }\big) \bigg].
	\end{align*}
\end{lemma}
\begin{proof}
By the tower property of expectation,
\begin{align*}
	 \bbE\Bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 \Bigg]
	 	&= \bbE\Bigg[ ~ \bbE\bigg[ \bigg( \frac{1}{| \baseest(1,1) |} \sum_{(v,1) \in \baseest(1,1)} N(v,1)\bigg)^2 ~ \bigg|~ \Nbase \bigg] ~\Bigg]\\
		&\leq \bbE\Bigg[ ~ \bbE\bigg[  \frac{1}{| \baseest(1,1) |} \max_{(v,i) \in \baseest(1,1) } \bbE | N(v,1) |^2 ~ \bigg|~ \Nbase \bigg] ~\Bigg]\\
		&\leq \bbE\Bigg[ ~  \frac{1}{| \baseest(1,1) |}~  \bbE\Big[ ~C \sigma^2 ~ \Big|~ \Nbase \Big]~ \Ind\big(\Nbase \geq 1\big) ~\Bigg]	\\
		&\leq C\sigma^2 \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg].
\end{align*}
\end{proof}


%%%	Technical Lemmas

\subsubsection{Technical Lemmas}
\paragraph{Idea}
\begin{itemize}
\item
	Note that for each $v \in [m]\setminus \{1\}$, $(v,1) \in \baseest(1,1)$ if and only if $M(v,1) = 1$ and $\dissimrow(1,v) \leq \eta$. 
	Also, $M(v,1) = 1$ is independent of $\dissimrow(1,v) \leq \eta$.
\item
	$| \baseest(1,1) |$ is defined based on the empirical version of $ \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2$ 
	based on $\Omega_1$ -- columns other than the first column. The uncertainty (statistical fluctuation) of that estimation scales as $\frac{1}{\sqrt{(n-1)p}}$. 
	Therefore, we expect the first term to be no greater than $(\eta - 2\sigma^2) + \frac{C}{\sqrt{(n-1)p}}$ \DG{Need to write this more formally.}

\item
	$ \bbE \Big[ \frac{1}{| \baseest(1,1) |} \Big]$ that ensures $| \baseest(1,1) |$ is sufficiently large with high probability, say, $\Prob{ | \baseest(1,1) | < \Nsmall } 	\leq \epssmall$. Then it follows that
	\begin{align*}
		\bbE \bigg[ \frac{1}{| \baseest(1,1) |} \bigg]
			&= \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Big| ~ | ~ \baseest(1,1) | \geq \Nsmall \bigg] \Prob{| \baseest(1,1) | \geq \Nsmall} \\
				&\quad + \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ | ~ \baseest(1,1) | < \Nsmall \bigg] \Prob{\baseest(1,1) | < \Nsmall}\\
			&\leq \frac{1}{\Nsmall} + \epssmall.
	\end{align*}
	It only remains to find a configuration $(\Nsmall, \epssmall)$ such that $\frac{1}{\Nsmall}, \epssmall \to 0$ simultaneously at the rate as fast as possible.
\end{itemize}

\paragraph{Upper bounding the contribution of signal on MSE bound}
\begin{lemma}\label{lem:signal_technical}
Let $\eta \geq 2\sigma^2$. The following inequality holds for user-user $k$-nearest neighbor algorithm:
	\begin{align*}
		&\bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2	\bigg]\\
			&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{\sqrt{2 c (n-1)p^2}} + \frac{2K e^{-\frac{c}{2} (n-1)p^2}}{c (n-1)p^2}
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg) \exp\Big( - \frac{(n-1)p^2}{8} \Big)\\
			&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ CK \bigg[  \frac{1}{\sqrt{ (n-1) p^2}} + \exp \big(-c (n-1)p^2\big) \bigg].
	\end{align*}
Here, $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$ and $C, c > 0$ are absolute constants.
\end{lemma}
\begin{proof}
\textbf{Step 1:}
Choose $v \in [m] \setminus \{1\}$ such that $(v,1) \in \baseest(1,1)$. Observe that 
\[
	\dissimrow(1,v) = \frac{1}{|\basesim(1) \cap \basesim(v)|} \sum_{j \in \basesim(1) \cap \basesim(v)} \big( Z(1,j) - Z(v,j) \big)^2.
\] 
Note that $Z(1,j) - Z(v,j) = \big( X(1,j) -X(v,j) \big) + \big( N(1,j) - N(v,j) \big)$. By the model assumptions, we have
\begin{align*}
	&|X(1,j) - X(v,j)| \leq \lip \diamrow \quad\forall v, j	\qquad \Rightarrow \qquad \big\| X(1,j) - X(v,j) \big\|_{\psi_2} 
		\leq \frac{\lip \diamrow}{\sqrt{\ln 2}},\\
	&\big\| N(1,j) - N(v,j) \big\|_{\psi_2} \leq \big\| N(1,j) \big\|_{\psi_2} + \big\| N(v,j) \big\|_{\psi_2} = 2\sigma.
\end{align*}
Therefore (cf. Vershynin's hdp-book, Lemma 2.7.6),
\begin{align*}
	\big\| Z(1,j) - Z(v,j) \big\|_{\psi_2} &\leq \big\| X(1,j) - X(v,j) \big\|_{\psi_2} + \big\| N(1,j) - N(v,j) \big\|_{\psi_2} 
		\leq  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma,\\
	\big\| \big(Z(1,j) - Z(v,j) \big)^2 \big\|_{\psi_1} &= \big\| Z(1,j) - Z(v,j) \big\|_{\psi_2}^2
		\leq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2.
\end{align*}
Let $K \triangleq \Big(  \frac{\lip \diamrow}{\sqrt{\ln 2}} + 2 \sigma \Big)^2$. When $|\basesim(1) \cap \basesim(v)| = N_v$, 
it follows from Bernstein's inequality (cf. Vershynin, hdp-book, Theorem 2.8.2; note that we use only one side of the 
two-sided inequality) that for any $t \geq 0$,
\begin{align*}
	\Prob{ \dissimrow(1,v) - \Exp{\dissimrow(1,v)} \leq - t} 
		\leq \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) N_v \bigg].
\end{align*}
Moreover, we can easily observe that $\Exp{\dissimrow(1,v)} = \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 + 2\sigma^2$. 
This leads to the following inequality: for any $t \geq 0$,
\begin{align}
	&\Prob{ \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2 \geq \dissimrow(1,v) - 2\sigma^2 + t  
		~ \Big|~ |\basesim(1) \cap \basesim(v)| = N_v}	\nonumber\\
		&\qquad\leq  \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) N_v \bigg].	\label{eqn:conc_dissim}
\end{align}

\textbf{Step 2:} Let $v^* \in [m] \setminus \{1\}$ denote the maximizer such that $(v^*, 1) \in \baseest(1,1)$ and 
\[	\Big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2
		= \max_{(v,i) \in \baseest(1,1) } \Big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \Big\|_{L^2}^2.	\]
According to the description of our user-user $k$-nearest neighbor algorithm, $\dissimrow(1,v^*) \leq \eta$.
\begin{align}
	&\bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \max_{(v,i) \in \baseest(1,1) } \big\|  f(\featrow{v}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	\bigg]	\nonumber\\
		&\qquad= \bbE_{\Frandom \setminus \featcol{1} } 
			\bigg[ \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	\bigg]	\nonumber\\
		&\qquad= \bbE_{N_v }  \Bigg[ \int_0^{\infty}
			\bbP\bigg( \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	 \geq s 
			~ \Big| ~  |\basesim(1) \cap \basesim(v)| = N_v \bigg) ~ds \Bigg].	\label{eqn:upper_signal_term.1}
\end{align}

Now we observe that 
\begin{align}
	& \int_0^{\infty} \bbP\bigg( \big\|  f(\featrow{v^*}, \cdot ) - f(\featrow{1}, \cdot) \big\|_{L^2}^2	 \geq s 
			~ \Big| ~  |\basesim(1) \cap \basesim(v)| = N_v \bigg) ~ds	\nonumber\\
		&\qquad\leq \int_0^{\eta - 2\sigma^2} ds
			+ \int_{0}^{K} \exp \bigg[ -c N_v \frac{t^2}{K^2} \bigg] ds
			+ \int_{K}^{\infty} \exp \bigg[ -c N_v \frac{t}{K} \bigg] ds	\nonumber\\
		&\qquad\leq \big( \eta - 2\sigma^2 \big) 
			+ \int_{0}^{\infty} \exp \bigg[ -c N_v \frac{t^2}{K^2} \bigg] ds
			+ \int_{K}^{\infty} \exp \bigg[ -c N_v \frac{t}{K} \bigg] ds	\nonumber\\
		&\qquad= \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v}.	\label{eqn:upper_signal_term.2}
\end{align}
Recall that for $a > 0$ and $b \in \Reals$,
\[	
	\int_0^{\infty} e^{-a x^2} dx = \frac{1}{2}\sqrt{\frac{\pi}{a}}
	\qquad\text{and}\qquad
	\int_b^{\infty} e^{-a x} dx = \frac{1}{a}e^{-ab}.	
\]
%\DG{***TODO - The following must be made a formal argument:}
%Since $N_v$ sharply concentrates to $(n-1)p^2$, the upper bound in \eqref{eqn:upper_signal_term.1} (using \eqref{eqn:upper_signal_term.2}) 
%becomes
%\[	 \big( \eta - 2\sigma^2 \big)
%			+ CK \bigg[  \frac{ \sqrt{\pi}}{2\sqrt{c (n-1) p^2}} + \frac{e^{-c (n-1)p^2}}{c (n-1)p^2} \bigg].	\]

\textbf{Step 3:} Observe that $ |\basesim(1) \cap \basesim(v)| \sim \textrm{Binomial}(n-1, p^2)$. By the binomial Chernoff theorem,
\[	\Prob{ N_v \leq \frac{1}{2} (n-1)p^2} \leq \exp\Big( - \frac{(n-1)p^2}{8} \Big).	\]
Therefore,
\begin{align*}
	&\bbE \Bigg[ \big( \eta - 2\sigma^2 \big)	+ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} \Bigg]\\
		&\qquad= \big( \eta - 2\sigma^2 \big)
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v > \frac{1}{2} (n-1)p^2 \bigg]
			\Prob{N_v > \frac{1}{2} (n-1)p^2}\\
			&\qquad\quad
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v \leq \frac{1}{2} (n-1)p^2 \bigg]
			\Prob{N_v \leq \frac{1}{2} (n-1)p^2}\\
		&\qquad\stackrel{(a)}{\leq} \big( \eta - 2\sigma^2 \big)
			+ \bbE \bigg[ \frac{K \sqrt{\pi}}{2\sqrt{c N_v}} + \frac{K e^{-c N_v}}{cN_v} ~\Big|~N_v > \frac{1}{2} (n-1)p^2 \bigg]\\
			&\qquad\quad
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg)
			\Prob{N_v \leq \frac{1}{2} (n-1)p^2}\\
		&\qquad\leq \big( \eta - 2\sigma^2 \big)
			+ \frac{K \sqrt{\pi}}{\sqrt{2 c (n-1)p^2}} + \frac{2K e^{-\frac{c}{2} (n-1)p^2}}{c (n-1)p^2}
			+ \bigg( \frac{K \sqrt{\pi}}{2\sqrt{c }} + \frac{K e^{-c}}{c} \bigg) \exp\Big( - \frac{(n-1)p^2}{8} \Big).
\end{align*}
The inequality in (a) follows from that $N_v \geq 1$ and $\frac{K e^{-c N_v}}{cN_v}$ is maximized when $N_v = 1$.
\end{proof}







				
\paragraph{Upper bounding the contribution of noise on MSE bound}
\begin{lemma}\label{lem:noise_technical}
	Let $\eta \geq 2\sigma^2 + K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$. 
	The following inequality holds for user-user $k$-nearest neighbor algorithm:
	\begin{align*}
		\bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg]
			&\leq 2 \bigg[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg]^{-1}	+ \frac{1}{m-1} \\
				&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)
				+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
	\end{align*}
\end{lemma}

%\DG{***TODO:}
%We expect $| \baseest(1,1) | \gtrsim (m-1)p~ \msra{ \frac{\sqrt{\eta - 2\sigma^2}}{\lip} }$

\begin{proof}
\textbf{Step 1:}
Let $\eta' = \eta - K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.
For each $v \in [m] \setminus \{ 1 \}$, the following two conditions
\begin{equation}\label{eqn:cond_good_row}
	M(v,1) = 1	\qquad\text{and}\qquad  \drow(\featrow{1}, \featrow{v}) \leq \frac{\sqrt{\eta' - 2\sigma^2}}{L}
\end{equation}
are satisfied with success probability\footnote{Note that the first condition solely depends on $M(v,1)$, while the second condition 
depends only on $\featrow{1}, \featrow{v}$, hence, they are independent events.} at least 
$p \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big)$. Let $\goodrows \subset [m] \setminus \{1 \}$ denote the set of row indices 
that satisfy the two conditions described in \eqref{eqn:cond_good_row}. By the binomial Chernoff bound,
\begin{equation}\label{eqn:upper_noise_term.1}
	\Prob{ |\goodrows| \leq \frac{1}{2} (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) }
		\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg).
\end{equation}

\textbf{Step 2:}
Next, we want to show that $\{(v,1): v \in \goodrows\} \subset \baseest(1,1)$ with high probability.
For that purpose, we first require $|\basesim(1) \cap \basesim(v) |$ to be sufficiently large for all $v \in \goodrows$. Observe that 
for each $v \in \goodrows$, $|\basesim(1) \cap \basesim(v) |$ is distributed following $\textrm{Binomial}(n-1, p^2)$. By the binomial 
Chernoff bound, we have 
\[	\Prob{|\basesim(1) \cap \basesim(v)| \leq \frac{(n-1)p^2}{2}} \leq \exp \Big( - \frac{(n-1)p^2}{8} \Big).	\]
Since $|\goodrows| \leq m-1$, it follows from the union bound that 
\begin{equation}\label{eqn:upper_noise_term.2}
	\Prob{ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| \leq \frac{(n-1)p^2}{2}} \leq (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).
\end{equation}

Due to the Lipschitzness assumption on the latent function, it follows that for all $v \in \goodrows$,
\begin{align*}
	\big\| f(\featrow{1}, \cdot) - \featrow{v}, \cdot) \big\|_{L^2}^2 \leq \eta' - 2\sigma^2.
\end{align*}
By \eqref{eqn:conc_dissim} and another application of the union bound, this implies that
\begin{align*}
	&\Prob{ \max_{v \in \goodrows }\dissimrow(1,v) \leq \eta' + t ~\bigg| ~ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2}}\\ 
		&\qquad\leq (m-1)  \exp \bigg[ -c \min \Big( \frac{t^2}{K^2}, \frac{t}{K} \Big) \frac{(n-1)p^2}{2} \bigg].
\end{align*}
Therefore\footnote{Recall that $\eta' = \eta - t$ with $t = K \max\Big( \sqrt{\frac{4 \log (m-1)}{c(n-1)p^2}}, \frac{4 \log (m-1)}{c(n-1)p^2} \Big)$.},
\begin{equation}\label{eqn:upper_noise_term.3}
	\Prob{ \max_{v \in \goodrows }\dissimrow(1,v) \leq \eta ~\bigg| ~ \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2}}
		\leq \frac{1}{m-1}.
\end{equation}
Observe that 
\begin{equation}\label{eqn:upper_noise_term.4}
	\text{if}\quad
	\max_{v \in \goodrows }\dissimrow(1,v) \leq \eta
	\qquad\text{then}\quad
	\{(v,1): v \in \goodrows\} \subset \baseest(1,1).
\end{equation}

\textbf{Step 3:}
Let 
\begin{align*}
	\Eva	&\triangleq \bigg\{  |\goodrows| > \frac{1}{2} (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg\}\\
	\Evb	&\triangleq \bigg\{  \max_{v \in \goodrows }\dissimrow(1,v) \leq \eta  \bigg\},\\
	\Evc	&\triangleq \bigg\{  \min_{v \in \goodrows }|\basesim(1) \cap \basesim(v)| > \frac{(n-1)p^2}{2} \bigg\}.
\end{align*}
By the law of total probability,
\begin{align*}
	\bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big)  \bigg]
		&\stackrel{(a)}{\leq} \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~ \Eva \cap \Evb  \bigg] \Prob{\Eva \cap \Evb} 
			+ \Prob{\Eva^c \cup \Evb^c }\\
		&\leq \bbE \bigg[ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) ~\Big|~ \Eva \cap \Evb  \bigg] 
			+ \Prob{\Eva^c} + \Prob{\Evb^c|\Evc} + \Prob{\Evc^c}\\
		&\stackrel{(b)}{\leq}
			2 \bigg[  (m-1)p  \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L} \Big) \bigg]^{-1}	+ \frac{1}{m-1} \\
				&\qquad+ \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg)
				+ (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big)
\end{align*}
where (a) follows from $ \frac{1}{| \baseest(1,1) |} ~ \Ind\big(\Nbase \geq 1\big) \leq 1$; and (b) follows from that \eqref{eqn:upper_noise_term.4} and
\begin{align*}
	\Prob{\Eva^c}	&\leq \exp\bigg( - \frac{(m-1)p}{8} \cdot \msrrow\Big( \frac{\sqrt{\eta' - 2\sigma^2}}{L}\Big) \bigg),
			&\because \eqref{eqn:upper_noise_term.1}\\
	\Prob{\Evb^c|\Evc} &\leq	\frac{1}{m-1},		
			&\because \eqref{eqn:upper_noise_term.3}\\
	\Prob{\Evc^c}	&\leq (m-1)\exp \Big( - \frac{(n-1)p^2}{8} \Big).		
			&\because\eqref{eqn:upper_noise_term.2}
\end{align*}

\end{proof}



\newpage


==> contents/prob_statement/model_ds.tex <==
\section{Setup}\label{sec:setup}

%%% ====================================================================
%%%	Model
%%% ====================================================================

\subsection{Our Model}\label{sec:model}
Suppose that there is an unknown $m \times n$ matrix $A$ which we would like to estimate. We observe only a fraction 
of the total $mn$ entries of $A$ with some noise added. Let $\obs \subset [m] \times[n]$ denote the index set of observed entries. 

Precisely, we consider the following data generation model. Our data matrix $Z$ is an $m \times n$ matrix that is generated 
as follows. Let $M \in \{0,1\}^{m \times n}$ be a binary matrix, which we call the masking matrix. We let $A \in \Reals^{m \times n}$ 
denote the signal matrix and $N \in \Reals^{m \times n}$ denote the noise matrix. For each $(u,i) \in [m] \times [n]$, 
\begin{equation}\label{eqn:gen_model}
	Z(u,i) = \begin{cases}
			A(u,i) + N(u,i)	&	\text{when }M(u,i) = 1,\\
			\text{unknown}	&	\text{when }M(u,i) = 0.
		\end{cases}
\end{equation}
For later use, we let $\Omega \triangleq \{ (u,i) \in [m] \times [n]: M(u,i) = 1 \}$ denote the set of index pairs of the observed entries. 

\subsubsection{Latent Variable Model}\label{sec:lv_model}
We assume $A(u,i)$ is generated by the following model.
\begin{itemize}
	\item
	Nonparametric model: there exists a latent function $f$ such that
	\begin{equation}\label{eqn:latent_model}
		A(u,i) = f( \featrow{u}, \featcol{i})	
	\end{equation}
	for all $(u,i) \in [m] \times [n]$. Here, $\featrow{u}, \featcol{i}$ denote latent varialbes associated with row $u$ 
	and column $i$, respectively.
	\item
	Regularity Assumptions
	\begin{itemize}
		\item
		For all $u \in [m]$, $\featrow{u} \in \latsprow$, where $(\latsprow, \drow)$ is a metric space such that 
		$\diam \latsprow = \sup_{\alpha, \beta \in \latsprow} \drow(\alpha, \beta) \leq \diamrow$. 
		Moreover, $\latsprow$ is equipped with a Borel probability measure $\murow$ and $\featrow{u}$ 
		is drawn i.i.d. according to $\murow$.
		\item
		For all $i \in [n]$, $\featcol{i} \in \latspcol$, where $(\latspcol, \dcol)$ is a metric space such that 
		$\diam \latspcol = \sup_{\alpha', \beta' \in \latspcol} \dcol(\alpha', \beta') \leq \diamcol$. 
		Moreover, $\latspcol$ is equipped with a Borel probability measure $\mucol$ and $\featcol{i}$ 
		is drawn i.i.d. according to $\mucol$.
		\item
		Latent function $f$ is $\lip$-Lipschitz in the sense that 
		\[	\big| f( \alpha_1, \alpha_1) - f( \beta_1, \beta_2) \big|
				\leq \lip \max \big( \drow(\alpha_1, \beta_1), \dcol(\alpha_2, \beta_2) \big).	\]
	\end{itemize}
\end{itemize}

\subsubsection{Noise}
We assume $N(u,i)$ is a centered, sub-gaussian random variable for all $(u,i) \in [m] \times [n]$ such that
\begin{itemize}
	\item
	Centered: $\bbE N(u,i) = 0$ for all $(u,i) \in [m] \times [n]$.
	\item
	Sub-gaussian: there exists $\sigma > 0$ such that $\| N(u,i) \|_{\psi_2} \leq \sigma$ for all $(u,i) \in [m] \times [n]$.\chris{add a footnote for defining the $\| \cdot \|_{\psi_2}$ notation?}
	\item
	Independent and identically distributed: $N(u,i)$'s are independent and identically distributed (due to the exchangeability).
\end{itemize}

\subsubsection{Masking}
We assume $M$ is a random matrix with each entry drawn as per $Bernoulli(p)$ for some $p \in (0,1]$, i.i.d. That is, for each 
$(u,i) \in [m] \times [n]$, 
\[	
	M(u,i) = \begin{cases}
			1	&	\text{with probability }p,\\
			0	&	\text{with probability }1-p.
			\end{cases}	
\]


%%% ====================================================================
%%%	Problem Statement
%%% ====================================================================

\subsection{Problem Statement: Blind Regression}
Note that the latent variable model representation in \eqref{eqn:latent_model} is not the unique representation, as there exists multiple
equivalent representations. Suppose that one applies a measure-preserving transformation $T$ on the latent feature space 
$\latsprow \times \latspcol$, and take the push-forward of $f$ with respect to $T$ ($f \circ T^{-1}$) as the new latent function. 
This new representation -- the pair of the latent space and the latent function -- yields the same data generation process. Therefore, 
the question of estimating the function $f$ itself is not well posed, and we focus our energy on predicting the values $A(u,i)$. 

\begin{problem}[Blind Regression]\label{prob:blind_regression}
	Given $Z \in \Reals^{m \times n}$ that is partially observed on $\Omega \subset [m] \times [n]$ as described in Section \ref{sec:model}, 
	we want to estimate the underlying matrix $A$.
\end{problem}
We call the problem of interest {\em Blind Regression} for the following reason. In the setting of {\em Regression}, one observes data containing features and associated labels; the goal is to learn the functional relationship (or model) between features and labels assuming that labels are noisy observations. In our setting, tuples $(\featrow{u}, \featcol{i})$ are the relevant (but unobserved) features and $Z(u,i)$ are noisy observations of associated labels $A(u,i) = f(\featrow{u},\featcol{i)})$. We want to predict the value of $f(\featrow{v},\featcol{i})$ for all pairs $(v,i)$. In the sense that we want to predict the function $f$ evaluated on new points given previous data, the task has the feel of Regression. However, the features $(\featrow{u}, \featcol{i})$ are {\em latent}; and thus we use the term {\em Blind Regression}. 

Given an estimator $\hat{A}$ for the unknown matrix $A \in \Reals^{m \times n}$ of interest, we use the mean-squared error (MSE) to evaluate the performance of the estimator, defined as 
\begin{equation}\label{eqn:MSE}
    \MSE(\hat{A}) = \Exp{ \frac{1}{mn}\sum_{u=1}^m \sum_{i=1}^n \left( \hat{A}(u,i) - A(u,i)\right)^2 }.
\end{equation}
The expectation here is taken over all sources of randomness in the data generation process: (i) realization of the latent variables; 
(ii) realization of the noise variables; and (iii) masking. 
% We may consider the latent function $f$ is unknown, yet deterministic.
An estimator $\hat{A}$ is called consistent if $\lim_{m, n \to \infty} \MSE(\hat{A}) = 0$. For a consistent estimator, we also want to 
establish an upper bound on the rate of convergence rate for the mean-squared error. Now we pose a follow-up question.
\begin{problem}
	Can we achieve a consistent estimator $\hat{A}$ for $A$ in the setup of Problem \ref{prob:blind_regression}? 
	If so, how fast does $\MSE(\hat{A})$ decay to $0$ as the problem size $m, n \to \infty$? 
\end{problem}

%%% ====================================================================
%%%	Connections to Other Models
%%% ====================================================================

\subsection{Discussion of Our Model}
\subsubsection{Exchangeability and Latent Variable Model}
The latent variable model is well motivated and arises as a canonical representation for row and column exchangeable data, cf.  \cite{Aldous81} and  \cite{Hoover82}. 
Suppose that our data matrix $Z$ is a particular realization of the first $m \times n$ entries of a random array $\bZ = \left\{\bZ(u,i) \right\}_{(u, i) \in \Nats \times \Nats}$, which satisfies \chris{Is the below notation clear the equivalently distributed is referring to the entire $\bZ$ and not just the marginals $\bZ(u,i)$?}
\begin{align}\label{eq:exchangeable}
 \bZ(u,i) \overset{d}{=} \bZ\left(\sigma(u), \tau(i)\right) ~\text{ for all } (u,i),
\end{align}
for every pair of permutations\footnote{The permutations over $\Nats$ are defined in the usual manner where only finitely many indices are {\em permuted}.} $\sigma, \tau$ 
of $\Nats$. We use $\overset{d}{=}$ to denote equivalently distributed, i.e. the random variables on both sides have the same distribution. Random array $\bZ$ satisfying 
\eqref{eq:exchangeable} is called exchangeable\footnote{To be precise, {\em separately} row and column exchangeable.}. 
%That is, a dataset is exchangeable if the distribution is invariant to permutations of the rows and columns. 
For an interested reader, \cite{Austin12} and \cite{OrbRoy2015} present overviews of exchangeable arrays.  

In practice, the use of exchangeable arrays as a model is appropriate for variety of reasons. For example, in the setting of a recommendation system with anonymized data, 
this property may be reasonable if the order of the users in the system does not intrinsically carry information about the type of user; or in other words, if a user in the system 
could equally likely have been located in any row of the dataset. 

In addition to exchangeability being quite a reasonable property for a wide variety of applications, it also leads to a convenient latent variable representation. The Aldous-Hoover representation theorem provides a succinct characterization for such exchangeable arrays. According to the theorem (see Corollary 3.3 in \cite{OrbRoy2015} for example), a random 
data array $\bZ$ is exchangeable if and only if it can also be represented as \chris{Is $\theta$ easily confused with $\theta(u,i)$?}
\begin{align} \label{eq:exch_form}
 \bZ\left( u,i \right) \overset{d}{=} f_{\theta}\big( \frow(u), \fcol(i), \theta(u,i) \big) ~\text{ for all }(u,i)
\end{align}
where $\theta$, $\big\{\frow(u)\big\}_{u \in \Nats}$, $\big\{\fcol(i)\big\}_{i \in \Nats}$, $\big\{\theta(u,i)\big\}_{(u,i) \in \Nats \times \Nats}$ are independent random variables 
drawn uniformly at random from the unit interval $[0,1]$, and $f_{\theta}$ is a measurable function indexed by the realization of $\theta$. 
%; that is, for any particular realization 
%$\theta = t$ with $t \in [0,1]$, $f_{\theta} = f_t$ where $f_{\theta} = f_t: [0,1]^3 \to \Reals$ is measurable. 
As described in \cite{OrbRoy2015}, this suggests the following generative model: 
%representation yields the following data generation process for $\bZ$:
\begin{enumerate}
	\item	Sample an instance of $\theta \sim U[0,1]$ determining the governing function $f_{\theta}$.
	\item Independently sample uniform random variables $\frow(u) \sim U[0,1]$, $\fcol(i) \sim U[0,1]$, $\theta(u,i) \sim U[0,1]$ for every row $u \in [m]$ and column $i \in [n]$.
	\item Compute the realized data matrix $Z$ according to 
	\begin{align*}
	Z(u,i) = f_{\theta}\big( \frow(u), \fcol(i), \theta(u,i) \big).
	\end{align*}
\end{enumerate}

By comparing the model from \eqref{eq:exch_form} with the latent variable model described in Section \ref{sec:lv_model} (cf. \eqref{eqn:gen_model}, \eqref{eqn:latent_model}), 
we can see that the latent variable model considered in this work is a restricted subclass of exchangeable models that additionally impose an additive noise model and 
regularity conditions on the function $f_{\theta}$ in exchange for the freedom to choose a more general latent space and the probability measure it is equipped with. \chris{reword/clarify this sentence}

\medskip
\paragraph*{Transforming between Models}
In our model we have conditioned on the universal index\footnote{Equivalently, we may think that $f_{\theta} = f$ for all $\theta \in [0,1]$. Note that we do not know what $f$ is a priori.} 
$\theta$, such that given partial observations from matrix $Z$ for a particular $f_{\theta}$, our goal is to learn predicted outcomes of the realized $f_{\theta}$. Our model takes 
the form of
\begin{align}
 	Z(u,i) =  f(\featrow{u}, \featcol{i}) + \eta(u,i)
	\end{align}
where $\{\featrow{u}\}_{u \in [m]}, \{\featcol{i}\}_{i \in [n]}, \{\eta(u,i)\}_{(u,i) \in [m] \times [n]}$ are sampled independently. We can transform this to the form of \eqref{eq:exch_form} by 
considering $f$ to be equal to the realized function $f_{\theta}$, considering the latent variables $\featrow{u} \sim \prxa$ and $\featcol{i} \sim \prxb$ to be higher dimensional 
representations of $\frow(u)$ and $\fcol(i)$ in spaces $\latspA$ and $\latspB$, and considering the noise term $\eta(u,i)$ to be generated by applying some transformation 
to the variable $\theta(u,i)$. Given these transformations, it becomes equivalent that 
\begin{align} \label{eqn:canonical_repn}
 	Z(u,i) = f_{\theta}\big( \frow(u), \fcol(i), \theta(u,i)  \big) =  f(\featrow{u}, \featcol{i}) + \eta(u,i).
	\end{align}
Our model additionally imposes regularity conditions on $f$ by requiring it to be Lipschitz continuous with respect to the higher dimensional representation 
$\latspA \times \latspB$ instead of being any arbitrary measurable function over $[0,1] \times [0,1]$. From a modeling perspective, we are effectively transferring 
the {\em model complexity} from a potentially complex measurable latent function over $[0,1] \times [0,1]$ to a simpler Lipschitz latent function over a potentially 
more complex latent variable space $\latspA \times \latspB$. The simple functional form provides analytic tractability for establishing theoretical results. 


\subsubsection{Connection to the Low-rank Model}
Suppose that the latent spaces $\latsprow$ and $\latspcol$ are equal dimensional vector spaces and the latent function $f$ is a bilinear form. This is a low-rank model with its rank being 
equal to $\min \big\{ \dim \latsprow, \dim \latsprow \big\}$ \chris{$\dim \latsprow = \dim \latsprow$?}. If we assume $\latsprow$ and $\latspcol$ are bounded and equipped with some metric topology, then this model is a specific case of our model with Lipschitz constant being $\big(\diam \latsprow + \diam \latspcol \big)$ (up to a multiplicative constant). Note that we utilize 
a different measure of `model complexity' than the rank of the parameter matrix. 

When the underlying function is truly bilinear and $\min \big\{ \dim \latsprow, \dim \latsprow \big\} \ll \diam \latsprow + \diam \latsprow$, then rank of the data matrix could 
be a better measure to capture the essential complexity of the model; note that the rank of the data matrix does not scale as the diameter of the latent space increases. 
However, if the underlying model is nonlinear, the data matrix is likely to have full rank, e.g., when $f(\featrow{u}, \featcol{i}) = g(\left< \featrow{u}, \featcol{i}\right>)$ for 
some monotone increasing nonlinear function $g$. In particular, when the size of the matrix far exceeds the `intrinsic model complexity' (and hence so does the rank 
of the data matrix), it would make more sense to use our measure. 
\DG{Should we compare with approximately low rank model?} \chris{We could reference Madeleine's paper on approximate low rankness of uniformly analytic fns}
%
%
%In the representation with uniform $[0,1]$ variables (see \ref{eqn:canonical_repn}), we have features in a 1-dimensional compact set $[0,1] \subset \Reals$, but the measurable function $f$ can have a complex form. For analytic purpose, we push complexity into features from the function in order to obtain metric regularity of the function at the cost of simplicity of the features. Specifically, we consider measurable transformation maps $\varphi_1, \varphi_2$, mapping $[0,1]$ to some compact metric spaces equipped with probability measures and satisfying 
%$$    f^{can}\left( U^{row}(u), U^{col}(i)\right)  = f^{reg}\left( \varphi_1\left(U^{row}(u)\right), \varphi_2\left(U^{col}(i)\right)\right). $$
%We assume $f^{reg}$, the push-forward of $f^{can}$ by $\varphi$, is Lipschitz. In the next section, we discuss on the operating assumptions in more detail.

%\dogyoon{We may want to discuss this latent variable/function assumption is not too restrictive here. I copy-and-pasted the comments I added to the NIPS poster temporarily, and will get back to discuss it in full detail: 
%1. Our data matrix is separately exchangeable. 
%2. We can consider a separately exchangeable random matrix and regard our data matrix as an instance of it. 
%3. In its limit, $X_{ij}= g(U, \alpha_i, \beta_j, \epsilon_{ij})$ for some measurable g and i.i.d. r.v.s by Aldous-Hoover theorem.
%4. We consider a function which does not depend on the first coordinate: $g(\alpha_i, \beta_j, \epsilon_{ij}) = f(\alpha_i, \beta_j)+\epsilon_{ij})$. 
%} 




==> contents/tensor_proof/tensor_lemma_proofs.tex <==
\subsection{Proof of Key Lemmas}

In this section we prove the five key lemmas introduced in the proof outline.

\subsubsection{Sufficiently many rows with good overlap}
Using the fact that every entry is independently observed uniformly at random, the size of the overlap between a pair of rows is distributed according to a Binomial random variable. Therefore Lemma \ref{lem:overlap_tensor} follows from a straightforward application of Chernoff's bound.

    \begin{proof} [Proof of Lemma \ref{lem:overlap_tensor}]
        A slight modification of the proof for Lemma \ref{lem:overlap} yields the result. It suffices to redefine $R_{uv}$ as 
        \begin{align*}
        R_{uv} & = \Ind \{ |\ovuvT|\geq \beta_l\} \Ind \{|\ovuvT| \leq \beta_h\}.
        \end{align*}
Since the measurement at each entry still happens i.i.d. with probability $p$, using Chernoff's bound for deviation from mean above and below, we can bound $\Prob{R_{uv} = 0}$. By an application of union bound as in Lemma \ref{lem:overlap}, we can obtain the desired result.	
    \end{proof}


%%% Lemma: Tensor Mean Concentration
\subsubsection{Concentration of mean and variance}
Assuming the overlap between two rows $u$ and $v$ is sufficiently large (but not too large), Lemmas \ref{lem:mean_tensor} and \ref{lem:variance_tensor} prove that the sample mean and variance, $\muvT$ and $\suvT$ of the difference $Z(u,i) - Z(v,i)$ concentrate around their expectations $\muuvT$ and $\siguvT^2$ with high probability. For any pair of rows $(u,v) \in [m] \times [m]$, recall the following definitions
\begin{align*}
     \muvT &:= \frac{1}{\left| \ovuvT \right|}\left(\sum_{j \in \ovuvT} Z(u,j) - Z(v,j)\right), \\
    \suvT &:= \frac{1}{\left| \ovuvT \right| - 1}\sum_{j \in \ovuvT} \left(Z(u,j) - Z(v,j) - \muvT\right)^2, \\
		&:= \frac{1}{2 \left| \ovuvT \right| (\left| \ovuvT \right| - 1)}\sum_{j, h \in \ovuvT \times \ovuvT} \left((Z(u,j) - Z(v,j)) - (Z(u,h) - Z(v,h))\right)^2, \\
    \tilde{m}_{uv}(i) &:= \frac{1}{n'}\sum_{j \in \cN_i} \left(Z(u,j) - Z(v,j)\right),\\
    \tilde{s}^2_{uv}(i) &:= \frac{1}{n'-1}\sum_{j \in \cN_i} \left(Z(u,j) - Z(v,j) - \tilde{m}_{uv}(i)\right)^2, \\
		&= \frac{1}{2n'(n'-1)}\sum_{j,h \in \cN_i \times \cN_i} \left((Z(u,j) - Z(v,j)) - (Z(u,h) - Z(v,h))\right)^2, \\
   \mu_{ab} &:= \bE_{\vvec{\bx}^{\pi}_2} \left[ f(a, \vvec{\bx}^{\pi}_2) - f(b, \vvec{\bx}^{\pi}_2) \right],\\
    \sigma_{ab}^2 &:= Var_{\vvec{\bx}^{\pi}_2} \left[ f(a, \vvec{\bx}^{\pi}_2) - f(b, \vvec{\bx}^{\pi}_2) \right].
\end{align*}
As $\ovuvT$ only contains columns $j$ for which both $Z(u,j)$ and $Z(v,j)$ are observed, i.e. $(u,j) \in \cD$ and $(v,j) \in \cD$, the quantities $\muvT$ and $\suvT$ can be computed from the data and are used in the algorithm. $\tilde{m}_{uv}(i)$ and $\tilde{s}^2_{uv}(i)$ is defined from the full matrix $Z$, which is fully determined by the latent row and column latent variables along with the individual noise terms. However, as many entries are unobserved, these quantities are not computable from the data and are defined for the purpose of the analysis. 

\begin{proof}[Proof of Lemma \ref{lem:mean_tensor}]
Without loss of generality, to simplify the notation, assume that $i = (n_{\pi(t_1 + 1)}, \dots n_{\pi(t)})$. Therefore
\begin{align*}
\cN_i &= \{j \in [n] ~s.t.~ j_k \neq i_k \text{ for all } k \in [t_2]\} \\
&= \{j \in [n] ~s.t.~ j_k \in [n_{\pi(t_1 + k)} - 1] \text{ for all } k \in [t_2]\} \\
&= \{j \in [n] ~s.t.~ \vvec{j} \in \times_{k \in [t_2]} [n_{\pi(t_1 + k)} - 1]\}.
\end{align*}
The proof is equivalent for all choice of $i \in [n]$ by symmetry.

By the triangle inequality, 
		$$\left| \muuvT - \muvT \right| \leq \left| \muuvT - \tilde{m}_{uv}(i) \right| + \left| \tilde{m}_{uv}(i) - \muvT \right|.$$
		Therefore, $\left| \muuvT - \muvT \right|  > \mslack$ implies that either $\left| \muuvT - \tilde{m}_{uv}(i) \right|$ or  $\left| \tilde{m}_{uv}(i) - \muvT \right|$ are larger than $\mslack/2$, such that a simple application of union bound results in
	\begin{align*}
		&\Prob{\left|\muvT - \muuvT \right| > \mslack \left| v \in \rowbaseT \right.} \\
	&=	\Prob{\left| \muuvT - \tilde{m}_{uv}(i) \right| + \left| \tilde{m}_{uv}(i) - \muvT \right| > \mslack \left| v \in \rowbaseT \right.} \\
	&\leq	\Prob{\left| \muuvT - \tilde{m}_{uv}(i) \right| > \tfrac{\mslack}{2} \left| v \in \rowbaseT \right.} 	\\
&\qquad	+ 	\Prob{ \left| \tilde{m}_{uv}(i) - \muvT \right| > \tfrac{\mslack}{2} \left| v \in \rowbaseT \right.} 	
	\end{align*}		
		
To bound the first term, we use McDiarmid's inequality (Theorem \ref{thm:McDiarmid}) to show that $\tilde{m}_{uv}(i)$ concentrates around $\muuvT$ due to the sampling of the latent variables and independent noise terms. Conditioned on  $|\ovuvT|$, we bound the second term using the Kontorovich-Ramanan inequality (Theorem \ref{thm:Kontorovich}) to show that $\muvT$ concentrates around $\tilde{m}_{uv}(i)$ since the observed datapoints are sampled without replacement from a finite set of columns. 

To apply McDiarmid's inequality for bounding $\left| \muuvT - \tilde{m}_{uv}(i) \right|$, we define a function $\xi_{ab}$ which maps from the latent variables and noise terms to $\tilde{m}_{uv}(i)$ for $\vvec{x}^{\pi}_1(\vvec{u}) = a$ and $\vvec{x}^{\pi}_1(\vvec{v}) = b$. We show that this function satisfies the bounded difference condition. The entries in row $u$ and $v$ of matrix $Z$ are fully determined by the row latent variables $\vvec{x}^{\pi}_1(\vvec{u})$ and $\vvec{x}^{\pi}_1(\vvec{v})$, the column latent variables $\{\vvec{x}^{\pi}_2(\vvec{j})\}_{j \in \cN_i}$, and the independent noise terms $\{\eta(u,j), \eta(v,j)\}_{j \in \cN_i}$. The $n'$ column latent variables are fully determined by the $\sum_{q \in \cI_2} (n_q - 1)$ latent variables for corresponding coordinates in the tensor. Recall that the number of relevant columns in the flattened matrix is $n' = \prod_{q \in \cI_2} (n_q - 1)$, such that in fact the number of free parameters is significantly smaller than the number of total columns.
Each column latent variable $\vvec{x}^{\pi}_2(\vvec{j})$ is associated to a vector of $t_2$ latent variables in the original tensor, 
	\[\vvec{x}^{\pi}_2 (\vvec{j}) =  \left( x_{\pi(t_1 + 1)} (j_1), \dots, x_{\pi(t_1 + t_2)} (j_{t_2}) \right).\]
Therefore, the set of column latent variables $\{\vvec{x}^{\pi}_2(\vvec{j})\}_{j \in \cN_i}$ is fully determined by the corresponding latent variables in the $t_2$ dimensions of the original tensor, described by the sets $\{x_{\pi(t_1 + 1)} (j)\}_{j \in [n_{\pi(t_1+1)} -1]},  \dots, \{x_{\pi(t_1 + t_2)} (j)\}_{j \in [n_{\pi(t_1 + t_2)} - 1]}$. 

For a pair of row latent variables $a,b \in \cX^{\pi}_1$, we construct function $\xi_{ab}$ to map from the column latent variables and individual noise terms to $\tilde{m}_{uv}(i)$ conditioned on $ \vvec{x}^{\pi}_1(\vvec{u}) = a, \vvec{x}^{\pi}_1(\vvec{v}) = b$,
\begin{align*}
\xi_{ab}: \times_{q \in \cI_2} (\cX_q)^{n_q - 1} \times \Reals^{2n'} \to \Reals.
\end{align*}
The function $\xi_{ab}$ is defined according to
    \begin{align}
        &\xi_{ab}\Big(\{x_q(l)\}_{q \in \cI_2, l \in [n_q - 1]},  \{\eta(u,j), \eta(v,j)\}_{j \in \cN_i}\Big) \nonumber \\
         &\qquad = \frac{1}{n'} \sum_{j \in \cN_i} \left( f\left(a, \vvec{x}^{\pi}_2(\vvec{j})\right) + \eta(u,j) - f\left( b, \vvec{x}^{\pi}_2(\vvec{j})\right) - \eta(v,j) \right)   \label{eq:def_xi_ab}
    \end{align}
    where $\vvec{x}^{\pi}_2(\vvec{j}) = \left( x^{\pi}_{2,1}(j_1), \ldots, x^{\pi}_{2, t_2}(j_{t_2}) \right)$.
		We will overload the notation and also let $\xi_{ab}$ denote the random variable which is evaluated with respect to the column latent variables and noise terms, leaving out the terms in the parentheses for readability. We can verify that by construction, 
		$$\xi_{\vvec{x}^{\pi}_1(\vvec{u}) \vvec{x}^{\pi}_1(\vvec{v})} = \tilde{m}_{uv}(i).$$
		Since the noise terms are zero-mean and $\vvec{x}^{\pi}_2(\vvec{j})$ are identically distributed for all $j \in [n]$,
		$$ \bE \xi_{ab} = \bE_{\bx^{\pi}_2} \left[ f(a, \bx^{\pi}_2) - f(b, \bx^{\pi}_2) \right] = \mu_{ab}.$$
		
		For any tensor dimension $q \in \cI_2$ and for any coordinate $l \in [n_q - 1]$, the associated latent variable $x_q(l)$ shows up in exactly $\frac{n'}{n_q - 1}$ terms of the summation in \eqref{eq:def_xi_ab}. We assumed in our model that the function $f$ is $L$-Lipschitz such that by for any $a,b \in \cX^{\pi}_1$ and $x_2 \in \cX^{\pi}_2$, 
		$$\left| f\left(a,x_2\right) - f\left( b,x_2\right) \right| \leq L D_{\cX^{\pi}_1},$$
where we recall that $D_{\cX^{\pi}_1}$ is the diameter of $\cX^{\pi}_1$. Since the above expression only takes values within $[-L D_{\cX^{\pi}_1}, L D_{\cX^{\pi}_1}]$, this implies that if we changed a single variable $x_q(l)$ arbitrarily, for each of the $\frac{n'}{n_q - 1}$ terms which it participates in, the value will at most change by $2 L D_{\cX^{\pi}_1}$, which is then divided by $n'$ from the term in front of the summation. Thus, the overall value of $\xi_{ab}$ can change at most by $\frac{2LD_{\cX^{\pi}_1}}{n_q - 1}$ when a single latent variable is changed arbitrarily.

For any $j \in \cN_i$, the noise variables $\eta(u,j)$ and $\eta(v,j)$ each only show up in a single term of the summation in \eqref{eq:def_xi_ab}. Furthermore, we assumed in our model statement that the noise is bounded, i.e. $\eta(u,j) \in [-B_e, B_e]$.  Thus, the overall value of $\xi_{ab}$ can change at most by $\frac{2 B_e}{n'}$ when a single additive noise variable is changed arbitrarily.
    
%    \dogyoon{***TODO: May want to discuss this more carefully} In fact there are $2n$ independent noise terms, for which the functional difference is bounded by $\frac{2B_e}{n}$. The contribution of these noise terms slightly degrades the tail bound to follow.    
      By McDiarmid's inequality, we can conclude that for any $\mslack > 0$ and $u,v \in [m]$,
    \begin{align*}
    &\Prob{\left|\tilde{m}_{uv}(i) - \muuvT\right| \geq \tfrac{\mslack}{2} ~|~ \vvec{x}^{\pi}_1(\vvec{u}) = a, \vvec{x}^{\pi}_1(\vvec{v})=b } \\
				&\qquad= \Prob{\left|\xi_{ab} - \bE \xi_{ab}\right| \geq \tfrac{\mslack}{2}} \\
        	   &\qquad\leq 2\exp\left(\frac{-\mslack^2}{8 (LD_{\cX^{\pi}_1})^2 \sum_{q \in \cI_2} \frac{1}{n_q - 1} + \frac{16B_e^2}{n'}}\right).
    \end{align*}
		Observe that $v \in \rowbaseT $ only depends on the locations of observed samples, specified by the set of data indices $\cD$, whereas $\tilde{m}_{uv}(i)$ and $\muuvT$ are completely independent from $\cD$. Additionally since the upper bound does not depend on $a$ and $b$, it follows that
$$\Prob{\left|\tilde{m}_{uv}(i) - \muuvT\right| \geq \tfrac{\mslack}{2} ~|~ v \in \rowbaseT} \leq 2\exp\left(\frac{-\mslack^2}{8(LD_{\cX^{\pi}_1})^2 \sum_{q \in \cI_2} \frac{1}{n_q - 1} + \frac{16B_e^2}{n'}}\right).$$
	
	
Next, we bound $\left| \tilde{m}_{uv}(i) - \muvT \right|$ using the Kontorovich-Ramanan inequality.
Recall that the set $\ovuvT$ denotes the columns in $\cN_i$ for which samples have been observed from both rows $u$ and $v$. Suppose that $\left| \ovuvT \right| = k$, such that $\ovuvT $ can be viewed as $k$ randomly chosen columns out of $n'$ total columns. This is equivalent to drawing $k$ elements uniformly at random from a finite population of $n'$ without replacement. We will define a function $\psi_{uvk}$ which maps from the $k$ sampled columns to the quantity $\muvT$,
$$\psi_{uvk}: \cN_i^k \to \Reals.$$
Let $J_1 \ldots J_k \in \cN_i$ denote the randomly selected column indices, then 
 $$\psi_{uvk}(\{J_1, \ldots, J_k\}) = \frac{1}{k} \sum_{l=1}^k (Z(u, J_l) - Z(v,J_l)).$$
We can verify that by construction, conditioned on $|\ovuvT| = k$, 
 $$\psi_{uvk}(\ovuvT) = \muvT \text{ and } \E[\psi_{uvk}(\ovuvT)] = \tilde{m}_{uv}(i).$$
For any two sequences $\{J_l\},\{J'\} \in \cN_i^k$, the function values differ by
\begin{align*}
&\psi_{uvk}(\{J_1, \ldots, J_k\}) - \psi_{uvk}(\{J'_1, \ldots, J'_k\}) \\
&\qquad= \frac{1}{k} \sum_{l=1}^k (Z(u, J_l) - Z(v,J_l) - Z(u, J'_l) + Z(v,J'_l)) \\
&\qquad= \frac{1}{k} \sum_{l: J_l \neq J'_l} (Z(u, J_l) - Z(v,J_l) - Z(u, J'_l) + Z(v,J'_l)).
\end{align*}
Recall that by definition of $B_0$ in \eqref{eq:def_B0_tensor}, for any $u, v \in [m]$ and $i \in [n]$, 
$$\left| Z(u,i) - Z(v,i) \right| \leq B_0,$$
since the latent space and noise terms are bounded. Therefore, if we consider the Hamming metric on $\cN_i^k$, we can verify that $\psi_{uvk}(\cdot)$ is $(\frac{2 B_0}{k})$-Lipschitz, since
\begin{align*}
\psi_{uvk}(\{J_1, \ldots, J_k\}) - \psi_{uvk}(\{J'_1, \ldots, J'_k\}) 
\leq \frac{2 B_0}{k} |\{l: J_l \neq J'_l\}|.
\end{align*}

Next we compute the mixing coefficient of the randomly chosen columns $\ovuvT = \{J_1, \dots J_k\}$, as defined in the setup of the Kontorovich-Ramanan inequality (see Theorem \ref{thm:Kontorovich} in Appendix \ref{sec:aux_concentration} for details). The sequence of columns $(J_1, \dots, J_k)$ is uniformly distributed amongst all $\frac{n'!}{(n'-k)!}$ possible sequences of choosing $k$ columns out of $n'$ total columns without replacement. The mixing coefficient $\Delta_k$ is defined according to
$\Delta_k := \max_{s \in [k]} \left( 1 + \sum_{s'=s+1}^k \bar{\lambda}_{ss'}  \right)$, where
\begin{align*}
    \bar{\lambda}_{ss'} := \sup_{\vvec{\tau} \in \cN_i^{s-1},  \atop w, \hat{w} \in \cN_i} 
\frac{1}{2}\sum_{\vvec{\tau}' \in \cN_i^{k-{s'}+1}} \Big| &\Prob{(J_{s'} \dots J_k) = \vvec{\tau}' ~|~ (J_1 \dots J_s) = (\vvec{\tau}, w)} \\
&\qquad- \Prob{(J_{s'} \dots J_k) = \vvec{\tau}' ~|~ (J_1 \dots J_s) = (\vvec{\tau}, \hat{w})} \Big|,
\end{align*}
where the supremum is only taken over valid sequences $(\vvec{\tau}, w)$ and $(\vvec{\tau}, \hat{w})$ which do no repeat any elements. 

Conditioned on $(J_1 \dots J_s) = (\vvec{\tau}, w)$, the sequence $(J_{s'} \dots J_k)$ is equally likely amongst all sequences of length $(k-s' + 1)$ chosen from the $n'$ columns without replacement as long as they also do not repeat any elements already chosen in the vector $(\vvec{\tau}, w)$, i.e. all permutations of length $(k-s' + 1)$ out of $n' - s$ remaining columns. Similarly, conditioned on $(J_1 \dots J_s) = (\vvec{\tau}, \hat{w})$, the sequence $(J_{s'} \dots J_k)$ is equally likely amongst all permutations of length $(k-s' + 1)$ out of the $n' - s$ remaining columns that do not contain any elements in $(\vvec{\tau}, \hat{w})$. There are a total of $\frac{(n'-s)!}{((n'-s)-(k-s'+1))!}$ such valid permutations.

Therefore, if $\tau'$ does not contain symbols $w$ or $\hat{w}$, then the probability of $(J_{s'} \dots J_k)$ $= \vvec{\tau}'$ is equal whether conditioned on $(J_1 \dots J_s)$ $= (\vvec{\tau}, w)$ or $(J_1 \dots J_s) = (\vvec{\tau}, \hat{w})$. If $\tau'$ contains both $w$ and $\hat{w}$, then it will have probability zero in both conditioned events. If $\tau'$ contains only one out of either $w$ or $\hat{w}$, then the absolute value of the difference in the conditional probabilities of $(J_{s'} \dots J_k) = \vvec{\tau}'$ will be equal to $\frac{((n'-s)-(k-s'+1))!}{(n'-s)!}$. The total number of such sequences $\tau'$ which contain only one out of either $w$ or $\hat{w}$ (and do not repeat elements in $\tau$) is equal to $2(k-s'+1) \frac{(n'-s-1)!}{((n'-s-1)-(k-s'))!}= \frac{2(k-s'+1)}{n'-s}\frac{(n'-s)!}{((n'-s)-(k-s'+1))!}$ . Therefore,
\begin{align*}
    \bar{\lambda}_{ss'} &= \frac{(k-s'+1)}{n'-s} \frac{(n'-s)!}{((n'-s)-(k-s'+1))!} \frac{((n'-s)-(k-s'+1))!}{(n'-s)!} \\
		&= \frac{(k-s'+1)}{n'-s}. 
\end{align*}

We can then compute the mixing coefficient $\Delta_k$, 
\begin{align}
\Delta_k %&= \max_{s \in [k]} \left( 1 + \sum_{s'=s+1}^k \bar{\lambda}_{ss'}  \right) \\
&= \max_{s \in [k]} \left( 1 + \sum_{s'=s+1}^k  \frac{(k-s'+1)}{n'-s} \right) \\
%&= \max_{s \in [k]} \left( 1 + \frac{1}{n-s} \sum_{s'=1}^{k-s}  (k-s-s'+1) \right) \\
%&= \max_{s \in [k]} \left( 1 + \frac{1}{n-s} \left((k-s+1)(k-s) - \sum_{s'=1}^{k-s} s' \right) \right)\\
%&= \max_{s \in [k]} \left( 1 + \frac{1}{n-s} \left((k-s+1)(k-s) - (k-s)(k-s+1)/2 \right) \right) \\
&= \max_{s \in [k]} \left( 1 + \frac{(k-s)(k-s+1)}{2(n'-s)}\right)	\label{eqn:mixing_coeff} \\
&= 1 + \frac{(k-1)k}{2(n'-1)}.
\end{align}
The last step follows from showing that the derivative with respect to $s$ is negative, such that the expression is maximized for the smallest value of $s$, which is $s = 1$.

Consequently, it follows from the Kontorovich-Ramanan theorem (Theorem \ref{thm:Kontorovich}) that for any $\mslack > 0$,
    \begin{align*}
        \Prob{\left|\muvT - \tilde{m}_{uv}(i)\right| \geq \tfrac{\mslack}{2} ~\left|~ |\ovuvT| = k\right.} 
				&=\Prob{\left|\psi_{uvk} - \bE \psi_{uvk}\right| \geq \tfrac{\mslack}{2} }\\
        	   &\leq 2\exp\left(\frac{-\mslack^2}{8 k \left(\frac{2B_0}{k} \right)^2 \left(1 + \frac{(k-1)k}{2(n'-1)}\right)^2  }\right)\\
	   &= 2\exp\left(\frac{- k \mslack^2}{32 B_0^2\left(1 + \frac{(k-1)k}{2(n'-1)}\right)^2  }\right)\\
	   &\leq 2 \exp \left(\frac{- \mslack^2}{32 B_0^2}  \frac{n'^2k}{\left( n' + k^2\right)^2}\right).
    \end{align*}
   The last inequality follows when we assume that $n' \geq 2$. Then $2('n-1) \geq n'$ and $1 + \frac{(k-1)k}{2(n'-1)} \leq 1 + \frac{k^2}{n'}$, hence, $\frac{k}{\left( 1+ \frac{(k-1)k}{2(n'-1)}\right)^2} \geq \frac{k}{\left( 1+ \frac{k^2}{n'}\right)^2} = \frac{n'^2k}{\left( n' + k^2 \right)^2}$. 
	
	We would like to compute a lower bound that holds for all $k$. By taking the derivative with respect to $k$,
   $$   \frac{\partial}{\partial k} \frac{n'^2k}{(n'+k^2)^2} = \frac{n'^2 (n'+k^2)(n'-3k^2)}{(n'+k^2)^4}.  $$ 
 Therefore, $\frac{n'^2k}{\left( n' + k^2 \right)^2}$ is monotone increasing for $k\leq \sqrt{\frac{n'}{3}}$, and monotone decreasing for $k > \sqrt{\frac{n'}{3}}$. In other words, for any $k \in [\beta_l, \beta_h]$,
   $$\frac{n'^2k}{\left( n' + k^2 \right)^2} \geq \min \left\{\frac{n'^2\beta_l}{\left( n' + \beta_l^2 \right)^2}, \frac{n'^2\beta_h}{\left( n' + \beta_h^2 \right)^2} \right\} =: \Delta.$$
  Therefore,
	    \begin{align*}
        &\Prob{\left|\muvT - \tilde{m}_{uv}(i)\right| \geq \tfrac{\mslack}{2} ~\left|~ v \in \rowbaseT \right.} \\
				&\qquad= \Prob{\left|\muvT - \tilde{m}_{uv}(i)\right| \geq \tfrac{\mslack}{2} ~\left|~ |\ovuvT| \in [\beta_l, \beta_h]\right.} \\
				&\qquad\leq 2 \exp \left(\frac{- \mslack^2}{32B_0^2}  \Delta \right).
	\end{align*}
	
	Finally, we combine the two bounds to obtain the final result.
    
\end{proof}    
    

%%% Lemma: Tensor Variance Concentration
\begin{proof} [Proof of Lemma \ref{lem:variance_tensor}]
Without loss of generality, to simplify the notation, assume that $i = (n_{\pi(t_1 + 1)}, \dots n_{\pi(t)})$. Therefore
\begin{align*}
\cN_i &= \{j \in [n] ~s.t.~ j_k \neq i_k \text{ for all } k \in [t_2]\} \\
&= \{j \in [n] ~s.t.~ j_k \in [n_{\pi(t_1 + k)} - 1] \text{ for all } k \in [t_2]\} \\
&= \{j \in [n] ~s.t.~ \vvec{j} \in \times_{k \in [t_2]} [n_{\pi(t_1 + k)} - 1]\}.
\end{align*}
The proof is equivalent for all choice of $i \in [n]$ by symmetry. Recall that $|\cN_i| = n' = \prod_{q \in \cI_2} (n_q - 1)$.


    In this proof, we will show concentration of $\suvT$ to $\bE \tilde{s}^2_{uv}(i)$, and then show that $\bE \tilde{s}^2_{uv}(i)$ conditioned on $\vvec{x}^{\pi}_1(\vvec{u})$ and $\vvec{x}^{\pi}_1(\vvec{v})$ is approximately equal to $\siguvT^2 + 2\gamma^2$. By the triangle inequality, 
    \[	\left| \bE \tilde{s}^2_{uv}(i) - \suvT \right| \leq \left| \bE \tilde{s}^2_{uv}(i) - \tilde{s}^2_{uv}(i)  \right| + \left| \tilde{s}^2_{uv}(i) - \suvT \right|.	\]
    In a similar vein as in the proof of the Lemma \ref{lem:mean_tensor}, $\left| \bE \tilde{s}^2_{uv}(i) - \suvT \right| > \vslack$ implies that either $\left| \bE \tilde{s}^2_{uv}(i) - \tilde{s}^2_{uv}(i)  \right| > \vslack/2$ or $\left| \tilde{s}^2_{uv}(i) - \suvT \right| > \vslack/2$. Again, a simple application of union bound results in 
    \begin{align*}
    	&\Prob{\left| \bE \tilde{s}^2_{uv}(i) - \suvT \right| > \vslack ~\left|~  v \in \rowbaseT \right.}\\
		&\leq \Prob{\left. \left| \bE \tilde{s}^2_{uv}(i) - \tilde{s}^2_{uv}(i)  \right| > \frac{\vslack}{2} \right| v \in \rowbaseT } + \Prob{\left. \left| \tilde{s}^2_{uv}(i) - \suvT \right| > \frac{\vslack}{2} \right|v \in \rowbaseT}
    \end{align*}

    To apply McDiarmid's inequality for bounding $\left| \bE \tilde{s}^2_{uv}(i) - \tilde{s}^2_{uv}(i)  \right|$, we define a function $\xi_{ab}$ which maps from the latent variables and noise terms to $\tilde{s}^2_{uv}(i)$ for $\vvec{x}^{\pi}_1(\vvec{u}) = a$ and $\vvec{x}^{\pi}_1(\vvec{v}) = b$. We show that this function satisfies the bounded difference condition. The entries in row $u$ and $v$ of matrix $Z$ are fully determined by the row latent variables $\vvec{x}^{\pi}_1(\vvec{u})$ and $\vvec{x}^{\pi}_1(\vvec{v})$, the column latent variables $\{\vvec{x}^{\pi}_2(\vvec{j})\}_{j \in \cN_i}$, and the independent noise terms $\{\eta(u,j), \eta(v,j)\}_{j \in \cN_i}$. 
    %The $n$ column latent variables are fully determined by the $\sum_{q \in \cI_2} n_q$ latent variables for corresponding coordinates in the tensor. Recall that the number of columns in the flattened matrix is $n = \prod_{q \in \cI_2} n_q$, such that in fact the number of free parameters is significantly smaller than the number of total columns. Each column latent variable $\vvec{x}^{\pi}_2(\vvec{j})$ is associated to a vector of $t_2$ latent variables in the original tensor, 
%    	\[\vvec{x}^{\pi}_2 (\vvec{j}) =  \left( x_{\pi(t_1 + 1)} (j_1), \dots, x_{\pi(t_1 + t_2)} (j_{t_2}) \right).\]
%Therefore, the set of column latent variables $\{\vvec{x}^{\pi}_2(\vvec{j})\}_{j \in [n]}$ is fully determined by the corresponding latent variables in the $t_2$ dimensions of the original tensor, described by the sets $\{x_{\pi(t_1 + 1)} (j)\}_{j \in [n_{\pi(t_1+1)}]},  \dots, \{x_{\pi(t_1 + t_2)} (j)\}_{j \in n_{\pi(t_1 + t_2)}}$. 

	For a pair of row latent variables $a,b \in \cX^{\pi}_1$, we construct function $\xi_{ab}$ to map from the column latent variables and individual noise terms to $\tilde{s}^2_{uv}(i)$ conditioned on $ \vvec{x}^{\pi}_1(\vvec{u}) = a, \vvec{x}^{\pi}_1(\vvec{v}) = b$,
\begin{align*}
\xi_{ab}: \times_{q \in \cI_2} (\cX_q)^{n_q-1} \times \Reals^{2n'} \to \Reals.
\end{align*}
We define $f_{ab}$ and $\eta_{uv}$ according to
\begin{align*}
f_{ab}\left( x \right) &= f(a,x) - f(b,x), \\
\eta_{uv}(j) &= \eta(u,j) - \eta(v,j).
\end{align*}
The function $\xi_{ab}$ is defined according to
    \begin{align}
        &\xi_{ab}\Big(\{x_q(l)\}_{q \in \cI_2, l \in [n_q-1]},  \{\eta(u,j), \eta(v,j)\}_{j \in \cN_i}\Big) \nonumber \\
         &\qquad = \frac{1}{2n'(n'-1)} \sum_{j, h \in \cN_i \times \cN_i} \left( f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(j) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right) - \eta_{uv}(h) \right)^2   \label{eq:def_xi_ab_var}
    \end{align}
    where $\vvec{x}^{\pi}_2(\vvec{j}) = \left( x^{\pi}_{2,1}(j_1), \ldots, x^{\pi}_{2, t_2}(j_{t_2}) \right)$.
		We will overload the notation and also let $\xi_{ab}$ denote the random variable which is evaluated with respect to the column latent variables and noise terms, leaving out the terms in the parentheses for readability. We can verify that by construction, 
\begin{align*}
\xi_{\vvec{x}^{\pi}_1(\vvec{u}) \vvec{x}^{\pi}_1(\vvec{v})} = \tilde{s}^2_{uv}(i) \text{ and }
\bE \xi_{ab} &= \bE\left[\left.  \tilde{s}^2_{uv}(i) \right| \vvec{x}^{\pi}_1(\vvec{u})=a, \vvec{x}^{\pi}_1(\vvec{v})=b \right].
\end{align*}

%By Equation \eqref{eq:var_sym} is derived from the symmetry (exchangeability implies identical distribution) and the linearity of expectation, and \eqref{eq:var_simp} follows from the observation that
    %\begin{align}
         %\bE \xi_{ab} &= \bE\left[\left.  \tilde{s}^2_{uv}(i) \right| \vvec{x}^{\pi}_1(\vvec{u})=a, \vvec{x}^{\pi}_1(\vvec{v})=b \right]	\nonumber\\
        		%&= \Exp{ \frac{1}{2 n(n-1)} \sum_{j \in [n] }\sum_{h \in [n]} \left( f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j}) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h}) - \eta_{uv}(\vvec{h})\right) \right)^2}	\nonumber\\
		%&= \frac{1}{2(n-1)}\Exp{\sum_{h } \left( f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{1})\right) + \eta_{uv}(\vvec{1}) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right) - \eta_{uv}(\vvec{h}) \right)^2}	\label{eq:var_sym}\\
		%&= \frac{1}{2(n-1)} \sum_{j'} \left[ Var_{\vvec{1}} - 2Cov_{\vvec{1} \vvec{j'}}+ Var_{\vvec{j'}}  \right]	\label{eq:var_simp}\\
		%&= \frac{1}{n-1} \sum_{j'}\left[ Var_{\vvec{1}} - Cov_{\vvec{1} \vvec{j'}}\right]	\label{eq:var_final}.
    %\end{align}
    %where the shorthand notations stand for $Var_j := Var \left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j})\right)$ and $Cov_{\vvec{j}\vvec{j'}} := Cov\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j}), f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j'})\right) + \eta_{uv}(\vvec{j'}) \right)$, respectively.  
    
     For any tensor dimension $q \in \cI_2$ and for any coordinate $l \in [n_q-1]$, the associated latent variable $x_q(l)$ shows up in at most $\frac{2n'(n'-1)}{n_q-1}$ terms out of $n'(n'-1)$ of the summation in \eqref{eq:def_xi_ab_var}, used to evaluate $\xi_{ab}$. We assumed in our model that the function $f$ is $L$-Lipschitz such that by for any $a,b \in \cX^{\pi}_1$ and $x_2 \in \cX^{\pi}_2$, 
		$$\left| f\left(a,x_2\right) - f\left( b,x_2\right) \right| \leq L D_{\cX^{\pi}_1},$$
where we recall that $D_{\cX^{\pi}_1}$ is the diameter of $\cX^{\pi}_1$.Therefore, 
\[	\left| f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j'})\right)  \right| \leq 2LD_{\cX^{\pi}_1}.	\]
We assumed that the noise was bounded such that $|\eta_{uv}(j)| \leq 2 B_e$. Therefore, 
$$\left| f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(j) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j'})\right) - \eta_{uv}(j') \right| \leq 2L D_{\cX^{\pi}_1} + 4 B_e.$$
If we changed a single variable $x_q(l)$ arbitrarily,  for each of the $\frac{2n'(n'-1)}{n_q-1}$ terms which it participates in, the value of the summand
\[	\left[ f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(j) - f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j'})\right) - \eta_{uv}(j') \right]^2	\]
will at most change by $2 \left( 2LD_{\cX^{\pi}_1} + 4B_e \right) \left( 2LD_{\cX^{\pi}_1} \right) + \left(2LD_{\cX^{\pi}_1}\right)^2 $ because if we consider a perturbation $\Delta$, $(X + \Delta)^2 - X^2 = 2X \Delta + \Delta^2$, which is then divided by $2n'(n'-1)$ from the term in front of the summation. Thus, the overall value of $\xi_{ab}$ can change at most by 
$$\frac{1}{n_q-1}\left( 2 \left( 2LD_{\cX^{\pi}_1} + 4B_e \right) \left( 2LD_{\cX^{\pi}_1} \right) + \left(2LD_{\cX^{\pi}_1}\right)^2 \right) = \frac{4 LD_{\cX^{\pi}_1}}{n_q-1} \left(3LD_{\cX^{\pi}_1} + 4B_e\right)$$
when a single latent variable is changed arbitrarily.
%\dogyoon{Perhaps we should further upper bound $LD_{\cX^{\pi}_1}$ by $B_0$}

For any $j \in \cN_i$, the noise variables $\eta(u,j)$ and $\eta(v,j)$ each shows up in exactly $2(n'-1)$ terms of the summation in \eqref{eq:def_xi_ab_var}. Furthermore, we assumed in our model statement that the noise is bounded, i.e. $\eta(u,j) \in [-B_e, B_e]$.  Thus, by a similar argument as above, the overall value of $\xi_{ab}$ can change at most by 
$$\frac{1}{n'} \left[ 2 \left( 2LD_{\cX^{\pi}_1} + 4B_e \right) \left( 2B_e \right) + \left(2B_e\right)^2 \right] = \frac{4B_e}{n'} \left( 2LD_{\cX^{\pi}_1} + 5 B_e\right)$$
when a single additive noise variable is changed arbitrarily.
    
    By McDiarmid's inequality, we can conclude that for any $\vslack > 0$ and $u,v \in [m]$,
    \begin{align*}
    &\Prob{\left|\tilde{s}^2_{uv}(i) - \bE \tilde{s}^2_{uv}(i) \right|  \geq \tfrac{\vslack}{2} ~|~ \vvec{x}^{\pi}_1(\vvec{u}) = a, \vvec{x}^{\pi}_1(\vvec{v})=b } \\
				&\qquad= \Prob{\left|\xi_{ab} - \bE \xi_{ab}\right| \geq \tfrac{\vslack}{2}} \\
        	   &\qquad\leq 2\exp\left(\frac{-\vslack^2}{32L^2D_{\cX^{\pi}_1}^2\left( 3LD_{\cX^{\pi}_1} + 4 B_e\right)^2\sum_{q=1}^{t_2} \frac{1}{n_q - 1} + \frac{64B_e^2\left( 2LD_{\cX^{\pi}_1} + 5 B_e\right)^2}{n'}}\right).
    \end{align*}
		Observe that $v \in \rowbaseT $ only depends on the locations of observed samples, specified by the set of data indices $\cD$, whereas $\tilde{s}_{uv}$ and $\siguvT$ are completely independent from $\cD$. Additionally since the upper bound does not depend on $a$ and $b$, it follows that
\begin{align*}
	&\Prob{\left|  \tilde{s}^2_{uv}(i) - \bE \tilde{s}^2_{uv}(i)  \right| \geq \tfrac{\vslack}{2} ~|~ v \in \rowbaseT}\\
	&\qquad \leq 2\exp\left(\frac{-\vslack^2}{32L^2D_{\cX^{\pi}_1}^2\left( 3LD_{\cX^{\pi}_1} + 4 B_e\right)^2\sum_{q=1}^{t_2} \frac{1}{n_q - 1} + \frac{64B_e^2\left( 2LD_{\cX^{\pi}_1} + 5 B_e\right)^2}{n'}}\right).
\end{align*}

		%\chris{getting rid of $\tilde{\sigma}$ because it's only used once ...}
  Next, we bound $\left| \tilde{s}^2_{uv}(i) - \suvT \right|$ using the Kontorovich-Ramanan inequality. Recall that the set $\ovuvT$ denotes the columns for which samples have been observed from both rows $u$ and $v$. Suppose that $\left| \ovuvT \right| = k$, such that $\ovuvT $ can be viewed as $k$ randomly chosen columns out of $n'$ total columns. This is equivalent to drawing $k$ elements uniformly at random from a finite population of $n'$ without replacement. We will define a function $\psi_{uvk}: \cN_i^k \to \Reals$, which maps from the $k$ sampled columns to the quantity $\suvT$.
Let $J_1 \ldots J_k \in \cN_i$ denote the selected column indices, then 
 \begin{align}
&\psi_{uvk}(\{J_1, \ldots, J_k\}) \nonumber \\
&= \frac{1}{2k(k-1)} \sum_{l=1}^k \sum_{l'=1}^k \left( Z(u, J_l) - Z(v,J_l) - Z(u, J_{l'}) + Z(v,J_{l'})\right)^2. \label{eq:def_psi_var}
\end{align}
We can verify that by construction, conditioned on $|\ovuvT| = k$, $\psi_{uvk}(\ovuvT) = \suvT$. Next we show that its expectation conditioned on the matrix $Z$ equals $\tilde{s}^2_{uv}(i)$. Since we condition on the matrix $Z$, the randomness only comes from the randomly sampled columns $\ovuvT = \{J_l\}_{l \in [k]}$. Observe that the randomly chosen column indices $J_l$ and $J_{l'}$ are identically distributed, and thus $Z(u,J_l) -Z(v, J_l)$ and $Z(u,J_{l'}) - Z(v,J_{l'})$ are also identically distributed. Recall from \eqref{eq:exp_sqdiff_id} that if two variables are identically distributed, then the expectation of the square of their difference is equal to two times the variance minus the covariance. Therefore if we let $X_l := Z(u, J_l) - Z(v,J_l)$, 
\begin{align*}
\Exp{\psi_{uvk}(\ovuvT)} &= \frac{1}{k (k-1)} \sum_{l=1}^k \sum_{l'=1}^k \left( \Var[X_l] - \Cov[X_l, X_{l'}] \right) \\
&= \Var[X_l] - \frac{1}{k (k-1)} \sum_{l=1}^k \sum_{l'\neq l} \Cov[X_l, X_{l'}]. 
\end{align*}
Conditioned on $Z$, for $l \neq l'$, the random variables $X_l$ and $X_{l'}$ are determined by the sampled columns $J_l$ and $J_{l'}$, which can be viewed as two samples drawn from a finite population of size $n'$ without replacement. Therefore, their covariance is equal to $-\frac{1}{n'-1}$ times the variance of the population. Therefore,
\begin{align*}
\Exp{\psi_{uvk}(\ovuvT)} 
= \Var[X_l] + \frac{1}{k (k-1)(n'-1)} \sum_{l=1}^k \sum_{l'\neq l} \Var[X_l] 
= \frac{n'}{(n'-1)} \Var[X_l]. 
\end{align*}
By construction, conditioned on $Z$, the variance of $X_l$ with respect to the randomly chosen column index $J_l$ is equal to $\frac{n'-1}{n'}\tilde{s}^2_{uv}(i)$, and the mean of $X_l$ with respect to the randomly chosen column index $J_l$ is equal to $\tilde{m}_{uv}$. Therefore $\Exp{\psi_{uvk}(\ovuvT)}  = \tilde{s}^2_{uv}(i)$.
 
Next we show that the function $\psi_{uvk}$ is Lipschitz with respect to the Hamming metric on $\cN_i^k$, and we compute the associated Lipschitz constant.
The definition of $\psi_{uvk}$ in \eqref{eq:def_psi_var} involves a double summation, and a particular index variable $J_l$ shows up in exactly $2(k-1)$ of these terms in the summation. Consider two sets of column indices $\{J_l \in \cN_i\}_{l \in [k]}$ and $\{J'_l \in \cN_i\}_{l \in [k]}$. For each position $l_0$ at which they differ, i.e. $J_{l_0} \neq J'_{l_0}$, we can bound the maximum resulting difference in the function value of $\psi_{uvk}$. By definition of $B_0$ in \eqref{eq:def_B0_tensor}, for any $u, v \in [m]$ and $i \in [n]$, $ \left|Z(u, i) - Z(v, i) \right| \leq B_0,$ since the latent space and noise terms are bounded. For any $J_l, J'_l \in [n]$, it follows that 
	\[\left( Z(u, J_l) - Z(v, J_l) - Z(u, J'_l) + Z(v, J'_l) \right)^2 \leq 4 B_0^2.\]
The difference in the value of $\psi_{uvl}$ evaluated with column indices $\{J_l\}_{l \in [k]}$ versus $\{J'_l\}_{l \in [k]}$ is bounded above by
\begin{align*}
	\psi_{uvk}(\{J_l\}_{l \in [k]}) - \psi_{uvk}(\{J'_l\}_{l \in [k]})  
	&\leq \frac{1}{2k(k-1)} 2(k-1) |\{l: J_l \neq J'_l\}| (4B_0^2) \\
	&= \frac{4B_0^2}{k} |\{l: J_l \neq J'_l\}|.
\end{align*}
Therefore, if we consider the Hamming metric on $\cN_i^k$, the function $\psi_{uvk}(\cdot)$ is $\left(\frac{4B_0^2}{k}\right)$-Lipschitz.

Next we compute the mixing coefficient of the randomly chosen columns $\ovuvT = \{J_1, \dots J_k\}$, as defined in the setup of the Kontorovich-Ramanan inequality (see Theorem \ref{thm:Kontorovich} in Appendix \ref{sec:aux_concentration} for details). This is exactly the same with the argument in the proof of Lemma \ref{lem:mean_tensor}. We just restate the mixing coefficient $\Delta_k$ obtained in \eqref{eqn:mixing_coeff}: 
\[	\Delta_k = 1 + \frac{(k-1)k}{2(n'-1)}.	\]
Consequently, it follows from the Kontorovich-Ramanan theorem (Theorem \ref{thm:Kontorovich}) that for any $\mslack > 0$,
    \begin{align*}
        \Prob{\left|\suvT - \tilde{s}^2_{uv}(i)\right| \geq \tfrac{\vslack}{2} ~\left|~ |\ovuvT| = k\right.} 
				&=\Prob{\left|\psi_{uvk} - \bE \psi_{uvk}\right| \geq \tfrac{\vslack}{2} }\\
        	   &\leq 2\exp\left(\frac{-\vslack^2}{8 k \left(\frac{4B_0^2}{k} \right)^2 \left(1 + \frac{(k-1)k}{2(n'-1)}\right)^2  }\right)\\
	   &= 2\exp\left(\frac{- k \vslack^2}{128 B_0^4\left(1 + \frac{(k-1)k}{2(n'-1)}\right)^2  }\right)\\
	   &\leq 2 \exp \left(\frac{- \vslack^2}{128 B_0^4}  \frac{n'^2k}{\left( n' + k^2\right)^2}\right).
    \end{align*}
   The last inequality follows when we assume that $n' \geq 2$. Then $2(n'-1) \geq n'$ and $1 + \frac{(k-1)k}{2(n'-1)} \leq 1 + \frac{k^2}{n'}$, hence, $\frac{k}{\left( 1+ \frac{(k-1)k}{2(n'-1)}\right)^2} \geq \frac{k}{\left( 1+ \frac{k^2}{n'}\right)^2} = \frac{n'^2k}{\left( n' + k^2 \right)^2}$. 
	
	We would like to compute a lower bound that holds for all $k$. By taking the derivative with respect to $k$,
   $$   \frac{\partial}{\partial k} \frac{n'^2k}{(n'+k^2)^2} = \frac{n'^2 (n'+k^2)(n'-3k^2)}{(n'+k^2)^4}.  $$ 
 Therefore, $\frac{n'^2k}{\left( n' + k^2 \right)^2}$ is monotone increasing for $k\leq \sqrt{\frac{n'}{3}}$, and monotone decreasing for $k > \sqrt{\frac{n'}{3}}$. In other words, for any $k \in [\beta_l, \beta_h]$,
   $$\frac{n'^2k}{\left( n' + k^2 \right)^2} \geq \min \left\{\frac{n'^2\beta_l}{\left( n' + \beta_l^2 \right)^2}, \frac{n'^2\beta_h}{\left( n' + \beta_h^2 \right)^2} \right\} =: \Delta.$$
  Therefore,
	    \begin{align*}
        \Prob{\left|\suvT - \tilde{s}^2_{uv}(i)\right| \geq \tfrac{\vslack}{2} ~\left|~ v \in \rowbaseT \right.}
				&= \Prob{\left|\suvT - \tilde{s}^2_{uv}(i)\right| \geq \tfrac{\vslack}{2} ~\left|~ |\ovuvT| \in [\beta_l, \beta_h]\right.} \\
				&\leq 2 \exp \left(\frac{- \vslack^2}{128B_0^4}  \Delta \right).
	\end{align*}
Combining the two bounds on $\left|\suvT - \tilde{s}^2_{uv}(i)\right|$ and $\left|\tilde{s}^2_{uv}(i) - \bE \tilde{s}^2_{uv}(i) \right|$ leads to a bound on the probability that $\left|\suvT - \bE \tilde{s}^2_{uv}(i) \right| \geq \vslack$.
	
Lastly, we bound the difference between $\bE\tilde{s}^2_{uv}(i)$ and $\siguvT^2 + 2\gamma^2$. By definition, we can write $\tilde{s}^2_{uv}(i)$, conditioned on $\vvec{x}^{\pi}_1(\vvec{u})=a$ and $\vvec{x}^{\pi}_1(\vvec{v})=b$,  according to
\begin{align*}
\tilde{s}^2_{uv}(i) = \frac{1}{2 n'(n'-1)} \sum_{j, h \in \cN_i \times \cN_i} \left( X_j - X_h \right)^2,
\end{align*}
where we define the variables 
\[X_j = Z(u,j) - Z(v,j) = f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j})\]
for all $j \in [n]$. Since the noise terms are i.i.d, and since $\vvec{x}^{\pi}_2(\vvec{j})$ are identically distributed for all $j \in \cN_i$, $\{X_j\}_{j \in \cN_i}$ are also identically distributed. 
When random variables $X_j$ and $X_h$ are identically distributed,
    \begin{align}
        \Exp{(X_j - X_h)^2} &= \Exp{X_j^2 - 2X_j X_h + X_h^2} \nonumber\\
        		&= 2 \Exp{X_j^2} - 2 \Exp{X_j X_h} \nonumber\\
		&= 2 \Var[X_j] - 2 \Cov[X_j, X_h]. \label{eq:exp_sqdiff_id}
    \end{align}
If $h = j$, then $\Cov[X_j, X_h] = \Var[X_j]$. Therefore, by substitution and using the fact that $\{X_j\}_{j \in \cN_i}$ are identically distributed, it follows that 
\begin{align*}
&\E\left[\left.  \tilde{s}^2_{uv}(i) \right| \vvec{x}^{\pi}_1(\vvec{u})=a, \vvec{x}^{\pi}_1(\vvec{v})=b \right] \\
&= \frac{1}{n'(n'-1)} \sum_{j \in \cN_i }\sum_{h \neq j, h \in \cN_i} \left( \Var[X_j]- \Cov[X_j, X_h] \right) \\
&= \Var[X_j] - \frac{1}{n'(n'-1)} \sum_{j \in \cN_i }\sum_{h \neq j, h \in \cN_i} \Cov[X_j, X_h].
\end{align*}
First we can show that because the noise terms are independent, and by definition of $\sigma_{ab}^2$, the variance is equal to
\begin{align*}
\Var[X_j] &= \Var[ f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j})] \\
 &= \Var[ f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right)] + \Var[\eta_{uv}(\vvec{j})]  \\
&= \sigma_{ab}^2 + 2 \gamma^2.
\end{align*}
Next we bound the contribution from the covariance terms. By definition, 
\begin{align*}
\Cov(X_j, X_h) & = \Cov\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right) + \eta_{uv}(\vvec{j}), f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right)+ \eta_{uv}(\vvec{h}) \right)\\
	&= \Cov\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right), f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right) \right) + \Cov\left(\eta_{uv}(\vvec{j}), \eta_{uv}(\vvec{h}) \right).
\end{align*}
Since the noise terms are independent across entries, $\Cov\left(\eta_{uv}(\vvec{j}), \eta_{uv}(\vvec{h}) \right) = 0$ if $j \neq h$. If the Hamming distance between $\vvec{j}$ and $\vvec{h}$ is $t_2$, it means that the entry corresponding to $j$ and $h$ in the original tensor do not share any coordinates, and therefore their associated latent variables $\vvec{x}^{\pi}_2(\vvec{j})$ and $\vvec{x}^{\pi}_2(\vvec{h})$ are independent, such that $ Cov\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right), f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right) \right)$ is equal to zero. For each $j$, there can exist at most $\sum_{q \in \cI_2} \frac{n'}{n_q-1} $ indices $h \in \cN_i$ (including $j$ itself) for which $d_H(\vvec{j},\vvec{h}) < t_2$, where $d_H(\vvec{j}, \vvec{h}) = |\{l : j_l \neq h_l\}|$ denotes the Hamming distance between $\vvec{j}$ and $\vvec{h}$. Furthermore, we know that the absolute value of the covariance of two identically distributed random variables is always less than the variance. We assume without loss of generality that $n_q \geq 2$, otherwise $\cN_i$ would be an empty set. It follows that 
\begin{align*}
& \left| \frac{1}{n'(n'-1)} \sum_{j \in \cN_i }\sum_{h \neq j, h \in \cN_i} \Cov(X_j, X_h)  \right| \\
&= \left| \frac{1}{n'(n'-1)} \sum_{j \in \cN_i }\sum_{h: h \neq j, \atop d_H(\vvec{j}, \vvec{h}) < t_2} \Cov\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right), f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{h})\right) \right) \right| \\
&\leq \frac{1}{n'(n'-1)} \sum_{j \in \cN_i }\sum_{h: h \neq j, \atop d_H(\vvec{j}, \vvec{h}) < t_2} \Var\left(f_{ab}\left(\vvec{x}^{\pi}_2(\vvec{j})\right)\right) \\
&\leq \frac{\sigma_{ab}^2 }{n'-1} \left(\sum_{q \in \cI_2} \left(\frac{n'}{n_q-1} - 1\right)\right)   \\
%&\leq \frac{\sigma_{ab}^2 }{n-1} \left(\sum_{q \in \cI_2} \left(\frac{n - n_q}{n_q}\right)\right)\\
&\leq \frac{\sigma_{ab}^2 }{n'-1} \left(\sum_{q \in \cI_2} \left(\frac{n' - 1}{n_q- 1}\right)\right)	\quad\because n_q \geq 2, \forall q \in \cI_2\\
&= \sigma_{ab}^2 \left(\sum_{q \in \cI_2} \frac{1}{n_q - 1}\right)
\end{align*}
Therefore, it follows that 
\begin{align*}
(1 - \theta) \siguvT^2 + 2\gamma^2 \leq \bE\tilde{s}^2_{uv}(i) \leq (1 + \theta) \siguvT^2 + 2\gamma^2 ,
\end{align*}
where $\theta = \sum_{q \in \cI_2} \frac{1}{n_q - 1} $, which converges to $0$ as $n_q \to \infty$ for all $q \in \cI_2$.

\end{proof}


%%% Lemma: Tensor Near Neighbors
\bigskip

\subsubsection{Sufficiently Many Good Neighbors}

\begin{proof}[Proof of Lemma \ref{lem:regularity_tensor}]
According to the Bayes' rule, the conditional probability of interest can be written as
\begin{align*}
    &\Prob{\left. \left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} > \zeta ~\right|~  |\rowbaseT| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] }\\
    &\qquad = \frac{\Prob{ \left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} > \zeta ~~\bigcap~~  |\rowbaseT| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] }}{\Prob{|\rowbaseT| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] }}\\
    &\qquad \leq 2 \Prob{ \left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} > \zeta },
\end{align*}
assuming that $ \Prob{|\rowbaseT| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] } \geq \frac{1}{2}$, which is true when $m$ and $n$ are sufficiently large from Lemma \ref{lem:overlap_tensor}. 

We can observe that this probability can be represented equivalently as
\begin{align*}
    \Prob{ \left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} > \zeta } &= \Prob{ \sum_{v \in \rowbaseT} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k}\\
    	&= \Prob{ \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k}.
\end{align*}
For any $N$, define event $Q := \left\{ \sum_{v } \Ind\left\{\siguvT^2 \leq \zeta \right\} < N \right\}$. Therefore we can condition on event $Q$ to show that
\begin{align*}
    &\Prob{ \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k}\\
    &\qquad = \Prob{ \left. \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k \right|Q} \Prob{Q}+\\
    &\qquad\qquad + \Prob{ \left. \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k \right|Q^c} \Prob{Q^c}\\
    &\qquad \leq  \Prob{Q} + \Prob{ \left. \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k \right|Q^c}.
\end{align*}

First we provide a bound for $\Prob{Q}$. For any $a,b \in \cX^{\pi}_1$, and random variable $\bx_2 \in \cX^{\pi}_2$, by the $L$-Lipschitz property of function $f$,
\begin{align}
\sigma_{ab}^2 &=\Var_{\bx_2}[f(a,\bx_2) - f(b,\bx_2)] \nonumber\\
&\leq \E_{\bx_2}[(f(a,\bx_2) - f(b,\bx_2))^2]  \nonumber \\
&\leq L^2 d_{\cX^{\pi}_1}(a,b)^2, \label{eq:sigmaT_Lipschitz_bd}
\end{align}
where we recall that the metric $d_{\cX^{\pi}_1}$ is defined as the maximum over the distance in each of the $t_1$ dimensions. Therefore, 
\[d_{\cX_{\pi(q)}}(x_{\pi(q)}(u_q), x_{\pi( q)}(v_q))  \leq \zeta^{1/2}L^{-1} \text{ for all } q \in [t_1]\]
implies that  $d_{\cX^{\pi}_1}(\vvec{x}^{\pi}_1(\vvec{u}),\vvec{x}^{\pi}_1(\vvec{v}))$ is less than $\zeta^{1/2} L^{-1}$, which implies $\siguvT^2 \leq \zeta$ by substituting into \eqref{eq:sigmaT_Lipschitz_bd}.
%
For any $t_1$-sequence of positive integers $(N_1, N_2, \dots, N_{t_1})$ such that $\prod_{q\in [t_1]} N_q \geq N$, 
\begin{align*}
	&\bigcap_{q \in [t_1]} \left\{ \sum_{l \in [n_{\pi(q)}]} \Ind\left\{  d_{\cX_{\pi(q)}}\left( x_{\pi(q)}(u_q), x_{\pi(q)}(l)\right) \leq \zeta^{1/2}L^{-1} \right\} \geq N_q \right\}\\
	&\qquad  \implies \left\{\sum_{v } \Ind\left\{\siguvT^2 \leq \zeta \right\} \geq N \right\}.
\end{align*}
Therefore, we have the following inequality from applying the union bound:
\begin{align*}
	\Prob{Q} &= \Prob{\sum_{v } \Ind\left\{\siguvT^2 \leq \zeta \right\} < N}\\
		&\leq \sum_{q \in [t_1]} \Prob{ \sum_{l \in [n_{\pi(q)}]} \Ind\left\{ d_{\cX_{\pi(q)}}\left( \bx_{\pi(q)}(u_q), \bx_{\pi(q)}(l) \right) \leq \zeta^{1/2} L^{-1} \right\} < N_q }.
\end{align*}
Because $\{\bx_{\pi(q)}(l)\}_{l \in [n_{\pi(q)}]}$ are drawn i.i.d. from $\cX_{\pi(q)}$, the indicator variables are i.i.d. Bernoulli random variables whose success parameter is at least $\phi_{\pi(q)} \left(\zeta^{1/2}L^{-1} \right)$ by definition of the underestimator function $\phi_{\pi(q)}$. Therefore, by Chernoff's bound, it follows that 
\begin{align}
    &\Prob{ \sum_{l \in [n_{\pi(q)}]} \Ind\left\{ d_{\cX_{\pi(q)}}\left( \bx_{\pi(q)}(u_q), \bx_{\pi(q)}(l) \right) \leq \zeta^{1/2} L^{-1} \right\} < N_q }\nonumber\\
    &\qquad \leq \Prob{\text{Binomial}\left(n_{\pi(q)}, \phi_{\pi(q)} \left(\zeta^{1/2} L^{-1} \right)\right) \leq N_q }\nonumber\\
    &\qquad \leq \exp \left( - \frac{(\mu_q - N_q )^2}{2 \mu_q} \right), \label{eqn:first_term}
\end{align}
for $N_q < \mu_q$ where $\mu_q := n_{\pi(q)} \phi_{\pi(q)} \left(\zeta^{1/2} L^{-1}\right)$. Given parameter $N$ and information on the underestimator functions $\{\phi_{\pi(q)}\}_{q \in [t_1]}$, we can optimize the choice of $\{N_q\}_{q \in [t_1]}$ by balancing $\frac{(\mu_q - N_q )^2}{2 \mu_q}$. %, but we will not discuss about that here.

Next we provide a bound for $\Prob{ \left. \sum_{v \in \rowbaseT } \Ind\left\{\siguvT^2 \leq \zeta \right\} < k \right|Q^c}$. 
The event $\left\{ v \in \rowbaseT \right\}$ is solely determined by the locations of the sampled datapoints represented in index set $\cD$, thus it is completely independent from the latent variables and the entry values. Thus it is independent from  $\left\{\siguvT^2 \leq \zeta \right\}$ as long as $v \neq u$. Therefore, the probability of interest
\begin{align*}
    &\Prob{ \left. \sum_{v } \Ind\left\{ v \in \rowbaseT \right\} \Ind\left\{\siguvT^2 \leq \zeta \right\} < k \right|Q^c}\\
    &\qquad=  \Prob{ \left. \sum_{v:  \siguvT^2 \leq \zeta} \Ind\left\{ v \in \rowbaseT \right\} < k \right|Q^c} \\
 &\qquad\leq \Prob{ \sum_{v=1, v\neq u}^{N}  \Ind\left\{ v \in \rowbaseT \right\} < k} \\
&\qquad= \Prob{ \big|\rowbaseT \cap ([N] \setminus \{u\})\big| < k} ,
\end{align*}
where we used the fact that $Q^c$ implies by definition that the set of rows $v$ such that $\Ind\left\{\siguvT^2 \leq \zeta \right\}$ is larger than $N$ and the probability of event of interest is monotonically decreasing in the number of such $v$s.
Recall that Lemma \ref{lem:overlap_tensor} proved concentration of $|\rowbaseT|$. By the same proof as Lemma \ref{lem:overlap_tensor}, replacing $m$ with $N$, it follows that for $k < Np$,
\begin{align}
    &\Prob{ |\rowbaseT \cap ([N] \setminus \{u\})| < k} 
		\leq \exp \left( - \frac{((N-1)p - k )^2}{2 (N-1)p} \right)  \label{eqn:second_term_a}\\
		&\qquad \qquad+  (N-1)\exp \left( - \frac{(n'p^2 - \beta_l )^2}{2 n'p^2} \right) +  (N-1)\exp \left( - \frac{(\beta_h - n'p^2 )^2}{3 n'p^2} \right).
\end{align}

We choose $N_q = 2^{-1/t_1} \mu_q  = 2^{-1/t_1} n_{\pi(q)} \phi_{\pi(q)}\left(\zeta^{1/2} L^{-1}\right)$, such that it also follows that
\[N = \prod_{q \in [t_1]} N_q = \frac{1}{2} \prod_{q \in [t_1]} n_{\pi(q)} \phi_{\pi(q)}\left(\zeta^{1/2} L^{-1}\right) = \frac{1}{2} m \phi^{\pi}_1\left(\zeta^{1/2} L^{-1}\right).\]
Therefore, given the constraint on $k$ such that $k \leq \frac{1}{8}mp \phi^{\pi}_1\left(\zeta^{1/2}L^{-1} \right)$, we can verify that $k < Np$. 

With this choice of $N_q$, the expression in \eqref{eqn:first_term} is upper bounded by
$$    \exp \left( - \frac{(\mu_q - N_q )^2}{2 \mu_q} \right) = \exp \left( - \frac{(1 - 2^{-1/t_1} )^2}{2} \mu_q \right).    $$
Since we may assume $N \geq 2$ (because $N=1$ gives a meaningless event $E$ and we are considering the large tensor limit as $n_q \to \infty, \forall q$), it holds that  $N-1 \geq \frac{N}{2}$. Therefore, the first expression in \eqref{eqn:second_term_a} is upper bounded by
$$     \exp \left( - \frac{((N-1)p - k )^2}{2 (N-1)p} \right) \leq \exp \left( -\frac{\left( \frac{1}{4}Np\right)^2}{2Np} \right) = \exp \left( -\frac{ Np }{32} \right) \leq \exp\left(-\frac{k}{8}\right).    $$
Using $N \leq \prod_{q \in \cI_1} n_q = m$ in \eqref{eqn:second_term_a} and combining everything together, we obtain the desired result.
\end{proof}



%%% Lemma: Tensor Chebyshev
\subsubsection{Tail Probability Bound Conditioned on Good Events}

\begin{proof}[Proof of Lemma \ref{lem:estimate_tensor}]
We redefine $S^k$ so that it denotes the set of the $k$ best row indices $v$ in $\rowbaseT$ which have minimum sample variance $\suvT$. We define $Err^k(u,i) := A(u,i) - \hat{A}^k(u,i)$ and are interested in its probabilistic tail bound. By the same argument as in the proof of Lemma \ref{lem:estimate}, its absolute value can be bounded as below
\begin{align*}
&\left| A(u,i) - \hat{A}^k(u,i) \right| \\
& \qquad	\leq  \left| \frac{1}{|S^k|} \sum_{v \in S^k} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuvT \right) \right| \\
& \qquad \qquad + \left| \frac{1}{|S^k|} \sum_{v \in S^k}  \muvT - \muuvT\right|.
\end{align*}

Recall that we denote $E' := \Ea' \cap \Eb' \cap \Ec' \cap \Ed'$. Following the same lines of argument as in the proof of Lemma \ref{lem:estimate}, we can show that
\begin{align*}
&\Prob{\left| A(u, i) - \hat{A}^k(u,i) \right| > \eps ~|~ E'}\\
&\qquad\leq \Prob{\left.\left| \frac{1}{|S^k|} \sum_{v \in S^k} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuvT \right) \right| > \eps - \mslack ~\right|~ E'}\\
&= \int_{ \vvec{y} \in (\cX^{\pi}_1)^m} \sum_{\cS_0 \subset [n]: |\cS_0| = k} \Prob{\left.\left| \text{``expr''} \right| > \eps - \mslack ~\right|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'} \nonumber \\
& \qquad \qquad \qquad \qquad \qquad \qquad \Prob{ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0 ~|~ E'} d\vvec{y}, 
\end{align*}
where ``expr'' denotes the expression $ \frac{1}{|S^k|} \sum_{v \in S^k} \left( A(u,i) - A(v,i) - \eta(v,i) - \muuvT \right)$.

Recall that we modified the tensor algorithm such that the overlap $\ovuvT$, sample variance $\suvT$, row base $\rowbaseT$, and thus the set $S^k$ are computed from the data matrix after removing all columns $j$ which share any of the original tensor coordinates, i.e. $j_k = i_k$ for any $k \in [t_2]$. Therefore, the event $E'$ and the set $S^k$ are independent from the $i$-th column latent feature $\vvec{x}_2(\vvec{i})$ and the noise terms $\eta(v,i)$ for any $v \in [m]$. Let $\vvec{\bx}_2$ be a random variable sampled independently from the product space $\cX^{\pi}_2$ with the associated product measure. Then we can verify that
\begin{align*}
&\E[A(u,i) - A(v,i) - \eta(v,i) - \muuvT ~|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'] \\
&= \E[f(\vvec{x}^{\pi}_1(\vvec{u}),\vvec{x}^{\pi}_2(\vvec{i})) - f(\vvec{x}^{\pi}_1(\vvec{v}),\vvec{x}^{\pi}_2(\vvec{i})) - \eta(v,i) ~|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E']  - \mu_{y_u y_v} \\
&= \E[f(y_u,\vvec{\bx}_2) - f(y_v,\vvec{\bx}_2) - \eta(v,i) ~|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E']  - \mu_{y_u y_v} \\
&= 0. 
\end{align*}

Next we apply Chebyshev's inequality and Cauchy-Schwarz inequality along with the fact that $\eta(v,i)$ is independent from $E'$ because the events in $E'$ do not depend on the data observed from column $i$.
\begin{align*}
&\Prob{\left.\left| \text{``expr''} \right| > \eps - \mslack ~\right|~ \left(\vvec{x}^{\pi}_1(\vvec{v}))\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E} \\
&\qquad\leq \frac{\Var\left[\left.\frac{1}{|S^k|} \sum_{v \in S^k} \left( A(u,i) - A(v,i) - \eta(v,i)\right) ~\right|~  \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E' \right]}{(\eps - \mslack)^2} \\
&\qquad\leq \frac{1}{(\eps - \mslack)^2} \left( \left(\frac{1}{k} \sum_{v \in \cS_0} \sqrt{\Var\left[A(u,i) - A(v,i)  \big|  \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right]}\right)^2 + \frac{\gamma^2}{k} \right).
\end{align*}


Next we will bound $\Var\left[A(u,i) - A(v,i)  ~\big|~  \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right]$ for any $v \in \cS_0$. Therefore,
\begin{align*}
&\Var\left[A(u,i) - A(v,i)  ~\big|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right] \\
&= \Var\left[f(y_u,\vvec{x}_2(\vvec{i})) - f(y_v,\vvec{x}_2(\vvec{i}))  ~\big|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right] \\
&= \Var\left[f(y_u,\vvec{\bx}_2) - f(y_v,\vvec{\bx}_2)  ~\big|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right] \\
&= \sigma_{y_u y_v}^2.
\end{align*}

Let $\tilde{\cV}$ denote the subset of rows $v \in \rowbaseT$ such that $\siguvT^2 \leq \zeta$. Conditioned on $\Ed$, the size of set $\tilde{\cV}$ must be at least $k$. Conditioned on $\Ec'$, for every $v \in \tilde{\cV} \subset \rowbaseT$, 
\[\suvT \leq \left(1 + \theta\right)\siguvT^2 + 2 \gamma^2+ \vslack \leq \left(1 + \theta\right)\zeta + 2 \gamma^2 + \vslack. \]
%
Therefore, it follows by definition of $S^k$ as the set of $k$ rows with minimum sample variance, that for all $v \in S^k$, $\suvT \leq \left(1 + \theta\right)\zeta + \vslack + 2 \gamma^2$. Again due to event $\Ec'$, this implies that for all $v \in S^k$, $\siguvT^2 \leq \frac{(1+\theta) \zeta + 2 \vslack}{1-\theta}$ because $(1-\theta)\siguvT^2 - \vslack \leq  \suvT - 2 \gamma^2 $.  
%
Therefore for all  $v \in S^k$, 
\begin{align*}
\Var\left[A(u,i) - A(v,i)  ~\big|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'  \right] \leq \frac{(1+\theta) \zeta + 2 \vslack}{1-\theta}.
\end{align*}

Finally we can show that
\begin{align*}
&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps ~|~ \left(\vvec{x}^{\pi}_1(\vvec{v})\right)_{v \in [m]} = \vvec{y}, S^k = \cS_0, E'} \\
&\qquad\leq \frac{1}{(\eps - \mslack)^2} \left(\frac{(1+\theta) \zeta + 2 \vslack}{1-\theta} + \frac{\gamma^2}{k} \right).
\end{align*}

Since this bound does not depend on the choice of $\vvec{y}$ and $\cS_0$, when we integrate over all choices of $\vvec{y}$ and $\cS_0$, we obtain the same bound.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:bad_event_bound}]
We restate the following conditioning events (defined in Lemma \ref{lem:estimate_tensor}) for readability:
\begin{align*}
E' &:= \Ea' \cap \Eb' \cap \Ec' \cap \Ed', \\
\Ea' &:= \left\{\left|\rowbaseT\right| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right]\right\}, \\
\Eb' &:= \left\{\left| \muv - \muuvT\right| \leq \mslack, ~\forall~ v \in \rowbaseT \right\}, \\
\Ec' &:= \left\{ \suvT \in \left[(1-\theta)\siguvT^2 -\vslack , (1+\theta)\siguvT^2  + \vslack \right], ~\forall~ v \in \rowbaseT \right\}, \\
\Ed' &:= \left\{\left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} \leq \zeta \right\},
\end{align*}

First of all, note that (see the proof of Theorem \ref{thm:main_tail} for more detail)
	\begin{align*}
			&\Prob{E'^c}	\leq \Prob{\Ea'^c} + \Prob{ \Eb'^c  | \Ea'} + \Prob{\Ec'^c | \Ea'} + \Prob{\Ed'^c | \Ea' }.
	\end{align*}
	
	Using Lemma \ref{lem:overlap_tensor}, we have
\begin{align*}
		\Prob{\Ea'^c}	&= \Prob{|\rowbaseT| \not\in \left[ \frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p \right]}\\
		&\leq (m-1) \exp \left( - \frac{\left(n'p^2-\beta_l\right)^2}{2n'p^2} \right) + (m-1) \exp \left( - \frac{\left(\beta_h - n'p^2\right)^2}{3n'p^2} \right)\\
	    	&\qquad\qquad + 2 \exp \left( - \frac{(m-1)p}{12} \right).
\end{align*}
Similarly, by using Lemma \ref{lem:mean_tensor} with union bound,
\begin{align*}
		\Prob{\Eb'^c | \Ea'} &= \Prob{\bigcup_{v \in \rowbaseT} \left\{ |\muuvT - \muv| > \mslack \right\}}\\
&\leq 3(m-1)p  \exp\left(\frac{-\mslack^2}{8L^2D^2 \theta + \frac{16B_e^2}{n'}}\right)\\
	&\qquad + 3(m-1)p\exp\left(\frac{- \mslack^2}{32(LD+2B_e)^2}\Delta\right),
\end{align*}
where we recall that $\Delta = \min \left\{ \frac{n'^2\beta_l}{\left(n' + \beta_l^2\right)^2}, \frac{n'^2\beta_h}{\left(n' + \beta_h^2\right)^2} \right\}$ and $\theta = \sum_{q \in \cI_2} \frac{1}{n_q-1}$ is a quantity which depends only on the shape of the given tensor instance, and it vanishes to $0$ as $n_q \to \infty, \forall q \in \cI_2$.

By using Lemma \ref{lem:variance_tensor} with union bound again,
\begin{align*}
	\Prob{\Ec'^c | \Ea'} &= \Prob{\bigcup_{v \in \rowbase} \left\{ \suvT \in \left[(1-\theta)\siguvT^2 -\vslack , (1+\theta)\siguvT^2  + \vslack \right] \right\}}\\
&\leq 3(m-1)p\exp\left(\frac{-\vslack^2}{32L^2D^2\left( 3LD + 4 B_e\right)^2\theta + \frac{64B_e^2\left( 2LD + 5 B_e\right)^2}{n'}}\right)\\
		&\qquad + 3(m-1)p\exp\left(\frac{- \vslack^2}{128(LD+2B_e)^4} \Delta\right).
\end{align*}

	
By Lemma \ref{lem:regularity_tensor} with $\mu_q := n_q \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right)$ and $\phi_q(r) := \ess \inf_{x' \in \cX_q} \bP_{\cX_q} \left(d_{\cX_q}(\bx, x') \leq r\right)$ as previously defined,
\begin{align*}
	\Prob{\Ed'^c | \Ea'} &\leq \sum_{q \in \cI_1} \exp \left( - \frac{(1 - 2^{-1/t_1} )^2}{2} \mu_q \right) + \exp\left(-\frac{k}{8}\right)\\
				&\qquad + (m-1)\exp \left( - \frac{(n'p^2 - \beta_l )^2}{2 n'p^2} \right) +  (m-1)\exp \left( - \frac{(\beta_h - n'p^2 )^2}{3 n'p^2} \right).
\end{align*}

Putting everything together, we obtain the following bound
\begin{align}
\Prob{E'^c}	&\leq	2(m-1) \exp \left( - \frac{\left(n'p^2-\beta_l\right)^2}{2n'p^2} \right) + 2(m-1) \exp \left( - \frac{\left(\beta_h - n'p^2\right)^2}{3n'p^2} \right)	\label{eqn:term1}\\
	&\qquad + 2 \exp \left( - \frac{(m-1)p}{12} \right)	\label{eqn:term2}\\
	&\qquad + 3(m-1)p  \exp\left(\frac{-\mslack^2}{8L^2D^2 \theta + \frac{16B_e^2}{n'}}\right)		\label{eqn:term3}\\
	&\qquad + 3(m-1)p\exp\left(\frac{- \mslack^2}{32(LD+2B_e)^2}\Delta\right)		\label{eqn:term4}\\
	&\qquad + 3(m-1)p\exp\left(\frac{-\vslack^2}{32L^2D^2\left( 3LD + 4 B_e\right)^2\theta + \frac{64B_e^2\left( 2LD + 5 B_e\right)^2}{n'}}\right)		\label{eqn:term5}\\
	&\qquad + 3(m-1)p\exp\left(\frac{- \vslack^2}{128(LD+2B_e)^4} \Delta\right)	\label{eqn:term6}\\
	&\qquad + \sum_{q \in \cI_1} \exp \left( - \frac{(1 - 2^{-1/t_1} )^2}{2} \mu_q \right) + \exp\left(-\frac{k}{8}\right)	\label{eqn:term7}.
\end{align}

Note that $\zeta, \mslack, \vslack$ are parameters which are introduced purely for the purpose of analysis. Requiring all exponential terms decay to $0$ as $m, n \to \infty$ restricts the range of values $\zeta, \mslack, \vslack$ can take. Define $q^* := \arg \min_{q \in \cI_1} n_q$. Then we choose $\mslack = \vslack = \max\left\{ (n_{q^*}-1)^{-1/3} , \left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}$. Also, we enforce $\zeta$ satisfies $\phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right)\geq c_q n_q^{-\frac{\log mp}{2 \log m}}$ so that $\mu_q \geq c_q n_q^{\delta/2}$ even for the worst choice of $p$, and $mp \phi^{\pi}_1\left( \sqrt{\frac{\zeta}{L^2}} \right) \geq \left(\prod_{q \in \cI_1} c_q\right) \sqrt{mp}$ as described in the theorem statement. 

Additionally, we require $\beta_l, \beta_h \to \infty$ as $m, n \to \infty$ while $n'p^2 - \beta_l, \beta_h - n'p^2 \to \infty$ as well. We will assume $\beta_h \leq n'^{2/3- \delta}$ for convenience in analysis. Lastly, we want $k \to \infty$, which is possible while satisfying the constraint $k \leq \frac{1}{8}mp \phi^{\pi}_1\left( \sqrt{\frac{\zeta}{L^2}} \right) = \frac{\prod_{q \in \cI_1} c_q}{8} \sqrt{mp}$, which originated from Lemma \ref{lem:estimate_tensor}. Let's suppose that we take $k = \frac{\prod_{q \in \cI_1} c_q}{8} \sqrt{mp}$ by default.
We will show these are sufficient conditions for the convergence of exponential error terms.

%Lastly, we can have $k \to \infty$ by taking $k =\frac{1}{8}mp \phi^{\pi}\left( \sqrt{\frac{\zeta}{L^2}} \right) = \frac{p}{8} \prod_{q \in \cI_1} n_q \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right) \geq \frac{\prod_{q \in \cI_1} c_q}{8} m^{\delta} \to \infty$. 

Given a sequence of problems of size $(m,n)$, suppose that $p = \omega(m^{-1})$ and $p = \omega(n'^{-1/2})$. Then $mp, n'p^2 \to \infty$ as $m, n \to \infty$, since $n' = \Theta(n)$. We may assume without loss of generality that $m$ and $n'$ are large enough such that $mp, n'p^2 \geq 2$. As $n_q \to \infty, \forall q$, we can observe that $\mslack, \vslack \to 0$. In addition, we have $\mslack \leq 1$, $\vslack \leq 1$, since we assumed $\beta_h \leq n'^{2/3- \delta}$. 

Now we will clean up the exponential error terms in Eq. \eqref{eqn:term1}-\eqref{eqn:term7} to obtain simpler yet more enlightening forms.

Eq. \eqref{eqn:term1}: 
Since $\beta_l \leq c_l n'p^2$, we have $(n'p^2 - \beta_l)^2 \geq \left[(1 - c_l) n'p^2 \right]^2$. Similarly, $\beta_h \geq c_h n'p^2$ implies that $(\beta_h - n'p^2)^2 \geq \left[(c_h - 1) n'p^2 \right]^2$. Therefore, the terms in Eq. \eqref{eqn:term1} are upper bounded by
$$    2(m-1) \exp \left( - \frac{\left(1 - c_l\right)^2}{2} n'p^2 \right) + 2(m-1) \exp \left( - \frac{\left(c_h - 1\right)^2}{3} n'p^2 \right).    $$

Eq. \eqref{eqn:term2}:
The term in Eq. \eqref{eqn:term2} is upper bounded by $2 \exp\left(-\frac{1}{24}mp \right)$, using the fact that $m-1 \geq \frac{m}{2}$ for $m \geq 2$, which is implied by our assumption that $mp \geq 2$. 

Eq. \eqref{eqn:term3} and \eqref{eqn:term5}:
Due to our choice of $\mslack$ (and $\vslack$), we have $\mslack = \vslack \geq  (n_{q^*} - 1)^{-1/3}$ where $q^* = \arg \max_{q \in \cI_1} \left((n_q - 1)^{-1/3} \right)$. For any constants $X, Y > 0$, because $(n_q-1) ^{-1} \leq (n_{q^*}-1)^{-1}, \forall q \in \cI_2$, and $n' = \prod_{q \in \cI_2} (n_q - 1) \geq n_{q^*} - 1$, it follows that
$$    \frac{\mslack^2}{X \sum_{q \in \cI_2} \frac{1}{n_q - 1} + Y \frac{1}{n'}} \geq \frac{(n_{q^*}-1)^{-2/3}}{\left(X t_2 + Y \right) (n_{q^*}-1)^{-1} } = \frac{(n_{q^*}-1)^{1/3}}{X t_2 + Y }.    $$

Eq. \eqref{eqn:term4} and \eqref{eqn:term6}:
Again from our choice of $\mslack$ (and $\vslack$), the following inequality is true: $\mslack \geq \max\left\{\left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}$. Meanwhile, $\Delta := \min \left\{ \Delta_l, \Delta_h \right\}$ where $\Delta_l := \frac{n'^2 \beta_l}{(n' + \beta_l^2)^2}$ and $\Delta_h := \frac{n'^2 \beta_h}{(n' + \beta_h^2)^2}$. Therefore, $\mslack^2 \Delta \geq \min \left\{  \left(\frac{n'^2}{\beta_h^3} \right)^{-2/3} \Delta_h, \beta_l^{-2/3} \Delta_l \right\}$.

From the assumption $\beta_h \geq \sqrt{n'}$, 
\begin{align*}
    \left(\frac{n'^2}{\beta_h^3} \right)^{-2/3} \Delta_h &= \left(\frac{n'^2}{\beta_h^3} \right)^{-2/3} \frac{n'^2 \beta_h}{\left(n' + \beta_h^2\right)^2}\\
    	&\geq \left(\frac{n'^2}{\beta_h^3} \right)^{-2/3} \frac{n'^2 \beta_h}{\left(2 \beta_h^2\right)^2}\\
	&= \frac{n'^{2/3}}{4\beta_h}.
\end{align*}
Because we assumed $\beta_h \leq n'^{2/3 - \delta}$, this value diverges no slower than $n'^{\delta}/4$ as $n' = \Theta(n) \to \infty$.

Similarly, from the assumption $\beta_l \leq \sqrt{n'}$,
\begin{align*}
    \beta_l^{-2/3} \Delta_l &= \beta_l^{-2/3} \frac{n'^2 \beta_l}{\left(n' + \beta_l^2\right)^2}\\
    	& \geq \beta_l^{-2/3} \frac{n'^2 \beta_l}{\left(2n'\right)^2}\\
	&= \frac{\beta_l^{1/3}}{4}.
\end{align*} 

Eq. \eqref{eqn:term7}:
$\mu_q = n_q \phi_q\left(\sqrt{\frac{\zeta}{L^2}}\right)\geq c_q n_q^{1 -\frac{\log mp}{2 \log m}} \geq c_q n_q^{1 -\frac{\log m}{2 \log m}} = c_q n_q^{1/2}$ because $p \leq 1$. We will leave $k$ as a free parameter, but our default choice for $k$, which is $\frac{\prod_{q \in \cI_1} c_q}{8} \sqrt{mp}$, diverges as $m \to \infty$.

Consequently, we have
\begin{align*}
\Prob{E'^c} &\leq 4(m-1) \exp \left( -c_1 n'p^2 \right) + 2 \exp \left( - \frac{1}{24} mp \right)\\
&\qquad	+ 6 (m-1)p \exp \left( -c_2 (n_{q^*} - 1)^{1/3}\right) + 6(m-1)p \exp \left( -c_3 \min \left\{ \frac{n'^{2/3}}{4\beta_h}, \frac{\beta_l^{1/3}}{4} \right\} \right)\\
&\qquad	+ t_1 \exp \left( -c_4 n_{q^*}^{1/2}\right) + \exp \left( -\frac{k}{8}\right),
\end{align*}
where 
\begin{align*}
q^* &:= \arg \min_{q \in \cI_1} n_q, \\
c_1 &:= \min \left\{ \frac{(1-c_l)^2}{2}, \frac{(c_h-1)^2}{3} \right\}, \\
c_2 &:= \min \left\{ \frac{1}{8L^2D^2 t_2 + 16B_e^2}, \frac{1}{32L^2D^2(3LD + 4B_e)^2 t_2 + 64B_e^2(2LD + 5B_e)^2}  \right\}, \\
c_3 &:= \min \left\{ \frac{1}{32(LD + 2B_e)^2}, \frac{1}{128(LD+2B_e)^4} \right\}, \\
c_4 &:= \min_{q \in \cI_q} \left\{ \frac{(1-2^{-1/t_1})^2}{2} c_q \right\}.
\end{align*}
Note that $c_1, c_2, c_3, c_4$ are absolute constants, which may depend only on the geometry of the latent spaces.

\end{proof}



==> contents/tensor_proof/tensor_pf_outline.tex <==

Recall that our tensor completion algorithm followed from flattening the tensor to a matrix and applying our user-user $k$-nearest neighbor method to the resulting matrix. Therefore, the proof follows a similar outline to the proofs of the matrix results. However, it requires a separate (and little more involved) proof since in the flattened matrix obtained from tensor, the row and column latent features are likely to be correlated, not independent from each other. This subtlety requires careful handling of various arguments which we present here.

Recall that in Sections \ref{sec:tensor_model} and \ref{sec:tensor_flatten_model}, we presented the latent variable model for a tensor, and we discussed the procedure for flattening a tensor to a matrix, and the model for the resulting flattened matrix.

\subsection{Tensor Model} We summarize the model and relevant notation for a $t$-order tensor $T_A \in  \Reals^{n_1 \times n_2 \times \dots n_t}$. For each dimension $q \in [t]$, each index $\alpha_q \in [n_q]$ is associated to a latent feature $x_q(\alpha_q)$ drawn i.i.d. from the compact metric space $\cX_q$ according to probability measure $P_{\cX_q}$. The space $\cX_q$ is endowed with metric $d_{\cX_q}$ and has diameter $D_{\cX_q}$. The underestimator function $\phi_q$ is defined in \eqref{eq:phi_tensor_def}. 

An entry of the tensor indexed by $\vvec{\alpha} = (\alpha_1, \dots \alpha_t) \in [n_1] \times \dots \times [n_t]$ is described by the $L$-Lipschitz function $f$ applied to the latent features according to \eqref{eq:tensor_model}. $T_Z  \in  \Reals^{n_1 \times n_2 \times \dots n_t}$ is the noisy tensor derived from $T_A$ by adding independent noise terms $\eta(\vvec{\alpha})$ to each entry $T_A(\vvec{\alpha})$ according to \eqref{eq:tensor_noise_model}. The additive noise terms $\eta(\vvec{\alpha})$ are assumed to be independent, zero mean, bounded between $[-B_e, B_e]$, and have uniform variance equal to $\gamma^2$. $\cD$ denotes the index set of observed entries, such that  $\vvec{\alpha} \in \cD$ with probability $p$ and $\vvec{\alpha} \notin \cD$ with probability $1-p$ for any index $\vvec{\alpha}$ independently of all other entries. 

\subsection{Flattened Matrix} 
There may be many ways to flatten a tensor into a matrix, each corresponding to a specific bi-partition of $[t]$ denoted by $(\cI_1, \cI_2)$ where $\cI_1 = \left\{ \pi(1), \dots, \pi(t_1) \right\}$ and $\cI_2 = \left\{ \pi(t_1 + 1), \dots, \pi(t) \right\}$ for some $1 \leq t_1 \leq t - 1$ and some permutation $\pi: [t] \to [t]$. Recall $t_2 = t - t_1$. Given a partitioning of the dimensions, the rows of the flattened matrix would correspond to taking the cartesian product of all dimensions in $\cI_1$, and the columns of the matrix would correspond to taking the cartesian product of all dimensions in $\cI_2$. If the dimensions of the matrix are denoted by $m \times n$, then $m = \times_{q \in \cI_1} [n_q]$ and $n = \times_{q \in \cI_2} [n_q]$.

A row $u$ in the matrix is associated to a vector of indices $\vvec{u} = (u_1, \dots, u_{t_1}) \in [n_{\pi(1)}] \times \dots \times [n_{\pi(t_1)}]$, and similarly a column $i$ in the matrix is associated to a vector of indices $\vvec{i} = (i_1, \dots, i_{t_2}) \in [n_{\pi(t_1 + 1)}] \times \dots \times [n_{\pi(t)}]$.
The corresponding row and column features are denoted by
\begin{align*}
	\vvec{x}^{\pi}_1 (\vvec{u}) &= \left( x^{\pi}_{1, 1} (u_1), \dots, x^{\pi}_{1, t_1} (u_{t_1}) \right) = \left( x_{\pi(1)} (u_1), \dots, x_{\pi(t_1)} (u_{t_1}) \right),\\
	\vvec{x}^{\pi}_2 (\vvec{i}) &= \left( x^{\pi}_{2, 1} (i_1), \dots, x^{\pi}_{2, t_2} (i_{t_2}) \right) = \left( x_{\pi(t_1 + 1)} (i_1), \dots, x_{\pi(t_1 + t_2)} (i_{t_2}) \right).
\end{align*}
The latent row features belong to space $\cX^{\pi}_1 = \times_{q \in \cI_1} \cX_q$, and the latent column features belong to $\cX^{\pi}_2 = \times_{q \in \cI_2} \cX_q$. We let $\cX^{\pi}_{1,k}$ denote $\cX_{\pi(k)}$ for $k \in [t_1]$, and we let $\cX^{\pi}_{2,k}$ denote $\cX_{\pi(t_1 + k)}$ for $k \in [t_2]$. We define the metric for the product spaces according to the max over the distance in the individual latent space associated to each dimension,
\begin{align}
d_{\cX^{\pi}_1}(\vvec{x}, \vvec{x}') = \max_{q \in [t_1]} (d_{\cX_{\pi(q)}}(x_q, x'_q)) \\
d_{\cX^{\pi}_2}(\vvec{x}, \vvec{x}') = \max_{q \in [t_2]} (d_{\cX_{\pi(t_1 + q)}}(x_q, x'_q)).
\end{align}
Therefore the diameter of $\cX^{\pi}_1$ is $D_{\cX^{\pi}_1} := \max(D_{\cX^{\pi}_{1,1}}, \dots D_{\cX^{\pi}_{1,t_1}})$. The measure associated to the row latent space is the product measure corresponding to $P_{\cX^{\pi}_{1,1}} \dots P_{\cX^{\pi}_{1,t_1}}$, and its underestimator function is denoted by
\[\phi^{\pi}_1(r) := \prod_{q \in \cI_1} \phi_q(r).\]
%\[d_{\cX^{\pi}_1}(x^{\pi}_1(u), x^{\pi}_1(u')) = \max(d_{\cX^{\pi}_{1,1}}(x^{\pi}_{1, 1} (u_1)), \dots , d_{\cX^{\pi}_{1,1}}(x^{\pi}_{1, 1} (u_1)))\]

If the tensors $T_A$ and $T_Z$ are drawn from the tensor latent variable model, then the entries of the associated matrices $A$ and $Z$, obtained by flatting the tensors $T_A$ and $T_Z$, can be described as:
\begin{align}
A(u,i) = f(\vvec{x}^{\pi}_1 (\vvec{u}), 	\vvec{x}^{\pi}_2 (\vvec{i})) \\
Z(u,i) = A(u,i) + \eta(u,i).
\end{align}
This flattened matrix satisfies some of the conditions required in the matrix setting in Section \ref{sec:setup}, namely $f$ is Lipschitz, the latent variables are drawn from a bounded metric space, and the data is observed with additive bounded zero-mean noise. We define
\begin{align}
B_0 \triangleq  L D_{\cX^{\pi}_1} + 2 B_e, \label{eq:def_B0_tensor}
\end{align}
such that for any $u,v \in [m]$ and any $i \in [n]$,
\begin{align*}
\left| Z(u,i) - Z(v,i) \right| 
&= \left| f(\vvec{x}_1(\vvec{u}), \vvec{x}_2(\vvec{i})) + \eta(u,i) - f(\vvec{x}_1(\vvec{v}), \vvec{x}_2(\vvec{i})) - \eta(v,i) \right| \\
&\leq L D_{\cX^{\pi}_1} + 2 B_e =: B_0.
\end{align*}

However the flattened matrix does not satisfy the condition that the row and column latent variables are fully independent. Although the latent variables for each coordinate of each dimension of the tensor are independently sampled, if two rows $\vvec{u}$ and $\vvec{u}'$ in the flattened matrix correspond to tensor indices that coincide, i.e. if $u_{h} = u_{h}'$ for any $h \in [t_1]$, then the corresponding component of the latent variable $x_{1,h}^{\pi}(u_h)$ and $x_{1,h}^{\pi}(u'_h)$ will be correlated, in fact they must be equal. The correlation structure amongst the rows and columns of the flattened matrix is very specific and follows from the partitioning and flattening of the tensor to a matrix. For some column $i$, recall that $\cN_i \subset [n]$ denote the set of columns which do not share a tensor coordinate with $i$, and thus whose latent features are uncorrelated with $\vvec{x}^{\pi}_2(\vvec{i})$, 
\[\cN_i := \{j \in [n] ~s.t.~ j_k \neq i_k \text{ for all } k \in [t_2]\}.\]
The number of remaining columns in the matrix after removing one coordinate from each tesnor dimension is denoted by
\[|\cN_i| = n' := \prod_{q \in \cI_2} (n_q - 1).\]

\subsection{Proof Outline}

The proof follows similar steps to the proof of the matrix results. The algorithm corresponds to first computing the empirical means and variances of the differences between pairs of rows in the flattened matrix. These computed variances are used to choose the $k$-nearest neighbors which are included in the final estimate. The differences we made to the algorithm is that the set $\rowbaseT$ both imposes and upper and lower bound on the overlap between rows. Additionally, since the matrix results from flattening a tensor, the latent variables for rows and columns are correlated according to the original tensor structure. Therefore, we modified the computation of empirical means and variances such that when we are estimating an entry at $(u,i)$, we only consider columns $j$ which do not share any coordinates in the original tensor representation, i.e. $i_k \neq j_k$ for all $k \in [t_2]$. In this way, the computation of $\muvT$, $\suvT$, and $\rowbaseT$ become fully independent from the latent variables associated to $i$ denoted by $\vvec{x}^{\pi}_2(\vvec{i})$.

The key steps of the proof are stated within a few lemmas that mirror the same format as the matrix proof. However, we will need to modify the proof of these corresponding tensor lemmas to account for the fact that the row and column features are no longer drawn independently from the product spaces $\cX^{\pi}_1, \cX^{\pi}_2$. We first prove that the overlaps between pairs of rows is sufficiently large, which is presented in Lemma \ref{lem:overlap_tensor} and is equivalent to the corresponding matrix Lemma \ref{lem:overlap}. Next we prove concentration of the empirical means and variances in Lemmas \ref{lem:mean_tensor} and \ref{lem:variance_tensor}, which correspond to the matrix Lemmas \ref{lem:mean} and \ref{lem:variance}. Then we prove that each row has sufficiently many ``good neighbors'', i.e. other rows whose latent features are close to the target row's latent features. This is presented in Lemma \ref{lem:regularity_tensor}, which corresponds to \ref{lem:regularity}. The proofs of Lemmas \ref{lem:mean_tensor}, \ref{lem:variance_tensor}, and \ref{lem:regularity_tensor} will need to account for the correlations across latent variables.  Finally, conditioned on these above good events, we combine them together to prove a bound on the probability of error in Lemma \ref{lem:estimate_tensor}. 

We first prove that every pair of rows has sufficient, but not too huge overlap with high probability. Specifically, Lemma \ref{lem:overlap_tensor} proves that for any $(u,i)$, the number of the candidate rows, $|\rowbaseT|$, concentrates around $(m-1)p$. This relies on concentration of Binomial random variables via Chernoff's bound, using the fact that every entry is independently observed uniformly at random. The proof is essentially identical to the proof of Lemma \ref{lem:overlap}, and the result upper bounds the probability of the complement of the following good event
\begin{align}
\Ea' := \left\{\left|\rowbaseT\right| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right]\right\}.\label{eq:def_Ea}
\end{align}
Because $|\ovuvT|$ only considers columns that are do not share any tensor coordinates with $i$, it is distributed according to a Binomial with parameters $n'$ and $p^2$, where $n' = \prod_{q \in \cI_2} (n_q - 1)$.
    \begin{lem}\label{lem:overlap_tensor} Given $p > 0$, $2 \leq \beta_l < n'p^2$, $n'p^2 \leq \beta_h < n'$ and $\theta \in (0, 1)$, for any $(u,i) \in [m] \times [n]$, %***TODO \dogyoon{we may need to use a different letter than $\alpha$ here}
    	\begin{align*}
	    &\Prob{|\rowbaseT - (m-1)p| > \theta (m-1)p}\\
	    &\qquad		\leq (m-1) \exp \left( - \frac{\left(n'p^2-\beta_l\right)^2}{2n'p^2} \right) + (m-1) \exp \left( - \frac{\left(\beta_h - n'p^2\right)^2}{3n'p^2} \right)\\
	    &\qquad\qquad + 2 \exp \left( - \frac{\theta^2}{3}(m-1)p \right).
	\end{align*}
    \end{lem}

%Discuss two-step proof?
Next, assuming the overlap between two rows $u$ and $v$ is sufficiently large (but not too large), Lemmas \ref{lem:mean_tensor} and \ref{lem:variance_tensor} prove that the sample mean and variance, $\muvT$ and $\suvT$ of the difference $Z(u,i) - Z(v,i)$ concentrate around their expectations $\muuvT$ and $\siguvT^2$ with high probability. For any pair of rows $(u,v) \in [m] \times [n]$, we define two levels of empirical means and variances. As defined in the algorithm, $\muvT$ and $\suvT$ are computed from the observed entries in the overlap of $u$ and $v$, where we recall that $j \in \ovuvT$ if $(u,j) \in \cD$, $(v,j) \in \cD$, and $j_k \neq i_k$ for all $k \in [t_2]$. \begin{align*}
     \muvT &:= \frac{1}{\left| \ovuvT \right|}\left[\sum_{j \in \ovuvT} Z(u,j) - Z(v,j)\right], \\
    \suvT &:= \frac{1}{\left| \ovuvT \right| - 1}\sum_{j \in \ovuvT} \left[Z(u,j) - Z(v,j) - \muvT \right]^2.
\end{align*}
We define $\tilde{m}_{uv}(i)$ and $\tilde{s}^2_{uv}(i)$ to be the mean and variances of the differences between rows $u$ and $v$ in the full matrix $Z$ including the unobserved entries, but not including all columns $j$ which share a tensor coordinate with $i$. Recall that the set $\cN_i$ denotes columns which have no shared tensor coordinate with $i$,
 \[\cN_i := \{j \in [n] ~s.t.~ j_k \neq i_k \text{ for all } k \in [t_2]\}.\]
The remaining number of columns would be $|\cN_i| = n' = \prod_{q \in \cI_2} (n_q - 1)$ instead of $n = \prod_{q \in \cI_2} n_q$.
\begin{align*}
    \tilde{m}_{uv}(i) &:= \frac{1}{n'}\sum_{j \in \cN_i} \left[Z(u,j) - Z(v,j)\right],\\
    \tilde{s}^2_{uv}(i) &:= \frac{1}{n'-1}\sum_{j \in \cN_i} \left[Z(u,j) - Z(v,j) - \tilde{m}_{uv}(i)\right]^2.
\end{align*}
While $Z$ may be fully instantiated from the latent row and column variables along with entrywise noise terms, only the entries denoted by $\cD$ are actually observed, such that we are not actually able to compute $\tilde{m}_{uv}(i)$ and $\tilde{s}^2_{uv}(i)$ from the observed dataset. Whereas  $\tilde{m}_{uv}(i)$ and $\tilde{s}^2_{uv}(i)$ denote the sample mean and variance between a pair of rows for the given sampled columns, $\muvT$ and $\suvT$ denote the sample mean and variance between a pair of rows for the observed datapoints, which can be thought of as drawn uniformly at random without replacement from the columns.
We define $\mu_{ab}$ and $\sigma_{ab}^2$ to be the mean and variance for a fixed pair of rows with latent features $a, b \in \cX^{\pi}_1$ and for a randomly sampled column feature $\vvec{\bx}^{\pi}_2$ according to the product measure over $P_{\cX^{\pi}_{2,1}} \dots P_{\cX^{\pi}_{2,t_2}}$:
\begin{align*}
\mu_{ab} &:= \bE_{\vvec{\bx}^{\pi}_2} \left[ f(a, \vvec{\bx}^{\pi}_2) - f(b, \vvec{\bx}^{\pi}_2) \right],\\
    \sigma_{ab}^2 &:= Var_{\vvec{\bx}^{\pi}_2} \left[ f(a, \vvec{\bx}^{\pi}_2) - f(b, \vvec{\bx}^{\pi}_2) \right].
\end{align*}

Due to the fact that the latent variables across columns in the flattened matrix are correlated according to the original tensor structure, the simple proof from Lemmas \ref{lem:mean} and \ref{lem:variance} are no longer sufficient. Instead we use a 2-step analysis, which arises from the equivalent perspective of the model as generated from a 2-stage sampling procedure. In step one, the latent variables and individual noise terms are sampled according to the distributions specified in the model, i.e. each feature of a coordinate in the original tensor representation is drawn i.i.d. and the noise terms are independent, zero-mean, and bounded. The matrices $A$ and $Z$ are fully determined from the latent variables and individual noise terms. In step two, the index set $\cD$ of observed entries is sampled such that for any $(u,i) \in [m] \times [n]$, with probability $p$, $(u,i) \in \cD$ independently of other entries. The algorithm only observes the entries in $Z$ which correspond to indices specified in the set $\cD$.

To prove that $\muvT$ concentrates around $\muuvT$, we first show using McDiarmid's inequality that $\tilde{m}_{uv}(i)$ concentrates around $\muuvT$ due to the sampling of the latent variables and independent noise terms. Second we show that conditioned on  $|\ovuvT|$, $\muvT$ concentrates around $\tilde{m}_{uv}(i)$ by the Kontorovich-Ramanan inequality, since the observed datapoints are sampled without replacement from a finite set of columns. We formally state the result in Lemma \ref{lem:mean_tensor}, which upper bounds the probability of the complement of the following good event
\begin{align}
\Eb' := \left\{\left| \muvT - \muuvT\right| \leq \mslack, ~\forall~ v \in \rowbaseT \right\}.\label{eq:def_Eb}
\end{align}
%%% Lemma: Tensor Mean Concentration
\begin{lem}\label{lem:mean_tensor}
        Given $(u, i) \in [m] \times [n]$, for any $\mslack > 0$, 
        \begin{align*}
        		&	\Prob{\left|\muvT - \muuvT \right| > \mslack \left| v \in \rowbaseT \right.}\\
		&\qquad \leq 2\exp\left(\frac{-\mslack^2}{8 (LD_{\cX^{\pi}_1})^2 \sum_{q=1}^{t_2} \frac{1}{n_q-1} + \frac{16B_e^2}{n'}}\right) + 2\exp\left(\frac{- \mslack^2}{32B_0^2}\Delta\right),	
	\end{align*}
	where $\Delta = \min \left\{ \frac{n'^2\beta_l}{\left(n' + \beta_l^2\right)^2}, \frac{n'^2\beta_h}{\left(n' + \beta_h^2\right)^2} \right\}$.
\end{lem}

Similarly, to prove that $\suvT$ concentrates around $\siguvT^2 + 2 \gamma^2$, we first show using McDiarmid's inequality that $\tilde{s}^2_{uv}(i)$ concentrates around $\siguvT^2 + 2 \gamma^2$ due to the sampling of the latent variables and independent noise terms. Second we show that conditioned on  $|\ovuvT|$, $\suvT$ concentrates around $\tilde{s}^2_{uv}(i)$ by the Kontorovich-Ramanan inequality, since the observed datapoints are sampled without replacement from a finite set of columns. We formally state the result in Lemma \ref{lem:variance_tensor}, which upper bounds the probability of the complement of the following good event
\begin{align}
\Ec' := \left\{ \suvT \in \left[(1-\theta)\siguvT^2 -\vslack , (1+\theta)\siguvT^2  + \vslack \right], ~\forall~ v \in \rowbaseT \right\}.\label{eq:def_Ec}
\end{align}
%%% Lemma: Tensor Variance Concentration    
    \begin{lem}\label{lem:variance_tensor}
        Given $u \in [m], i \in [n]$, for any $\vslack > 0$,
				%and $2 \leq \beta_l \leq \beta_h \leq n^{2/3}$\chris{this condition only needed/mentioned below to make error bound vanish?}, 
        \begin{align*}
        		&	\Prob{ \suvT - 2\gamma^2  \in \left[(1-\theta) \siguvT^2 - \vslack ,   (1+\theta)\siguvT^2 + \vslack \right] \left| v \in \rowbaseT \right.}\\
		%&	\Prob{ (1-\theta) \siguvT^2 + 2\gamma^2 - \vslack \leq	\suv^2	\leq (1+\theta)\siguvT^2 + 2\gamma^2 + \vslack \left| v \in \rowbaseT \right.}\\
		&\qquad \leq 2\exp\left(\frac{-\vslack^2}{32L^2D_{\cX^{\pi}_1}^2\left( 3LD_{\cX^{\pi}_1} + 4 B_e\right)^2\sum_{q=1}^{k_2} \frac{1}{n_q - 1} + \frac{64B_e^2\left( 2LD_{\cX^{\pi}_1} + 5 B_e\right)^2}{n'}}\right)\\
		&\qquad\qquad + 2 \exp \left(\frac{- \vslack^2}{128B_0^4}  \Delta \right),	
	\end{align*}
	where $\theta = \sum_{q \in \cI_2} \frac{1}{n_q -1}$ is a quantity which depends only on the shape of the given tensor and vanishes to $0$ as $n_q \to \infty, \forall q\in\cI_2$. The overlap-dependent factor in the exponent $\Delta = \min \left\{ \frac{n'^2\beta_l}{\left(n' + \beta_l^2\right)^2}, \frac{n'^2\beta_h}{\left(n' + \beta_h^2\right)^2} \right\}$.
\end{lem}    

From Lemmas \ref{lem:mean_tensor} and \ref{lem:variance_tensor}, we observe that the error bound vanishes as $n \to \infty$ if and only if $\Delta \to \infty$, which occurs when $\beta_l = \omega \left( 1\right)$ and $\beta_h = o \left( n^{2/3}\right)$, since $\beta_l \leq \beta_h$ and $n' = \Theta(n)$ by definition.

In Lemma \ref{lem:regularity_tensor}, we prove that for any index pair $(u,i)$, there exists $k$ ``good'' neighboring rows in $\rowbaseT$, whose variance $\siguvT^2$ is sufficiently small. Unlike Lemma \ref{lem:regularity}, we cannot assume our row features are drawn independently the product latent space. However, we recall that the row features come from the original tensor structure, in which for each dimension, the latent feature associated to each coordinate is drawn independently and identically distributed. Consider a row $u$ in the flattened matrix, with a vector of latent features $\vvec{x}^{\pi}_1(\vvec{u}) = (x^{\pi}_{1,1}(u_1), \dots, x^{\pi}_{1,t_1}(u_{t_1}))$. For each dimension of the original tensor $q \in [t_1]$, by Chernoff's bound with high probability there are sufficiently many coordinates whose latent feature is close to $x^{\pi}_{1,q}(u_q)$. Then by combining these events by a simple union bound, it follows that there are sufficiently many rows $v \in [m]$ in the flattened matrix whose latent feature vector $\vvec{x}^{\pi}_1(\vvec{v})$ is close to $\vvec{x}^{\pi}_1(\vvec{u})$, implying that there are at least $k$ good neighbors. Let $\big\{\siguvT^2\big\}_{v \in \rowbaseT}^{(k)}$ denote the value of the $k$-th minimum element in the set $\big\{\siguvT^2\big\}_{v \in \rowbaseT}$. The following Lemma  \ref{lem:regularity_tensor} upper bounds the probability of the complement of the following good event
\begin{align}
\Ed' := \left\{\left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} \leq \zeta \right\}.\label{eq:def_Ed}
\end{align}
%%% Lemma: Tensor Near Neighbors
\begin{lem}\label{lem:regularity_tensor}
		Given $u \in [m]$, $i \in [n]$, for any $\zeta > 0$ and for any positive integer $k \leq \frac{1}{8}mp \phi^{\pi}_2\left( \sqrt{\frac{\zeta}{L^2}} \right) = \frac{p}{8} \prod_{q \in [t_1]} n_{\pi(q)} \phi_{\pi(q)} \left(\sqrt{\frac{\zeta}{L^2}}\right)$,
        \begin{align*}	
				&\Prob{\left. \left\{\siguvT^2\right\}_{v \in \rowbaseT}^{(k)} > \zeta ~\right|~  |\rowbaseT| \in \left[\frac{1}{2}(m-1)p, \frac{3}{2}(m-1)p\right] } \\
				&\qquad	\leq  \sum_{q \in \cI_1} \exp \left( - \frac{(1 - 2^{-1/t_1} )^2}{2} \mu_q \right) + \exp\left(-\frac{k}{8}\right)\\
				&\qquad\qquad + (m-1)\exp \left( - \frac{(n'p^2 - \beta_l )^2}{2 n'p^2} \right) +  (m-1)\exp \left( - \frac{(\beta_h - n'p^2 )^2}{3 n'p^2} \right),	
	\end{align*}
        where $\mu_q := n_{\pi(q)} \phi_{\pi(q)} \left(\sqrt{\frac{\zeta}{L^2}}\right)$ and $\phi_{\pi(q)}(r) := \ess \inf_{x' \in \cX_{\pi(q)}} \bP_{\cX_{\pi(q)}} \left(d_{\cX_{\pi(q)}}(\bx, x') \leq r\right)$.
\end{lem}

Given that there exist $k$ good neighbors in $\rowbaseT$ whose variance is small, and conditioned on the event that all the sample variances concentrate, it follows that the true variance between $u$ and its $k$ nearest neighbors are small with high probability. Each of these good events were denoted as $\Ea', \Eb', \Ec'$ and $\Ed'$, defined in \eqref{eq:def_Ea}, \eqref{eq:def_Eb}, \eqref{eq:def_Ec}, and \eqref{eq:def_Ed} respectively, and we let $E'$ denote the intersection of these good events,
\[E' := \Ea' \cap \Eb' \cap \Ec' \cap \Ed'.\]
We can provide a bound on the tail probability of the estimation error conditioned on $E'$ by using Chebyshev's inequality, similar to that in Lemma \ref{lem:estimate} with minor changes. %\chris{We will have to account for the fact that the latent variable $\vvec{x}^{\pi}_2(\vvec{i})$ associated to column $i$ is no longer independent from the events that the sample means and variances concentrate, since it is correlated to the latent variables of other columns as well. ... this comment no needed after fix}
%%% Lemma: Tensor Chebyshev
\begin{lem}\label{lem:estimate_tensor}
Given $\mslack > 0$, $\vslack > 0$, for any $\eps > \mslack$, $\zeta \geq 0$ and any positive integer $k \leq \frac{1}{8}mp \phi^{\pi}_1\left( \sqrt{\frac{\zeta}{L^2}} \right)$, the tail probability of the estimation error is bounded by
\[\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps ~|~ E'} \leq \frac{1}{(\eps - \mslack)^2} \left( \frac{(1+\theta) \zeta + 2 \vslack}{1-\theta} + \frac{\gamma^2}{k} \right).\]
       where %$\mu_q := n_q \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right)$ and
%$\phi_q(r) := \ess \inf_{x' \in \cX_q} \bP_{\cX_q} \left(d_{\cX_q}(\bx, x') \leq r\right)$, and 
$\theta = \sum_{q \in \cI_2} \frac{1}{n_q -1}$ is a quantity which depends only on the shape of the given tensor and vanishes to $0$ as $n_q \to \infty, \forall q\in\cI_2$.
\end{lem} 

Then we bound the ``bad'' event, denoted by the complement of $E'$ according to the above definition. 
    \begin{lem}\label{lem:bad_event_bound} Suppose that
        \begin{align*}
		& \max \left\{ m^{-1 + \delta}, n'^{-\frac{1}{2} + \delta} \right\} \leq p \leq n'^{-\frac{1}{6}- \delta} ~\text{ for some } \delta > 0\\
		&\forall q \in \cI_1, \zeta \text{ satisfies } \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right)\geq c_{q} n_q^{-\frac{\log mp}{2 \log m}} \text{ for some } c_{q} > 0,\\
		&2 \leq \beta_l \leq c_l \min\left\{ n'p^2, n'^{1/2}\right\} \text{ for some }c_l \in (0, 1),\\
		& c_h \max \left\{ n'^{1/2}, n'p^2 \right\} \leq \beta_h \leq n'^{\frac{2}{3}-\delta}\text{ for some }c_h > 1 \text{ and}\\
		&k \leq \frac{1}{8}mp \phi^{\pi}_1\left( \sqrt{\frac{\zeta}{L^2}} \right) = \frac{p}{8} \prod_{q \in \cI_1} n_q \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right).
	\end{align*}
Then 
     \begin{align*}
	\Prob{E'^c}	&	\leq 4(m-1) \exp \left( -C_1 n'p^2 \right) + 2 \exp \left( - \frac{1}{24} mp \right)\\
	&\qquad	+ 6 (m-1)p \exp \left( -C_2 (n_{q^*} - 1)^{1/3}\right) + 6(m-1)p \exp \left( -C_3 \min \left\{ \frac{n'^{2/3}}{4\beta_h}, \frac{\beta_l^{1/3}}{4} \right\} \right)\\
	&\qquad	+ t_1 \exp \left( -C_4 n_{q^*}^{1/2}\right) + \exp \left( -\frac{k}{8}\right).
    \end{align*}
where $q^* := \arg \min_{q \in \cI_1} n_q$ and $\mslack = \vslack = \max\left\{ (n_{q^*} - 1)^{-1/3}, \left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}$. Here, $\theta = \sum_{q \in \cI_2} \frac{1}{n_q -1 }$ is a quantity which depends only on the shape of the given tensor and vanishes to $0$ as $n_q \to \infty, \forall q\in\cI_2$.
Note that
    \begin{align*}
        C_1 &:= \min \left\{ \frac{(1-c_l)^2}{2}, \frac{(c_h-1)^2}{3} \right\},\\
        C_2 &:= \min \left\{ \frac{1}{8L^2D^2 t_2 + 16B_e^2}, \frac{1}{32L^2D^2(3LD + 4B_e)^2 t_2 + 64B_e^2(2LD + 5B_e)^2}  \right\},\\
        C_3 &:= \min \left\{ \frac{1}{32(LD + 2B_e)^2}, \frac{1}{128(LD+2B_e)^4} \right\},\\
        C_4&:= \min_{q \in \cI_q} \left\{ \frac{(1-2^{-1/t_1})^2}{2} c_q \right\}
    \end{align*}
are some absolute constants, which may depend only on the geometry of the latent spaces.
    \end{lem}
		
		
%%% Tensor Tail bound
Finally we combine the lemmas which bound each of the deviating events to get a final bound on the tail probability of the error. 

%\dogyoon{***TODO: may want to discuss a bit on the constraint on the sample complexity - that is actually a condition on the matricization rather than the sample complexity; in the sense that it wouldn't matter when $t= 2$}

%\dogyoon{***TODO: $\delta$ plays the role of a ``slack''  - it may be needed to deal with it more properly}
    \begin{thm}\label{thm:tensor_tail} Suppose that
        \begin{align*}
		& \max \left\{ m^{-1 + \delta}, n'^{-\frac{1}{2} + \delta} \right\} \leq p \leq n'^{-\frac{1}{6}- \delta} ~\text{ for some } \delta > 0\\
		&\forall q \in \cI_1, \zeta \text{ satisfies } \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right)\geq c_{q} n_q^{-\frac{\log mp}{2 \log m}} \text{ for some } c_{q} > 0,\\
		&2 \leq \beta_l \leq c_l \min\left\{ n'p^2, n'^{1/2}\right\} \text{ for some }c_l \in (0, 1),\\
		& c_h \max \left\{ n'^{1/2}, n'p^2 \right\} \leq \beta_h \leq n'^{\frac{2}{3}-\delta}\text{ for some }c_h > 1 \text{ and}\\
		&k \leq \frac{1}{8}mp \phi^{\pi}_1\left( \sqrt{\frac{\zeta}{L^2}} \right) = \frac{p}{8} \prod_{q \in \cI_1} n_q \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right).
	\end{align*}
	For any given $\eps > \max\left\{  \max_{q \in \cI_1} \left((n_q-1 )^{-1/3}\right), \left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}$, the tail probability of the error of the estimate produced by the user-user $k$-smoothed variant of our method with overlap parameters $\beta_l, \beta_h$ is upper bounded by:
     \begin{align*}
	&\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}\\
	&	\leq \frac{1}{(\eps - \mslack)^2} \left(\frac{(1+\theta) \zeta + 2 \vslack}{1-\theta} + \frac{\gamma^2}{k} \right) + \Fc',
    \end{align*}
		where 
    \begin{align*}
	\Fc'&= 4(m-1) \exp \left( -C_1 n'p^2 \right) + 2 \exp \left( - \frac{1}{24} mp \right)\\
		&\qquad	+ 6 (m-1)p \exp \left( -C_2 (n_{q^*} - 1)^{1/3}\right) + 6(m-1)p \exp \left( -C_3 \min \left\{ \frac{n'^{2/3}}{4\beta_h}, \frac{\beta_l^{1/3}}{4} \right\} \right)\\
		&\qquad	+ t_1 \exp \left( -C_4 n_{q^*}^{1/2}\right) + \exp \left( -\frac{k}{8}\right),
    \end{align*}
		with $q^* := \arg \min_{q \in \cI_1} n_q$ and $\mslack = \vslack = \max\left\{ (n_{q^*}-1)^{-1/3}, \left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}$. Here, $\theta = \sum_{q \in \cI_2} \frac{1}{n_q -1}$ is a quantity which depends only on the shape of the given tensor and vanishes to $0$ as $n_q \to \infty, \forall q\in\cI_2$.
Note that
    \begin{align*}
        C_1 &:= \min \left\{ \frac{(1-c_l)^2}{2}, \frac{(c_h-1)^2}{3} \right\},\\
        C_2 &:= \min \left\{ \frac{1}{8L^2D^2 t_2 + 16B_e^2}, \frac{1}{32L^2D^2(3LD + 4B_e)^2 t_2 + 64B_e^2(2LD + 5B_e)^2}  \right\},\\
        C_3 &:= \min \left\{ \frac{1}{32(LD + 2B_e)^2}, \frac{1}{128(LD+2B_e)^4} \right\},\\
        C_4&:= \min_{q \in \cI_q} \left\{ \frac{(1-2^{-1/t_1})^2}{2} c_q \right\}
    \end{align*}
are some absolute constants, which may depend only on the geometry of the latent spaces.
    \end{thm}


%%% MSE
By integrating the upper bound on the tail of the error probability, we obtain an upper bound on the MSE of the estimate, as stated in the final Theorem \ref{thm:main_tensor}.










%================ Contents below this line are not printed ============================
\iffalse{
Recall from results in Section \ref{sec:main.result}, we require the fraction of observed entries, $p$ to scale at least as $\max\left( m^{-1 + \delta}, n^{-1/2 + \delta} \right)$. That is, from a given total number of entries $mn$, we need to observe effectively
$N = \max(n, m \sqrt{n})$ entries (ignoring the $\delta > 0$ exponent). Given choice of selecting $m, n$ while keeping $mn = \prod_r k_r$ fixed, the $N$ is minimized when we select $n = m^2$ leading to $N \sim (mn)^{2/3}$. This suggests that we should flatten tensor in such a way that $|\cT_1|^2 \sim |\cT_2|$. With this insight, for a symmetric tensor (i.e. $k_1 = \dots = k_t$), we summarize the following result. 
\begin{thm} \label{tensor:simple}
For a $t$-order tensor $T \in \Reals^{\ell^t}$, given any partition $(\cT_1, \cT_2)$ of $[t]$, let $A_T$ denote the equivalent matrix which results from flattening the tensor according to the partition $(\cT_1, \cT_2)$ with $|\cT_1| \leq |\cT_2|$. Assume that the latent space is a compact set in $\Reals^d$ equipped with the Lebesgue probability measure. Suppose that $p \geq \max\left( \ell^{-|\cT_1|/3 + \delta}, \ell^{-|\cT_2|/2 + \delta} \right)$ for some $\delta > 0$. The $k$-smoothed estimator with $\beta = \ell^{|\cT_2|} p^2/2$ and $k = \frac{(\ell^{|\cT_1|}-1)p}{4}\max((\ell^{|\cT_2|}p^2)^{-d/2}, (\ell^{|\cT_1|}p)^{-2/3})$ achieves
        \[	MSE(\hat{A_T}) = \tilde{O}(L^2 \max((\ell^{|\cT_2|}p^2)^{-1/3}, (\ell^{|\cT_1|}p)^{-4/3d}) + \gamma^2 (\ell^{|\cT_1|}p)^{-1/3}). \]
\end{thm}

\begin{proof}
 Given a tensor $T \in \Reals^{\ell^t}$ and a bipartition $(\cT_1, \cT_2)$ of the index set $[t]$, we can unfold a tensor into a matrix $A_T$ according to that mode so that each tuple in $[\ell]^{\cT_1}$ and in $[\ell]^{\cT_2}$ encode the row and column indices of $A_T$. Plugging in the number of rows $m = \ell^{|\cT_1|}$ and the number of columns $n = \ell^{|\cT_2|}$ in Theorem \ref{main:simple} leads to an desired upper bound. As suggested above, we can achieve an minimal sample complexity requirement $p \geq \ell^{-t/3 + \delta}$ for some $\delta > 0$ by taking a partition $(\cT_1, \cT_2)$ of $[t]$ such that $|\cT_1| = t/3$ and $|\cT_2| = 2t/3$.
\end{proof}
}\fi


==> contents/tensor_proof/tensor_proofs.tex <==
%%% Tensor Tail bound
\subsection{Proof of Main Results for Tensor Completion}

\begin{proof}[Proof of  Theorem \ref{thm:tensor_tail}]
The proof follows from simply combining the results from Lemmas  \ref{lem:estimate_tensor} and \ref{lem:bad_event_bound}. By conditioning on event $E'$, it follows that
	\begin{align*}
			\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}	
			&\leq \Prob{\left.\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| E'}  +  \Prob{E'^c}.
	\end{align*}
	
	By Lemma \ref{lem:estimate_tensor},
	\begin{align*}
			\Prob{\left. \left| A(u,i) - \hat{A}^k(u,i) \right| > \eps \right| E'}	&\leq  \frac{1}{(\eps - \mslack)^2} \left(\frac{(1+\theta) \zeta + 2 \vslack}{1-\theta} + \frac{\gamma^2}{k} \right).
	\end{align*}

By Lemma \ref{lem:bad_event_bound}, $\Prob{E'^c} \leq \Fc' $ for
\begin{align*}
\Fc'	&= 4(m-1) \exp \left( -c_1 n'p^2 \right) + 2 \exp \left( - \frac{1}{24} mp \right)\\
&\qquad	+ 6 (m-1)p \exp \left( -c_2 (n_{q^*}-1)^{1/3}\right) + 6(m-1)p \exp \left( -c_3 \min \left\{ \frac{n'^{2/3}}{4\beta_h}, \frac{\beta_l^{1/3}}{4} \right\} \right)\\
&\qquad	+ t_1 \exp \left( -c_4 n_{q^*}^{1/2}\right) + \exp \left( -\frac{k}{8}\right),
\end{align*}
where $q^* := \arg \min_{q \in \cI_1} n_q$, and $ c_1, c_2, c_3, c_4$ are some absolute constants derived in Lemma \ref{lem:bad_event_bound}, which may depend only on the geometry of the latent spaces.

Therefore, 
     \begin{align*}
	\Prob{\left| A(u,i) - \hat{A}^k(u,i) \right| > \eps}
	&	\leq \frac{1}{(\eps - \mslack)^2} \left(\frac{(1+\theta) \zeta + 2 \vslack}{1-\theta} + \frac{\gamma^2}{k} \right) + \Fc'.
    \end{align*}
		
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:main_tensor}]
    The proof is the same with that of Theorem \ref{thm:main_theorem}, and follows by integrating the tail of the probability bound presented in Theorem \ref{thm:tensor_tail}.
\end{proof}



\subsection{Results Given an Optimal Flattening and Uniform Probability Measure}

In this section, we simplify the results from Theorem \ref{thm:main_tensor} when the latent probability measure is a uniform measure over a $d$ dimensional Euclidean cube. We thus compute the specific form of the underestimator function $\phi^{\pi}_1(\cdot)$, which leads to concrete bounds. We then choose specific expressions for $\zeta$, and $k$ to ensure that the mean squared error of our user-user $k$-nearest neighbor algorithm converges to zero. The parameter $\zeta$ in Theorem \ref{thm:main_tensor} is introduced purely for the purpose of analysis, and is not used within the implementation of the the algorithm. Recall that it is used to define event $\Ed'$, which holds when the $k$ rows in $\rowbaseT$ with minimum variance all satisfy $\siguvT \leq \zeta$.  Intuitively, $\zeta$ is the thresholding parameter for the membership of similar neighbors. 


\begin{proof}[Proof of Corollary \ref{coro:uniform_tensor}]

Recall that we assumed an equilateral tensor with $n_q = l$ for all $q \in [t]$, and we assumed that the algorithm is applied to a user-optimally flattened tensor, such that $|\cI_1| = t - \lfloor \frac{2t}{3}\rfloor$, and $|\cI_2| = \lfloor\frac{2t}{3}\rfloor$. Therefore,
    \begin{align*}
    	l^{\frac{t}{3}} \leq m &= l^{t - \lfloor \frac{2t}{3}\rfloor} \leq l^{\lceil\frac{t}{3}\rceil},\\
	l^{\lfloor\frac{2t}{3}\rfloor} \leq n &= l^{\lfloor\frac{2t}{3}\rfloor} \leq l^{\frac{2t}{3}},\\
	(l-1)^{\lfloor\frac{2t}{3}\rfloor} \leq n &= (l-1)^{\lfloor\frac{2t}{3}\rfloor} \leq (l-1)^{\frac{2t}{3}}.
    \end{align*}

When the latent space for each coordinate $q \in \cI_1$ is a cube in $\Reals^d$ equipped with the uniform probability measure, then for $q \in \cI_1$,
\[ \phi_q\left( \sqrt{\frac{\zeta}{L^2}} \right) = C(2L)^{-d} \zeta^{d/2},\]
where $C$ is a normalization constant to ensure $\phi_q(\cX_q) = 1$. Therefore, the corresponding underestimator function of the corresponding product space is
\begin{align*}
\phi^{\pi}_1\left(\sqrt{\frac{\zeta}{L^2}}\right) 
&= \prod_{q \in \cI_1} \phi_q \left(\sqrt{\frac{\zeta}{L^2}}\right) \\
&= \left(C (2L)^{-d} \zeta^{d/2} \right)^{t_1}.
\end{align*}
As specified in the conditions of Theorem \ref{thm:main_tensor}, we need to choose $\zeta$ so that for all $q$, 
\begin{equation}
\phi_q\left(\sqrt{\frac{\zeta}{L^2}}\right) = C(2L)^{-d} \zeta^{d/2} \geq c_q n_q^{-\frac{\log mp}{2 \log m}} \text{ for some } c_q \geq 0.
\end{equation}
Therefore we need
\begin{align}
\zeta \geq \left(\frac{c_q}{C}\right)^{2/d} (2L)^{2} n_q^{-\frac{\log mp}{d \log m}}
\end{align}
for all $q$. Since $m = l^{|\cI_1|}$ and $n_q = l ~\forall~ q$, it follows that
    $$    n_q^{-\frac{\log mp}{\log m}} = l^{-\frac{\log mp}{|\cI_1|\log l}} = \left(mp\right)^{-\frac{1}{|\cI_1|}}. $$
    Therefore, we will let $c_q = 1$, and choose $\zeta = \frac{ (2L)^2}{C^\frac{2}{d}} \left(mp\right)^{-\frac{1}{d|\cI_1|}}$, which satisfies the above conditions.

Since we have $\phi_{q}\left( \sqrt{\frac{\zeta}{L^2}}\right) \geq \left( mp \right)^{-\frac{1}{2|\cI_1|}}$ for each $q \in \cI_1$, taking $k = \frac{1}{8} \sqrt{mp}$ satisfies the required condition that
     $$k = \frac{mp}{8} \left( \left(mp\right)^{-\frac{1}{2|\cI_1|}} \right)^{|\cI_1|} \leq\frac{mp}{8} \phi^{\pi}_{q} \left( \sqrt{\frac{\zeta}{L^2}}\right).$$

The assumption that $p \geq \max \left\{ m^{-1 + \delta}, n'^{-\frac{1}{2} + \delta} \right\}$ for some $\delta > 0$ guarantees that $mp$ and $n'p^2$ diverge to $\infty$ as $m, n \to \infty$, which occurs when $l \to \infty$. For the choice of $\beta_l = \frac{1}{2} \min \left\{ n'p^2, \sqrt{n'}\right\}$ and $\beta_h = 2 \max \left\{ n'p^2, \sqrt{n'}\right\}$, we can verify that $\Fb' \to 0$ and $l \to \infty$.  By definition
    $$\Fb' = \max\left\{ \left(n_{q^*} -1\right)^{-1/3}, \left( \frac{n'^2}{\beta_h^3} \right)^{-1/3}, \beta_l^{-1/3}\right\}.$$
    Each of these terms shrink to $0$ as $l \to \infty$, using the fact that $p \geq n'^{-\frac{1}{2} + \delta}$, and $p \leq n'^{-\frac{1}{6}- \delta}$ for some $\delta > 0$,
    \begin{align*}
        \left(n_{q^*}-1\right)^{-1/3} &= (l-1)^{-1/3},\\
         \left(\frac{n'^2}{\beta_h^3}\right)^{-1/3} & = \frac{2 \max \left\{ n'p^2, \sqrt{n'}\right\}}{n'^{2/3}} \leq 2 \max \left\{ n'^{-2\delta}, n'^{-1/6} \right\}, \\
         \beta_l^{-1/3} &= \left(\frac{1}{2}\min \left\{ n'p^2, \sqrt{n'} \right\}\right)^{-1/3} \leq \left(\frac{1}{2} \min \left\{ n'^{2\delta}, \sqrt{n'}\right\}\right)^{-1/3}.
    \end{align*}
		
    Next, we will show $\Fa' \to 0$ as $l \to \infty$. First of all, $\theta = \sum_{q \in \cI_1} \frac{1}{n_q-1} = \frac{t - \lfloor \frac{2t}{3}\rfloor}{l-1} \leq \frac{t}{l-1} \to 0$ as $l \to \infty$. To be more specific, we can assume that $\theta \leq \frac{1}{2}$ whenever $l \geq 2t + 1$. Therefore, by plugging in the conditions on $\theta$ and the expressions for $\zeta, k,n', $ and $\Fb'$, it follows that
\begin{align*}
         \Fa' &= \frac{(1+\theta) \zeta + 2 \Fb'}{1-\theta} + \frac{\gamma^2}{k}\\
         		&\leq 3\zeta + 4\Fb' + \frac{\gamma^2}{k}\\
		&\leq \left[ 3\frac{ (2L)^2}{C^{\frac{2}{d}}} + 4 + 8\gamma^2 \right]\max\left\{ (mp)^{-\frac{1}{d|\cI_1|}}, (l-1)^{-\frac{1}{3}}, \frac{\beta_h}{(l-1)^{\frac{2}{3}|\cI_2|}}, \beta_l^{-\frac{1}{3}}, (mp)^{-\frac{1}{2}} \right\}\\
		&\to 0 \quad as ~l \to \infty.
     \end{align*}

To show that $\Fc'$ decays exponentially fast as $l$ grows, we need to show that the exponents in each of the terms in $\Fc'$ (see the expression in Theorem \ref{thm:main_tensor}) grow faster than the multiplicative coefficients in front. The multiplicative factors $4(m-1)p, 6(m-1)p, t_1$ contribute at most only a logarithmic increase in $l$ when included into the exponents. By showing that the exponents grow polynomially with $l$, it follows that $\Fc'$ decays exponentially with $l$. We can verify this by simply plugging in the choices for $n'$, $m$, $n_q$, $k$, $\beta_l$ and $\beta_h$, and additionally using the conditions that $\max \left\{ m^{-1 + \delta}, n'^{-\frac{1}{2} + \delta} \right\} \leq p \leq n'^{-\frac{1}{6}- \delta}$ for some $\delta > 0$. We list the simplified expressions for each of the terms in the exponents below, showing that they indeed increase polynomially in $l$.
    \begin{align*}
        n'p^2 & \geq (l-1)^{\frac{2t}{3}\delta},\\
        mp &\geq l^{\frac{t}{3}\delta},\\
        (n_{q^*}-1)^{1/3} &= (l-1)^{1/3},\\
        n_{q^*}^{1/2} &= l^{1/2},\\
        k &= \frac{1}{8}\sqrt{m} \geq \frac{1}{8} l^{\frac{t}{6}} \\
        \frac{n'^{\frac{2}{3}}}{\beta_h} &= \frac{1}{2} \min \left\{ n'^{\frac{1}{6}}, \frac{n'^{\frac{2}{3}}}{n'p^2} \right\} \geq \frac{1}{2} \min \left\{ n'^{\frac{1}{6}}, n'^{2\delta} \right\} \\
        \frac{\beta_l^{\frac{1}{3}}}{4} &= \frac{1}{4\sqrt[3]{2}} \min\left\{ \left(n'p^2 \right)^{\frac{1}{3}}, n'^{\frac{1}{6}} \right\}\geq \frac{1}{4\sqrt[3]{2}} \min\left\{ n'^{\frac{2}{3}\delta}, n'^{\frac{1}{6}} \right\}.
    \end{align*}
 
From the definition of expression $\Fa'$ in Theorem \ref{thm:main_tensor}, it follows that $\Fa' \geq \frac{2 \Fb'}{1-\theta} \geq 2\Fb'$, because $\theta = \sum_{q \in \cI_2} \frac{1}{n_q -1} = \frac{\lfloor \frac{2t}{3}\rfloor}{l-1} \in (0, 1]$. Therefore, if we can certify that $\Fc'$ decays exponentially fast as $l$ (and thus $n$ and $m$) grows, and that $\Fa' \leq \frac{1}{2}$ when $l$ is sufficiently large compared to $t$, then by the same lines of argument as in the proof of Corollary \ref{coro:uniform}, we can argue that $\Fa'$ dominates the mean-squared-error thereby achieving a similar form of diminishing error bound.

We then simplify the remaining terms assuming $\Fa' \leq \frac{1}{2}$. This can be assumed once we show that $\Fa' \to 0$ as $l \to \infty$, which can be deduced from observing that $\Fb' \to 0$, $\zeta \to 0$, $\theta \to 0$, and $k \to \infty$ as $l \to \infty$ as $l \to \infty$. If $\Fa' \leq \frac{1}{2}$ is assumed, we can apply the same idea as in the proof of Corollary \ref{coro:uniform}, where we upper bound $\Fb' \leq \frac{1}{2}\Fa'$, and then simplify the terms in the MSE bound presented in Theorem \ref{thm:main_tensor} using $\log \left(\frac{2B_0}{\Fa'}\right) \geq 1$ as long as $\Fa' \leq \frac{1}{2}$ and $B_0 \geq 1$:
    \begin{align}
        MSE(\hat{A}) &\leq  2 \Fa' \ln \left( \frac{2B_0}{\Fa'}\right) + \left(\Fa' + \Fb' \right)^2 + 2\Fb' + 4B_0^2 \Fc' \nonumber\\
				  &\leq 2 \Fa' \ln \left( \frac{2B_0}{\Fa'}\right) + \frac{9}{4}\Fa' + \Fa' + 4B_0^2 \Fc' \nonumber\\
        		&\leq \frac{21}{4} \Fa' \ln \left( \frac{2B_0}{\Fa'}\right) + 4 B_0^2 \Fc'. \label{eqn:tensor_simplified}
    \end{align}

    Plugging the bounds for $\Fa'$ and $\Fc'$ into Eq. \eqref{eqn:tensor_simplified} gives the simplified bound presented in Corollary \ref{coro:uniform_tensor}.
    \end{proof}





%================ Contents below this line are not printed ============================
\iffalse{
Recall from results in Section \ref{sec:main.result}, we require the fraction of observed entries, $p$ to scale at least as $\max\left( m^{-1 + \delta}, n^{-1/2 + \delta} \right)$. That is, from a given total number of entries $mn$, we need to observe effectively
$N = \max(n, m \sqrt{n})$ entries (ignoring the $\delta > 0$ exponent). Given choice of selecting $m, n$ while keeping $mn = \prod_r k_r$ fixed, the $N$ is minimized when we select $n = m^2$ leading to $N \sim (mn)^{2/3}$. This suggests that we should flatten tensor in such a way that $|\cT_1|^2 \sim |\cT_2|$. With this insight, for a symmetric tensor (i.e. $k_1 = \dots = k_t$), we summarize the following result. 
\begin{thm} \label{tensor:simple}
For a $t$-order tensor $T \in \Reals^{\ell^t}$, given any partition $(\cT_1, \cT_2)$ of $[t]$, let $A_T$ denote the equivalent matrix which results from flattening the tensor according to the partition $(\cT_1, \cT_2)$ with $|\cT_1| \leq |\cT_2|$. Assume that the latent space is a compact set in $\Reals^d$ equipped with the Lebesgue probability measure. Suppose that $p \geq \max\left( \ell^{-|\cT_1|/3 + \delta}, \ell^{-|\cT_2|/2 + \delta} \right)$ for some $\delta > 0$. The $k$-smoothed estimator with $\beta = \ell^{|\cT_2|} p^2/2$ and $k = \frac{(\ell^{|\cT_1|}-1)p}{4}\max((\ell^{|\cT_2|}p^2)^{-d/2}, (\ell^{|\cT_1|}p)^{-2/3})$ achieves
        \[	MSE(\hat{A_T}) = \tilde{O}(L^2 \max((\ell^{|\cT_2|}p^2)^{-1/3}, (\ell^{|\cT_1|}p)^{-4/3d}) + \gamma^2 (\ell^{|\cT_1|}p)^{-1/3}). \]
\end{thm}

\begin{proof}
 Given a tensor $T \in \Reals^{\ell^t}$ and a bipartition $(\cT_1, \cT_2)$ of the index set $[t]$, we can unfold a tensor into a matrix $A_T$ according to that mode so that each tuple in $[\ell]^{\cT_1}$ and in $[\ell]^{\cT_2}$ encode the row and column indices of $A_T$. Plugging in the number of rows $m = \ell^{|\cT_1|}$ and the number of columns $n = \ell^{|\cT_2|}$ in Theorem \ref{main:simple} leads to an desired upper bound. As suggested above, we can achieve an minimal sample complexity requirement $p \geq \ell^{-t/3 + \delta}$ for some $\delta > 0$ by taking a partition $(\cT_1, \cT_2)$ of $[t]$ such that $|\cT_1| = t/3$ and $|\cT_2| = 2t/3$.
\end{proof}
}\fi


==> contents/tensor_results/tensor_survey.tex <==


%\subsection{Background}	
%	*** Literature Review
%\cite{, Bazerque2013, Bhaskara2014, Xu2013, Yuan2015, Barak2015, Zhang2015, , Krishnamurthy2013, RP2013, LS2013, Kressner2014, Tang2015, , }




%%% ======== materials below do not appear ====================
\iffalse{
\begin{itemize}
    \item	Can we go beyond low rank regime? What benefits can we achieve?
        \subitem	Sample complexity: $C^6 nr \log^2 n$ observations (from Candes-Tao)
    \item	tensor completion by flattening
        \subitem	Many tensor methods rely on flattening	[Liu, Musialski, Wonka, Ye], [Gandy, Recht, Yamada],			
[Signoretto, De Lathauwer, Suykens],	[Tomioko, Hayashi, Kashima], [Mu, Huang, Wright, Goldfarb]
        \subitem	When $n_1 = n_2 = n_3$, we would need $\tilde{O}(n^2 r)$
        \subitem	Sum-of-squares approach requires $\tilde{O}(n^{3/2} r)$, which is nearly optimal (through 3SAT reduction) [Barak, Moitra]
\end{itemize}
}\fi
